The Graph Lottery Ticket Hypothesis: Finding Sparse, Informative Graph Structure

Graph learning methods help utilize implicit relationships among data items, thereby reducing training label requirements and improving task performance. However, determining the optimal graph structure for a particular learning task remains a challenging research problem. In this work, we introduce the Graph Lottery Ticket (GLT) Hypothesis - that there is an extremely sparse backbone for every graph, and that graph learning algorithms attain comparable performance when trained on that subgraph as on the full graph. We identify and systematically study 8 key metrics of interest that directly influence the performance of graph learning algorithms. Subsequently, we define the notion of a "winning ticket" for graph structure - an extremely sparse subset of edges that can deliver a robust approximation of the entire graph's performance. We propose a straightforward and efficient algorithm for finding these GLTs in arbitrary graphs. Empirically, we observe that performance of different graph learning algorithms can be matched or even exceeded on graphs with the average degree as low as 5.

==> data/clustering/amazon_electronics_computers.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 33.01907603048968 3.619786147287054 97.80443474363322 34.754981902303676 33.01907603048968 3.619786147287054 97.80443474363322 34.754981902303676 28.850845388736467 3.5996790911996457 97.14620095105404 30.78725749037185 27.093523154681847 4.242458635097276 91.2451997087127 28.782626785863997 27.36081070952488 4.268304300026945 91.71554094281412 29.038793604223866 19.856680315282198 10.790342036139222 71.63650621427512 34.79069348419087
1.2 34.18963883809413 4.45090102034883 96.79881562198187 35.90554423944291 34.18963883809413 4.45090102034883 96.79881562198187 35.90554423944291 29.109015468658413 3.8789089674938757 96.03242480986547 30.99938562459649 29.925869678372912 7.333600264118073 86.22539228467151 31.47733009048887 31.061620255828736 7.202526141020574 87.03591827012409 32.56969977633985 21.450699443166503 12.708894837799917 71.07706963849532 35.631687588802144
1.3 35.10864306479265 5.72980432044823 95.60980088665842 36.754696607573855 35.10864306479265 5.72980432044823 95.60980088665842 36.754696607573855 29.21434551030298 4.018499585311108 94.88700724986427 31.11834768641325 33.17504406311868 13.168167479808012 82.69081962041162 34.6557350882294 34.046018525897736 10.590184410847467 83.79106594580372 35.45248189029743 22.58766238405033 12.835959319089469 69.8770616718036 36.0360789895087
1.4 35.173041506344966 5.911990027387494 94.40282761369316 36.817359629613115 35.173041506344966 5.911990027387494 94.40282761369316 36.817359629613115 29.598708581528044 4.0425185706703015 94.03308573774953 31.490502654438192 35.66820035338434 16.42340098466737 79.95575109345255 37.087035626879825 37.173269025730896 15.01430584720686 81.4192399189094 38.51195323160931 23.879978032886314 14.388248582231261 69.10222891837859 36.70540878246814
1.5 37.518041031065756 7.484635758706619 93.59741947409834 39.065316015488385 37.518041031065756 7.484635758706619 93.59741947409834 39.065316015488385 30.112691955206277 4.433222874439342 93.09504963020231 31.970427983445937 38.232399522146224 20.59918084594965 78.06259112809934 39.6119999106829 39.78688249390377 19.58652350559083 79.72767818934432 41.07624673594685 25.139166859141078 15.47096540139002 68.69391980992269 37.35424239130837
2.0 42.03293772306732 11.228308672765372 90.13477972318263 43.3661030503299 42.03293772306732 11.228308672765372 90.13477972318263 43.3661030503299 31.846064809761852 6.184203023808985 89.37648069057825 33.843755461495476 43.33835675056136 27.272668321957088 72.64790154332375 44.67072804412025 47.33115244654728 31.67423796413097 76.0217114863127 48.49417734995871 30.123492129443463 20.752450421608657 66.38350104961907 39.89864732998876
2.5 45.150438396584505 15.885611344990291 88.1636519809588 46.35975141315666 45.150438396584505 15.885611344990291 88.1636519809588 46.35975141315666 33.77943672059885 8.33367557839836 88.31996021505407 35.73903044412708 45.925368515767396 29.267401416422494 70.05987658815059 47.21894335838673 49.46065060960626 33.359968787032955 74.86262846471857 50.58566532788949 32.73899356388269 21.922090677487617 65.50019272028081 41.03916891827854
3.0 47.59457202266056 18.856717668949766 86.93049799013932 48.732641394468125 47.59457202266056 18.856717668949766 86.93049799013932 48.732641394468125 35.33437222219254 10.301044453574844 87.47415873743473 37.31202379190947 46.401548548358384 30.174119987383204 68.18031907385482 47.72349986275053 50.72911387276478 34.53910189886742 73.92816820236388 51.827653096835846 34.9105978995048 22.59641806094565 64.75552635329304 41.99530127057851
3.5 48.924018861898524 20.463065380552596 86.0274123533364 50.03600152261421 48.924018861898524 20.463065380552596 86.0274123533364 50.03600152261421 36.063682842031625 10.951503085256467 86.95447155120715 37.971785269317664 45.63259889624432 28.7196804948065 67.00739834001352 46.94519974469628 50.148977031372475 34.89634521233968 72.49212246699095 51.297390543205424 36.422079083497415 23.205177466471017 64.45819311944751 42.53263585919139
4.0 49.878667960285455 21.499536805694735 85.31643197919132 50.95077285231725 49.878667960285455 21.499536805694735 85.31643197919132 50.95077285231725 37.57290998050603 11.950587306965604 86.32485513156871 39.44916333523412 46.70683234457068 28.179489265348412 66.77846072201824 47.981292650179384 51.125346939262194 36.82837434574712 72.32263969472726 52.26025505913615 38.90063108693791 24.128741147701877 64.26781298521833 44.2097060064521
4.5 49.89713310588851 20.83005854699607 84.54106210115778 50.97083565612508 49.89713310588851 20.83005854699607 84.54106210115778 50.97083565612508 37.80613948513903 12.403177144922948 86.10293835360787 39.558279885885284 47.74382153908366 30.308497000252434 66.58245834239148 48.9841109609637 51.706712223593975 35.44504189353061 73.07717389526135 52.80657678568841 41.141338576751544 26.314768932236433 64.52064152493978 45.752849858263865
5.0 51.065033452139616 22.111068208385163 84.05808944162555 52.11524495620312 51.065033452139616 22.111068208385163 84.05808944162555 52.11524495620312 39.63865825788356 13.356910486045503 85.34427885070515 41.26213868555009 48.10755365068009 28.702307762207667 66.24010209636799 49.3125361056992 52.47841323042768 35.27195155894963 72.95273564016821 53.54564762453575 42.18229791118245 26.7937832858815 64.28767666554951 46.3019340711821
5.5 51.558191412826716 22.14527965856664 83.30803009908863 52.590068908259546 51.558191412826716 22.14527965856664 83.30803009908863 52.590068908259546 40.34035717884123 13.842300690833229 84.511823564624 41.944411602983436 47.74722877472242 29.507896255766415 65.6941398332172 48.95987794387226 52.9829691423105 36.021296176692395 72.94047838704381 54.03559524854201 42.993217443166074 25.58207202254491 64.2953911085348 46.701388058297184
6.0 51.34126942699051 22.17334278752997 82.81037579987446 52.37780265471804 51.34126942699051 22.17334278752997 82.81037579987446 52.37780265471804 41.88902249267274 15.761000478262845 83.23003140028466 43.463466927756905 48.515167120968954 28.47210440316622 65.67459365504062 49.681914891025045 52.60960273998181 36.26042839311127 72.68301704707142 53.670615608051385 44.002604359836006 25.876662247852 64.28119953624541 47.362195371684926
6.5 51.595403880424165 23.614374898818504 82.26378180812958 52.61788930025365 51.595403880424165 23.614374898818504 82.26378180812958 52.61788930025365 44.15547454171814 17.599039658702118 82.55889075703384 45.57997646205328 49.07608288897784 29.14979193128596 65.41483513125922 50.23511855318774 52.88213567016786 36.190841565653436 72.60475202715642 53.932446508399835 44.85623339536461 26.692707619301743 64.35636556501521 47.9377581825307
7.0 52.780796176432446 25.063460303529894 81.77602759111103 53.7991083578613 52.780796176432446 25.063460303529894 81.77602759111103 53.7991083578613 43.90172759488548 16.859435752832887 81.66010286648884 45.30090915992505 49.43417234861445 28.965655408127024 65.19041442474659 50.572686229814344 54.066007541362445 37.600037670064346 72.34170032127993 55.092035025764616 45.78814885325278 28.19107633601881 64.02397644799984 48.63576695112775
7.5 51.8393247660887 24.248977023041398 81.30167246195583 52.879490681120544 51.8393247660887 24.248977023041398 81.30167246195583 52.879490681120544 43.95358888025321 17.31324875572536 80.9415188909538 45.28495633415389 48.47991995277983 28.667152189264577 64.99700491870011 49.641324386243454 53.56913286149653 37.21927281098497 72.11108262038103 54.606206223450904 45.461762754694774 27.057374880654265 64.07983240527801 48.10163740675619
8.0 53.268995841953156 24.9929881083243 80.67717720440329 54.260197931865264 53.268995841953156 24.9929881083243 80.67717720440329 54.260197931865264 45.86603140866258 19.070925048155736 80.18517402599213 47.161577825475845 50.42772057108923 30.049033849241003 65.10604631258727 51.528267140501846 53.20285971400771 36.88400256476624 71.9048040758315 54.246623323763664 46.91434034990952 29.073467505473904 63.996036431016755 49.37121344774978
8.5 54.1016512592941 29.055731139542484 79.93591591826525 55.1002131367715 54.1016512592941 29.055731139542484 79.93591591826525 55.1002131367715 45.90262359771663 18.873266092895786 79.36425421923106 47.2029413609656 50.10010738619361 29.92501984838659 64.72880702690651 51.216940636168815 53.63688387806525 36.93871739272582 71.52156036428691 54.67034164030971 47.94575508711819 29.23277564519713 64.00680401264687 50.1969936552084
9.0 54.034282390884705 28.234547601616445 79.31830255657937 55.01979857210502 54.034282390884705 28.234547601616445 79.31830255657937 55.01979857210502 47.69195523963866 21.498322739428495 78.50343658042495 48.89648605284378 50.05899453666235 30.693927571465252 64.62332166340057 51.18045645005414 53.52096470105129 36.07560142871985 71.09398862260427 54.55609141755928 47.83903810785303 28.905446324018808 64.18276637023055 50.02028837296615
9.5 52.82218583493082 28.461311231534697 78.46243207601009 53.83157442599058 52.82218583493082 28.461311231534697 78.46243207601009 53.83157442599058 47.1824058480223 20.741682301972958 77.82091316775058 48.39083495956581 49.92378549107796 29.345218979377513 64.60403057081099 51.049851099026945 53.33883420117321 35.543931973444224 71.01403152235784 54.37873991842548 47.00685595676759 27.680992223462514 63.894640701405855 49.09436929187644
10.0 55.50237445907202 40.32230571160351 77.74014757880482 56.50516404971583 55.50237445907202 40.32230571160351 77.74014757880482 56.50516404971583 49.291890636266295 22.60562080407534 77.05696085622452 50.41310326385439 50.22932998623252 29.096601654880583 64.4561202715965 51.33738078145572 53.51742251308532 36.52285616313121 70.61669581859785 54.5531956717703 48.68761722058134 28.862798368673214 64.0241935953189 50.625301217845


==> data/clustering/amazon_electronics_photo.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 38.92790694136933 6.769812568121028 97.49896880636888 40.41647161286537 38.92790694136933 6.769812568121028 97.49896880636888 40.41647161286537 32.09354595534025 6.000344036950459 97.11931012952488 33.74390334442442 39.103411613967346 10.987615383865297 91.79314867222394 40.394919577460875 38.18095639176505 10.24426566474137 91.96608602817697 39.49660217074662 29.515997668138755 19.04912592827198 78.47518799312606 42.690893263464744
1.2 39.65665374108558 7.384900930175356 96.53640014721032 41.10245590462299 39.65665374108558 7.384900930175356 96.53640014721032 41.10245590462299 32.61862473459786 7.019027113577048 96.19866442879774 34.22548827644673 41.91188618680969 16.033173570208774 87.8666687863324 43.092579624904324 41.89455638664714 15.742948271368176 88.34111735096573 43.06283576454077 31.23298488787353 22.174867587177566 77.51285534643057 43.5880445628088
1.3 39.72585113268982 8.606423799699439 95.38727568513725 41.135032752372695 39.72585113268982 8.606423799699439 95.38727568513725 41.135032752372695 32.73486257523652 7.676793387216217 94.88118251841907 34.330146756862895 44.60710161336972 21.141950287126992 84.87907133326566 45.69868007365393 45.071339949427895 21.66967119690249 85.66433171013192 46.13847086074759 33.33678238050112 23.413218105570568 76.92029048466436 44.816752505523596
1.4 41.707973361899406 12.830246283555748 94.4051000891004 43.065452094623986 41.707973361899406 12.830246283555748 94.4051000891004 43.065452094623986 33.149571198910365 7.9539914225971735 93.52558710212526 34.69334181942631 48.06022173338268 28.535346895713783 83.16221306510752 49.0831342015053 47.41645107361578 27.007054818443958 83.71713470627272 48.42577815880567 34.78991751484563 26.08234377718729 76.6843967585135 45.540129770107995
1.5 42.78599996855682 13.490027469776097 93.32286186144299 44.0733205629093 42.78599996855682 13.490027469776097 93.32286186144299 44.0733205629093 33.04120705649618 8.102241104652427 92.45394329196353 34.55412035692772 50.776928377500596 34.56296296752669 81.80497753509584 51.759376305464876 50.58196905036093 34.015194535019596 82.46215832603386 51.52965094249484 36.690231091465975 28.939705666109877 76.38267203823249 46.70382925697634
2.0 47.70329261878906 23.031311530100265 89.3623266410409 48.81294065939994 47.70329261878906 23.031311530100265 89.3623266410409 48.81294065939994 34.309177661819724 9.300567821948768 88.25894120834438 35.82418368928071 55.58523053851489 44.66652158148016 78.0781805632855 56.47920512835854 57.41419944103336 47.111994004640664 79.75295562910192 58.24443871335207 41.92926700851719 35.59323964733349 75.0005578848054 49.75666040979001
2.5 51.16293293036034 26.972035872859397 87.3840765185447 52.160417022916505 51.16293293036034 26.972035872859397 87.3840765185447 52.160417022916505 34.45123875928767 9.83802262214433 85.41004737668463 36.02935753694357 59.56399504445202 51.07217713738187 77.17561025048971 60.38898754871853 59.85929038819413 49.34126163957212 79.06569202091744 60.63827249180822 46.198156399032484 40.37112967134478 74.57723774148998 52.405717512439956
3.0 53.69781934287109 31.693731571295547 85.713315878521 54.61998082755572 53.69781934287109 31.693731571295547 85.713315878521 54.61998082755572 36.240295764806 15.540425104713057 83.98109978372193 38.12543107686075 59.622536884246394 49.94902624008994 76.15291983257201 60.46202411079029 61.3206613661758 51.37163740577243 78.59462147036362 62.073757649101566 49.718131246476496 43.91810897804351 74.37400280642454 54.71283174209055
3.5 55.10527412076801 31.398285857520815 85.11010154463816 55.99309216128046 55.10527412076801 31.398285857520815 85.11010154463816 55.99309216128046 37.28822295046735 19.251100984432785 84.14122141018274 39.15897080677978 60.07085837417768 50.42002749343809 75.42419094501398 60.87275156719093 60.548491464658724 48.450115391389026 77.19141158111744 61.33897439092917 52.50427853864693 45.98714583175543 74.41479241036288 56.628111844120454
4.0 57.94395075398231 40.672753489552434 84.45475093072291 58.79025061056541 57.94395075398231 40.672753489552434 84.45475093072291 58.79025061056541 38.96804847014882 22.03368088898249 84.749363949825 40.85336774899454 61.84791426123625 52.18701029833601 75.17867715420977 62.61771716882838 60.79291619785195 49.313251508383054 77.5166144365225 61.57649694853262 54.278681799952125 47.94859139048685 74.37163640026164 57.84192038906147
4.5 57.072458578140036 37.87194377298909 84.01588324916422 57.902393948872955 57.072458578140036 37.87194377298909 84.01588324916422 57.902393948872955 39.555220904993895 23.968049431648794 84.67856040922672 41.531869730018464 61.764370756468544 51.781318209197444 74.98110980871056 62.52685576116297 63.33329865284989 53.55085703418945 78.48585120818846 64.060085668231 55.11394897897761 47.3561454387234 74.12274302780763 58.20289324338077
5.0 59.18934404353866 42.8060691229717 83.83600518688411 59.9842136785372 59.18934404353866 42.8060691229717 83.83600518688411 59.9842136785372 40.71520762198916 20.93627111793129 84.36980992676291 42.44416799769016 62.30822195521982 53.21794892638418 75.00280199252789 63.048772191273336 63.09657968551058 53.27369613294446 78.00809492574118 63.82213539756737 56.77152780924744 50.02330275310698 74.0942256264557 59.4870258566864
5.5 58.53262687118528 42.944929743602614 83.48147054268779 59.33668690413072 58.53262687118528 42.944929743602614 83.48147054268779 59.33668690413072 42.185754942988495 24.461520292778165 84.0000811157014 43.93622322016412 63.078610904452404 54.963404372640426 74.99580043935325 63.80032501038565 64.32227641308619 54.692806506853344 78.43539983704426 65.01563220785636 58.06473496222054 50.80227034779766 74.14175563441535 60.43866989981904
6.0 59.886194305961936 44.05792565807028 83.64081862802524 60.66813381095892 59.886194305961936 44.05792565807028 83.64081862802524 60.66813381095892 44.860284810251905 29.276690786383984 83.86939364251029 46.5934065047686 63.21426893783661 54.72438011118912 74.87915963853993 63.929185971017155 64.57953827899775 55.47958263099374 78.32191731964593 65.26983299391472 59.18141111987176 51.93198119405699 74.00634091711417 61.29099850456531
6.5 60.20827348298802 45.55149095548442 83.61018828366771 60.98641519492002 60.20827348298802 45.55149095548442 83.61018828366771 60.98641519492002 45.8066699294359 31.20223232210204 84.17355410274074 47.24697677550405 63.437862951656165 54.807743127361384 74.73617301697054 64.1525126721382 64.87453979978334 55.76114443717597 78.27715891818478 65.55826020935719 59.47450834786011 51.64042388864478 73.84656498070723 61.42941787874412
7.0 62.4760580778592 50.54009236121221 83.30005497181446 63.209671683887414 62.4760580778592 50.54009236121221 83.30005497181446 63.209671683887414 47.15299095069898 30.810358367603392 84.52489189768319 48.48456261643548 64.07899673189522 55.55795992055229 74.5933788246196 64.77374297199202 64.49306381910577 55.12199140387942 78.02957841589064 65.18803218144404 59.64754641166756 51.42021174916444 73.79811403744796 61.46237189138169
7.5 62.9202046664869 52.219944048871156 83.05516164504408 63.651879252326204 62.9202046664869 52.219944048871156 83.05516164504408 63.651879252326204 50.09698527214754 33.66470831765503 84.59079966684368 51.23033382044548 63.56987353588145 54.56738515511882 74.3171619037448 64.28201980526718 64.83863170900976 55.561564777943865 77.95523642216251 65.52357485830265 61.02370981889981 52.88627338561439 73.87864155571884 62.633747129469974
8.0 62.15049890741089 49.40782432139763 82.79467443553538 62.89454047234743 62.15049890741089 49.40782432139763 82.79467443553538 62.89454047234743 51.079256481019755 35.447564503938516 84.84983652761409 52.27306671977371 63.76766464718173 54.75925481320147 74.36596651016953 64.46980403641994 65.15623416507442 56.25020639920674 77.89711185724721 65.83157252050826 61.087262666482566 53.04272156868516 73.81336206014193 62.59799501666791
8.5 64.6798453188741 55.54180172623414 82.63786120809715 65.37014806860323 64.6798453188741 55.54180172623414 82.63786120809715 65.37014806860323 53.35905440529049 37.555624184000884 84.91783390682383 54.512511238271365 64.36903297841482 55.55681644345369 74.25542082761172 65.06071590754604 64.86844921476053 54.77978900015442 77.54156275188325 65.54988131303594 62.77632057953153 54.08717417154578 73.92222244586345 64.17140464413886
9.0 63.674102664856235 52.904063905370016 82.41446032828625 64.39123145095803 63.674102664856235 52.904063905370016 82.41446032828625 64.39123145095803 54.82507188798794 39.89427697222744 84.73042519222854 55.93713059732117 64.06251539381904 55.422739864773405 74.21266770255993 64.75469218731745 65.1442910757718 56.40082861079553 77.61463135373901 65.82395887541692 62.53235267496847 54.35059680453552 73.86304793238227 63.83379161379309
9.5 64.91833649202384 56.28740577568037 82.33438628181226 65.60860087469888 64.91833649202384 56.28740577568037 82.33403634306707 65.60860087469888 51.95744838606026 36.14906243404697 83.75117852268717 53.05252042880706 64.01007305754192 54.76291210087958 73.8858348244781 64.70435983409446 65.77223660619777 56.995444758804915 77.5287618676941 66.43716707176831 62.44733647558751 53.754515294539914 73.62895727209141 63.65702738754372
10.0 65.46476779162973 56.37171842340629 82.13401131090109 66.14119919040071 65.46476779162973 56.37171842340629 82.13393806464715 66.14119919040071 54.90471613939334 39.30477324895909 83.60866307318852 56.06090409668389 64.51021987439893 55.56826433747436 74.06742571612288 65.1960822756166 65.31623781595928 55.957193260462276 77.38203186991768 65.99886069945289 62.966490850175326 54.86517005924676 73.90440293219514 64.10732518880981


==> data/clustering/arxiv.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 22.312462471000018 1.314432010652899 98.39978908590629 23.153719862216843 22.312462471000018 1.314432010652899 98.39978908590629 23.153719862216843 22.948335329117604 1.4663363321755603 99.0120293632874 23.956825020368015 26.781321181654633 6.678433335566614 92.89140083674073 27.376381139505597 25.817042759740232 4.620583160622784 93.24644200698297 26.3155390380921 20.491155787315737 13.792909076246712 76.28150040971711 40.5122675381069
1.2 24.21492655084347 2.376935899870524 96.19974064547095 24.88397252175992 24.21492655084347 2.376935899870524 96.19974064547095 24.88397252175992 24.10271701765575 2.2836081112664974 98.10441559070406 25.23529941414343 29.86760145973944 14.351316956371999 88.97415985193884 30.458990700031453 30.004692735926348 11.47098319277671 89.34314362414027 30.38402323363486 21.33898475153811 16.298786349112003 75.00583379643906 40.51378258874719
1.3 26.459698751569817 3.599226876754271 94.39209828379396 27.013544889575336 26.459698751569817 3.599226876754271 94.39209828379396 27.013544889575336 25.436100714827504 3.3092135675619394 97.07551730956393 26.592242775401065 31.77756835865346 19.687933366509228 86.34693327330372 32.40538448786653 32.570166792190335 17.724526684045415 86.61094677078239 32.90032745076329 22.232637322818675 18.926643983344327 74.31731159699267 40.61692895898227
1.4 28.271885962054466 5.328455559039018 92.78489647407582 28.747762086441682 28.271885962054466 5.328455559039018 92.78489647407582 28.747762086441682 26.29168685999125 4.114603646962496 95.82887060517159 27.445655486202586 33.2012542800052 22.437370000547848 84.29541602029317 33.830123561255164 34.35495820023042 23.060711097549124 84.64362692077388 34.68201199199895 22.686541831245993 17.832364280382983 73.84940771768781 40.37126090502648
1.5 29.826813009273696 6.6360045963456225 91.34767496096364 30.24293482111537 29.826813009273696 6.6360045963456225 91.34767496096364 30.24293482111537 26.72384136459961 5.888322917524878 94.88928093783964 27.899232939150558 33.933826867850584 22.198093742380593 82.61338296497195 34.54134041120845 35.805001704960496 25.779238066087302 83.18947779409436 36.110416917409445 23.372753720808824 18.00665061198032 73.79887219080985 40.34997577320324
2.0 35.095804600545826 14.068915392832288 86.59278731149105 35.33429495170169 35.095804600545826 14.068915392832288 86.59278731149105 35.33429495170169 28.91157507317733 7.174545819004196 90.64559662519028 30.20843732879472 35.85367896676627 25.620593202123388 77.55181685954618 36.43125705151393 38.30779963678818 29.511989952127283 78.7799060614476 38.56870714588653 26.578001450732902 18.25712082367006 73.41042778220839 40.2260985843237
2.5 37.47053973629501 17.803207371190368 83.43940986332517 37.69313552980095 37.47053973629501 17.803207371190368 83.43940986332517 37.69313552980095 30.577225066846314 8.262045412330025 87.41597584329647 31.800969780151306 36.824456297553894 24.65418524822774 75.78060717830081 37.26225482710134 39.29926708159044 29.903625395854867 76.667631812293 39.555101080791786 29.514115999359802 20.648207206294856 72.6798901822155 40.492799276069356
3.0 38.45309181911702 20.283043785798643 81.6748833651651 38.66424625794821 38.45309181911702 20.283043785798643 81.6748833651651 38.66424625794821 34.76723084924521 13.504725586577191 84.48462346628212 35.278915534817585 37.715626725277545 24.608765749830415 74.33912857948548 38.099375816798506 39.655253182403946 29.669204484434157 75.82618818884626 39.95358350642658 31.423228358518813 21.02921617711391 72.38256049213531 40.35616744435133
3.5 39.096362035651374 21.05774291183021 80.42461527389258 39.322652519589276 39.096362035651374 21.05774291183021 80.42461527389258 39.322652519589276 37.51216970411077 18.7398297650804 82.54329429164443 37.78629097023664 38.388241858709485 24.7078664824139 73.44118921430282 38.73560181990351 39.575887527842205 27.7779826684531 75.42652097510876 39.84799030718978 33.09850107317508 22.25419991983873 71.93610285615955 40.32552643818536
4.0 39.39076514076502 20.69130021155468 79.76967848267772 39.61197603376686 39.39076514076502 20.69130021155468 79.76967848267772 39.61197603376686 39.11334226922346 21.74384712605705 80.88807948145578 39.368637020959994 38.53089242226698 24.38787697338073 72.6509500373716 38.86365623472949 39.55992734603756 26.862439726197046 74.71900312113434 39.82206043520461 34.44112780894231 23.07664932009609 71.69986854075273 40.22627780559894
4.5 39.92487957236509 22.69905900994989 78.67267690499054 40.15390555587198 39.92487957236509 22.69905900994989 78.67267690499054 40.15390555587198 38.950825576048686 23.206306222951827 79.1417377526652 39.20584252191803 38.86430138249411 24.409045822202454 72.13168330832306 39.16291274659458 39.455723397337394 24.657832308454225 74.16263725525218 39.71686345926581 35.790238682974085 24.267299835844902 71.35534500476437 40.31616421052029
5.0 39.877373353322874 21.960411992506636 77.85218552360665 40.091819748062655 39.877373353322874 21.960411992506636 77.85218552360665 40.091819748062655 39.0558582132802 20.85212691778114 77.37929896371953 39.30431610374945 38.8488389044907 25.48604440290455 71.55175908090769 39.14913483978678 39.690576659525576 24.47563546684597 73.48843256113759 39.94598491275207 36.65871551031156 23.772839740467614 71.08411053952352 40.033694925532465
5.5 39.651673002221756 22.504435223178582 76.41543965312515 39.883196510761124 39.651673002221756 22.504435223178582 76.41543965312515 39.883196510761124 39.117119957936815 21.90652917405557 76.12248769865654 39.36650401380133 39.294665738889755 24.681034648245745 71.39507595569884 39.570033360862055 39.618316728599375 24.534912436086866 72.90960929034696 39.87341220837178 37.64527079528434 24.314273246566348 70.94647405125218 40.06146955480044
6.0 39.657894701829335 23.006592349164258 75.16821267811548 39.889759541283055 39.65764999346734 23.006562784736857 75.16829338497303 39.88951562114823 39.90791741414653 25.366014186505996 74.95584736276831 40.13609248710517 39.376584668398515 24.962846755226877 71.0181225514588 39.652154616405646 39.27701605387121 23.112818997577328 72.02524872310121 39.529563639214736 38.21338206945132 24.299669781016313 70.60177032561768 39.75380568712438
6.5 39.215556548303404 24.767070942339974 72.88745359095007 39.47478485539758 39.20853859636079 24.763878484858047 72.88725815742951 39.46779665096346 39.647350480687734 24.440416302375965 72.85305266094471 39.89560546322569 39.499165689071354 24.470044623416708 70.65639996782119 39.76277111821398 39.57032989416779 25.040056689669832 71.29681518328773 39.82393751735024 39.051399243643026 24.88251963861798 70.52217765705477 39.7941410291353


==> data/clustering/cifar10_100.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 4.286254932759247 0.27385856096268396 97.1257077576687 31.119962980730353 4.286254932759247 0.27385856096268396 97.1257077576687 31.119962980730353 4.342053088501014 0.24900722881062634 97.18381924941795 31.14403852726353 2.5613536005331303 0.13242641663482171 90.41554076874037 29.899000719733138 2.7279564760831163 0.15424272196250477 90.7075582109436 30.037565139420163 1.7708960051826785 0.2019887483654009 48.08307241264946 33.42777988018789
1.2 4.270637914795406 0.3192664851614105 95.41464558324296 31.18385854627982 4.270637914795406 0.3192664851614105 95.41464558324296 31.18385854627982 4.347991203718935 0.3147623000929542 95.20918261749054 31.25228672796109 2.6068044894704943 0.16343468783356646 83.967269835738 30.02753775481286 2.8891037787821094 0.21560574770034024 84.57123418721166 30.267685936699735 1.8523555370730436 0.2853846665663959 46.084086770601 33.463477676742606
1.3 4.307977587763469 0.4007243486325895 93.34422234183745 31.31560361131186 4.307977587763469 0.4007243486325895 93.34422234183745 31.31560361131186 4.400669183875407 0.38183871065137615 93.08398777738891 31.35309658567063 2.688292883886998 0.19144847022616335 78.46274575826072 30.154516351760957 2.969705541649222 0.2816666245651371 79.45564222534867 30.438503230719217 1.9185053288990173 0.4021138874258648 44.639819194836754 33.53782455592879
1.4 4.2430987592651785 0.5205409366210958 91.37305722588117 31.38630566483674 4.2430987592651785 0.5205409366210958 91.37305722588117 31.38630566483674 4.458284603615286 0.4701596142617974 91.13030643776744 31.45565966177721 2.6976073275613177 0.22479161291206357 73.76022715910861 30.23127836290958 3.1339156511684876 0.41434285282413474 75.23190578880433 30.680244342581958 1.9750735650718503 0.5080507342597753 43.34492159688942 33.58041368060834
1.5 4.223488242142637 0.6751956381847014 89.35619232664023 31.54983520677056 4.223488242142637 0.6751956381847014 89.35619232664023 31.54983520677056 4.481145984691988 0.5445999878232585 89.06853392882418 31.550026465058234 2.8157783525460287 0.2895538437251462 69.76647044430443 30.40359083298509 3.2669689869690663 0.699087062965192 72.00712708553787 30.969192460748786 2.057540337190009 0.6763387278971905 42.75021478241011 33.6657137725002
2.0 4.26218312133917 1.09291622779016 83.04483288218172 31.914244566546778 4.26218312133917 1.09291622779016 83.04483288218172 31.914244566546778 4.423551320757756 1.0207464212387811 80.35650249754968 31.787100589657243 3.1961702665102876 0.9930076803961663 56.29660192756019 31.126561078587443 3.7526224590137685 1.8122990135833967 62.3248996238076 31.925209635144913 2.3492434085871117 1.1633409556411831 39.88888753045571 33.80089619190701
2.5 4.285574722969209 1.4121809440891429 78.81224326222058 32.16401742872636 4.285574722969209 1.4121809440891429 78.81224326222058 32.16401742872636 4.423676925130138 1.2703391027346262 74.7633441686144 32.03108027934311 3.6471180701199106 2.387996996652703 50.447094167980744 31.965968952249064 3.98848944800827 3.06446991439223 58.64204428552051 32.51646214018747 2.5246991307954243 1.4914138141746875 37.622961838140434 33.85939758670988
3.0 4.303814431509741 1.7347344525288677 76.22818868507143 32.36368877044768 4.303814431509741 1.7347344525288677 76.22818868507143 32.36368877044768 4.384182546366333 1.4410353866623518 71.87968529884108 32.145103918936115 3.897764688502439 2.946441739984642 47.35945901354489 32.325198321235256 4.143315882085552 2.9552164341746656 57.191080492623605 32.68125424914824 2.6153852069827193 1.8433642648303141 36.469076150132786 33.921924555767774
3.5 4.243751053846851 1.850196025617565 74.52014912449651 32.45599873851387 4.243751053846851 1.850196025617565 74.52014912449651 32.45599873851387 4.33555597093097 1.4637173501203435 69.48835720819584 32.17193438556326 3.9566078844202255 3.2624718052105304 44.45949084968313 32.495577787532184 4.091682193502162 2.9518428443281506 55.33797873117167 32.71174638215987 2.716721950471361 2.0790362003169047 36.79862280564775 33.94742302759155
4.0 4.3159192425848465 2.1040612338280353 72.55241393044145 32.60664885821307 4.3159192425848465 2.1040612338280353 72.55241393044145 32.60664885821307 4.339858991658809 1.6060483204898022 68.12552906293125 32.33633354478683 4.036552694734513 3.5606397181859233 42.78290407679539 32.65675473029571 4.142703711934911 3.090386722049545 54.383460439109236 32.74485727061028 2.830127987949444 2.2413857724382305 36.226593539292985 33.95173292388696
4.5 4.4439055005321375 2.154066457207271 71.80428469459044 32.71469100467886 4.4439055005321375 2.154066457207271 71.80428469459044 32.71469100467886 4.2873844603234055 1.713362466080643 67.78010503874931 32.34101065326486 4.033387761819017 3.8544620118986064 41.088403061011334 32.7584889355992 4.146692362234646 3.5320733192611433 53.2157077968739 32.853265544050075 2.9098522400979077 2.3003019751604055 36.65277245352579 33.94813041902693
5.0 4.3415285665394965 2.1173774608937 70.7965492739141 32.685408459565814 4.3415285665394965 2.1173774608937 70.7965492739141 32.685408459565814 4.254518957459775 1.9443931154931224 65.4831693177439 32.45779188586773 4.080712048907621 3.780267469898351 40.274760002401834 32.82523528685291 4.13748576449857 4.026002969381694 52.2949154875364 32.94277357262134 2.949339137419448 2.5340986607341707 36.12320872150433 33.95876864856608
5.5 4.335878953258676 2.2701126660303808 70.10813787792738 32.712091577314304 4.335878953258676 2.2701126660303808 70.10813787792738 32.712091577314304 4.227280276831969 1.9102890683106604 65.35737468686163 32.46618669441234 4.059203545005048 3.9361463637054643 39.25453277626901 32.8601051596917 4.133663100342951 4.181038691656668 51.78078148781594 33.02689833062774 2.992274991107844 2.54231966450635 36.084328957013604 33.94483610199354
6.0 4.353252951434973 2.511810185101405 69.37862059904288 32.757052015633796 4.353252951434973 2.511810185101405 69.37862059904288 32.757052015633796 4.29955657797831 2.0188132763709294 64.79987523609087 32.54601331453134 4.192989631939876 3.998163822881251 39.884424803291566 32.97302841367068 4.206271111834015 4.27504839761289 51.59562255947897 33.051901138536344 3.0548168261501 2.623651710759505 36.01320788418562 33.94594111594191
6.5 4.3112549729974745 2.054398807601871 69.41862456758498 32.63959369842326 4.3112549729974745 2.054398807601871 69.41862456758498 32.63959369842326 4.32867476742786 1.9589156732505775 63.644776167774495 32.588359457286984 4.184513663042938 4.304805219775398 39.022799082700764 33.030682373178074 4.21407294745786 4.280625084037748 51.51181763544486 33.06775564828256 3.088489761115205 2.7332923918999423 35.76982449153691 33.93007609435146
7.0 4.200556837754347 2.147520230221085 68.5033481837458 32.67045724318854 4.200556837754347 2.147520230221085 68.5033481837458 32.67045724318854 4.234856456131371 2.0709647232288764 63.66590768052915 32.581482710610295 4.153646394199723 4.160635294026129 38.32773398324672 32.989853281397004 4.146591387605457 3.9243638484286176 51.769860042916584 32.98724520613761 3.1120731108658446 2.637654383617858 35.84123599676487 33.89065639280678
7.5 4.282025629064258 1.9483728180530377 68.24671979101605 32.63922622831617 4.282025629064258 1.9483728180530377 68.24671979101605 32.63922622831617 4.296777945665064 1.9637367676533033 62.781921969338306 32.589349041899595 4.205426299179227 4.1703156222556315 38.079632180631975 33.03268194211314 4.214202449654605 4.071255628877005 51.495050153278335 33.023779624884064 3.1399633578052595 2.75522201444517 35.40394504731659 33.89151877855834
8.0 4.35078720602136 2.1166703227412924 67.57690408912211 32.731382747462014 4.35078720602136 2.1166703227412924 67.57690408912211 32.731382747462014 4.316765843148995 2.008172135922379 62.28163287282922 32.64202515802569 4.214761398897819 4.149203211800605 38.13797758516938 33.04534675194855 4.233798259617652 3.7513447903981714 51.653367971112665 33.01793594892501 3.166588680581993 2.7928444425970245 35.336975707003994 33.88811541453245
8.5 4.28280310305652 1.9113240950018402 67.0905248220354 32.66670448153977 4.28280310305652 1.9113240950018402 67.0905248220354 32.66670448153977 4.028662426450381 1.9018224680436921 62.07716321992843 32.50454197950937 4.217789158082506 4.190435426558263 37.936768330245705 33.06496688320452 4.28097254003637 3.5437052139662786 51.44208467504961 32.96305568737204 3.1975225504815477 2.8100981360030994 35.16452094525335 33.86849129447743
9.0 4.099184605752406 2.215825802961118 66.61540900021365 32.630412731356415 4.099184605752406 2.215825802961118 66.61540900021365 32.630412731356415 4.287224511142872 2.286819387842266 61.740747787298 32.7489516745109 4.234446303194321 4.078026688347952 37.564294094590146 33.062993966597645 4.236657129606827 3.470438312310535 51.066194739997364 32.94881887602122 3.2058016146383777 2.94846552164711 35.068419136797395 33.87002461830869
9.5 4.02309865644334 2.2826054400121456 65.95213805466675 32.674734067252885 4.02309865644334 2.2826054400121456 65.95213805466675 32.674734067252885 4.233794575755341 2.1190532609257824 61.35589101539958 32.66395913406569 4.219276901082218 4.053041849492906 37.33870135380999 33.0661270625667 4.244353384559183 3.5897161536488356 51.04282364768598 32.96260707705644 3.2417292867801777 2.8608967518013646 35.024182961564215 33.84501543327788
10.0 4.068212208767739 2.057230924482282 66.12117726401559 32.650937283875834 4.068212208767739 2.057230924482282 66.12117726401559 32.650937283875834 4.138943369668146 2.0267969453903794 61.140552019472395 32.579914286968595 4.219474746094661 4.219119181139224 37.11015941087372 33.06269503507538 4.223567873879332 3.77626202862608 50.65584287813053 33.003706854270185 3.279652239925749 2.855310125187044 35.12385867482483 33.830725172783346


==> data/clustering/citeseer.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 22.534776470376634 3.6529094671282394 97.09645426850977 30.458857077409352 22.534776470376634 3.6529094671282394 97.09645426850977 30.458857077409352 21.696889452936556 3.8018358283324982 96.93035334991032 29.699498248765398 23.909334889776765 5.6728473880500925 94.94485595568935 31.761282658800866 23.704103300936595 5.197523235348511 95.02737095737469 31.539430620787645 21.216350130431266 5.3477820265031815 92.99539928381563 33.53380580885031
1.2 23.288472454839642 4.672755346318801 96.10327422145397 31.14029856555569 23.288472454839642 4.672755346318801 96.10327422145397 31.14029856555569 22.914432484362468 5.4345096084401945 95.95238321799377 30.846922417984413 24.102869415409636 6.989510912068439 93.35313451557161 31.98568097366784 24.228691741708527 6.590860597311754 93.44409731833979 32.07252685090115 21.901851192095563 6.303692287647392 92.1155999134956 33.46517076244846
1.3 23.821422146784123 5.017611657885337 94.8648668132338 31.63558967442913 23.821422146784123 5.017611657885337 94.8648668132338 31.63558967442913 22.944075092419684 5.358118132157603 94.32924459793594 30.89006164783038 24.414692574312006 7.780580841325826 92.29223285476316 32.323349516419434 24.798227632113576 7.611598018295681 92.10343046236864 32.624739443123055 22.619844030959253 6.67161754577238 91.29672281248412 33.36495045808925
1.4 24.19830883446456 5.530698452588494 93.1988191967997 31.981390962009705 24.19830883446456 5.530698452588494 93.1988191967997 31.981390962009705 23.42674242479596 5.952642521729587 93.43566714613922 31.372342884829653 24.99665758589429 8.776301057691901 91.37667511153602 32.88635095852919 24.97785236034001 8.029151502897786 91.22774903947699 32.81190451358817 23.52749110718314 7.859178353989307 90.82213785566428 33.53694464056412
1.5 24.370473662271536 7.044237035177302 91.70140722869581 32.21312113844138 24.370473662271536 7.044237035177302 91.70140722869581 32.21312113844138 24.483554883303555 7.262765083876651 92.10821410199358 32.438536778076745 25.03416759260909 8.566522944656423 90.49034069226305 32.92855703898089 25.002605543579136 8.931389297878107 90.41070387010981 32.88452722147389 24.037804037733554 7.993957802060287 90.08214065105817 33.32632025883021


==> data/clustering/cora.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 31.646901475213195 6.235871288152593 96.22406406015969 34.707528957361546 31.646901475213195 6.235871288152593 96.22406406015969 34.707528957361546 30.82814399072103 7.5852525822206935 96.05060515074817 33.8211649841348 34.160252734162086 10.192049082947104 92.19487765043735 37.01067411405768 34.023581039984506 9.726732866769618 92.17129920821355 36.86477309218128 29.593751988993144 11.268907606021305 88.30344743444647 39.03924952584295
1.2 33.70682772246051 7.326423751957842 94.36071130405278 36.70907360574126 33.70682772246051 7.326423751957842 94.36071130405278 36.70907360574126 31.55431780973061 7.63685637078277 95.62529505333744 34.65161016496321 35.66335159877568 13.061657668158979 89.74904986319174 38.36364344712078 35.457828421942715 12.309251974239615 89.59559561171805 38.170304950805836 31.31621355166442 12.566292431294512 87.18655502524427 39.700994883513694
1.3 33.74337577333236 8.590826570287664 92.1243724274888 36.64516278765771 33.74337577333236 8.590826570287664 92.1243724274888 36.64516278765771 33.95007293802807 10.039397890632888 93.84423628493505 36.94231631873538 36.36076908129194 14.124677397269089 87.80935645645172 39.014083229856034 36.24153213500185 13.917122149328224 87.59962249891606 38.883264167375444 33.54892820989704 15.165336097642387 86.1534858224866 40.61957452786199
1.4 34.99885298197037 10.239410205170326 90.55382688651943 37.785546396989794 34.99885298197037 10.239410205170326 90.55382688651943 37.785546396989794 33.878187895196646 10.385610150525675 91.92716910917034 36.76013257592597 38.508209691701154 16.756796489304257 86.32035444438428 41.04251482923992 37.843719420867515 16.150809726953426 86.11714621731495 40.39133586450902 34.37643928886843 15.593270681873722 85.2122264535034 40.531944321942504
1.5 37.924484305973714 12.575160969972293 88.86227531768454 40.504223178747516 37.924484305973714 12.575160969972293 88.86227531768454 40.504223178747516 34.76188112685911 10.894428497170553 89.60152002672841 37.56763259381709 39.62707961770393 18.583557878188955 85.09687068812373 42.12423242976695 38.70241418886261 16.98319593506959 84.99181259914727 41.22593840590801 36.32103012737618 17.234290973180983 84.34414491105645 41.69405988213145
2.0 40.63733491859646 20.054072190792485 81.91494823231355 43.10036181299943 40.63733491859646 20.054072190792485 81.91494823231355 43.10036181299943 40.63050298134579 18.731990922474555 81.60412177432698 43.075578459058335 42.30190113545671 23.853992622518867 81.47836680288393 44.7169030201689 41.96163972384272 23.70378551595656 81.3906937581667 44.373910864725254 41.91740097006733 23.021888849752212 81.46116695593717 44.45784990364117


==> data/clustering/cora_full.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 35.70752253780586 7.8263191387844575 98.31672479644153 41.47321982339929 35.70752253780586 7.8263191387844575 98.31672479644153 41.47321982339929 35.49270102096077 8.855137187753757 98.09811097146223 41.362962452622696 38.32081843171431 12.6809694841127 94.0966948742177 42.95566528945518 37.62354232760651 11.906821044293348 94.07223649435895 42.412182115524494 31.90784858684531 14.233234834136347 87.31199341654174 51.571869882056035
1.2 35.96654529854591 9.129383196330107 96.62821723303277 41.27984715334694 35.96654529854591 9.129383196330107 96.62821723303277 41.27984715334694 36.54152836989345 10.434551602813869 96.65328653347387 42.39129543666477 40.12779500590663 16.179193860537584 91.30364588357631 44.24197009438064 39.417046509764724 15.28037425584067 91.16580737873761 43.50549783558767 33.341263471154434 15.25037207726801 86.62479149577088 51.41135706033947
1.3 37.560247636872454 12.518499753151374 94.72804173900222 42.3906701365253 37.560247636872454 12.518499753151374 94.72804173900222 42.3906701365253 37.28784829899262 11.904209386049388 94.93713218269806 42.944398649030845 41.521164916075534 17.735797987442286 89.55636611234426 45.39655605636798 41.49945058908816 18.179723861058733 89.23856089671531 45.232502036470834 34.33405118067617 15.697650360866671 85.98359624033478 51.0878708322402
1.4 39.46778261363136 13.962690951354967 92.95059841880044 43.96330788170282 39.46778261363136 13.962690951354967 92.95059841880044 43.96330788170282 37.32436707700572 12.489627305099946 93.4194752993428 42.84763637023167 42.56686440201498 18.7949940165384 88.1639947429498 46.265575209278 42.20085711862044 19.051281067183517 87.74821241736126 45.74693959504773 35.230030617418414 16.33230667852901 85.37826943344534 50.72556144365158
1.5 40.38723632775053 16.992260926908582 91.5897861288313 44.46319294489844 40.38723632775053 16.992260926908582 91.5897861288313 44.46319294489844 38.07184469019177 13.83686911124575 91.883121813204 43.75140408295592 43.02829209240288 19.726092271966998 87.12353506439993 46.602646214397936 43.46279581080552 20.321491190790987 86.72551458075738 46.85140958207595 36.245172426041975 17.04717699909484 84.97719866807621 50.56902303112155
2.0 44.2533332723149 20.297039377856734 86.62211729378997 47.63500539321634 44.2533332723149 20.297039377856734 86.62211729378997 47.63500539321634 40.527665976492024 18.494222880944694 87.28827361361884 45.282883600209416 44.22726839054841 20.252521361292594 84.04561230317202 47.599230701208086 44.794439241507504 20.86288490127139 83.6403632422426 47.94148229448542 40.08783840713276 18.69747311799894 83.31740757487793 49.754760073778954
2.5 44.750320787292885 20.373700177965887 83.63509111014963 47.98358058557612 44.750320787292885 20.373700177965887 83.63509111014963 47.98358058557612 43.65519586879706 20.01584918358061 85.25968111960027 47.400515108681205 44.52487876608197 20.257685303962162 82.5384540974602 47.826155514650345 45.346053354275774 20.918583362056676 82.24990461510954 48.501198824216154 42.186665470039046 19.40354682676078 82.38117750834313 48.810290927729454
3.0 45.89455859807493 21.388035074885774 82.24210115843016 49.056825878736795 45.89455859807493 21.388035074885774 82.24210115843016 49.056825878736795 44.115629769454436 19.791151781436042 83.03645619907618 47.34559858877632 45.19530715313936 20.802246466365222 81.65564912223007 48.39147333837603 45.400999327655626 20.73152458427295 81.7407856683377 48.53826145304768 44.106521594189516 20.034866780054053 81.53388636964168 48.47039438154393


==> data/clustering/fashion_mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 25.921124370026494 5.151955534341178 88.52013845550873 40.33734643115013 25.921124370026494 5.151955534341178 88.52013845550873 40.33734643115013 25.424882682493717 5.436488154174173 88.46384744312982 39.935119618223155 27.47705564739258 16.39713739818289 86.99086583633273 42.54938918590586 27.487043803907085 16.205805458800285 87.06094607215388 42.572213900251505 16.528102460112173 13.062866913662951 85.09415462366563 39.61288274657308
1.2 26.057854739024393 5.623726301184447 88.80452835078894 40.521167464427506 26.057854739024393 5.623726301184447 88.80452835078894 40.521167464427506 25.58221522153622 5.662669883337766 88.78768540015956 40.0586299771201 28.480570002733508 21.338994793962254 86.8466927180241 43.6963477945897 28.66404527656443 22.152786963634956 86.7910647690309 43.98137737143818 16.93672433051003 13.607725221031682 85.09425120218147 39.76624707708228
1.3 26.349337210759654 6.159317384467391 89.0658521829841 40.793509461263135 26.349337210759654 6.159317384467391 89.0658521829841 40.793509461263135 25.6647639454898 6.002207564015981 89.05583885177862 40.14983867780109 28.86357404496992 23.539743783522134 86.79494358662657 44.14018245802941 28.991268387296444 24.59133013959891 86.7963027694066 44.405628174372026 17.24217733368658 14.382002910825076 85.01451216062199 39.916474623770995
1.4 26.35548623119278 7.11010285468422 89.29050267793285 40.903204979529704 26.35548623119278 7.11010285468422 89.29050267793285 40.903204979529704 25.595868662500664 6.085767355064524 89.28085240798124 40.12291790984149 28.94432201937432 24.551874921502787 86.74625769034895 44.28903186672158 28.59024716143388 25.661506043144154 86.55251830298558 44.24150896846477 17.570533234813208 14.909033210937281 84.89671268586486 40.03902734762228
1.5 26.308620463917055 6.944763032126954 89.46384685584053 40.878784843399494 26.308620463917055 6.944763032126954 89.46384685584053 40.878784843399494 25.4915234781491 6.104602531022076 89.43805032463456 40.04334448276664 28.992520448212726 25.03013542183698 86.66934908547394 44.3857366085981 28.34146837429765 25.241836924228473 86.28248131272996 44.11332853569692 17.822506954497687 15.316914088241179 84.83558450164705 40.12869169061446
2.0 26.716077019289123 9.385824736342618 90.11067236374559 41.45397206771481 26.716077019289123 9.385824736342618 90.11067236374559 41.45397206771481 25.609430272408268 6.167538743994875 89.54272339599957 40.172063417556934 29.039493240273124 25.878226589649945 86.11039019390245 44.51638912030917 28.709391095840665 26.924342421425436 86.07808175460644 44.483904387458146 19.030648060618567 16.85039635311367 84.22183404946233 40.6001940971501
2.5 26.81586307657219 9.953771007043665 90.15920231053497 41.65263752599378 26.81586307657219 9.953771007043665 90.15920231053497 41.65263752599378 25.620369532080854 6.5865633890026105 89.71424170710247 40.24502960561159 29.019041292264347 26.530546410158262 85.2563039672686 44.56599275794126 29.281218833179327 26.579815012377228 86.63926947529164 44.75420531748102 19.933380384593825 17.850640518427863 83.50664385976968 40.96723647913273
3.0 27.46190872816026 11.029394428885638 90.22175466504129 42.2896265150782 27.46190872816026 11.029394428885638 90.22175466504129 42.2896265150782 25.60902338977949 6.84951744831783 89.82547428048997 40.258920774388436 29.087720379024507 26.612915181961704 84.49725288101668 44.62064125706134 29.16249908266743 26.086473620905977 86.2891100758566 44.6878789501017 20.670841830041418 18.62848611236044 82.61750371197667 41.260034846284675
3.5 27.474060510968336 11.820543215442639 90.05648492930456 42.365746112528605 27.474060510968336 11.820543215442639 90.05648492930456 42.365746112528605 25.733327384002173 7.428875159642054 89.46083761568438 40.401752548275574 29.10756905672661 26.696383104523154 83.6115457499783 44.637152607807664 27.963656442559685 26.159166286527448 83.86937650962197 44.04126610665477 21.23616646038701 19.119886144710765 81.65870759871375 41.451657670246576
4.0 27.802995285456767 12.180817798727054 89.7950158276516 42.645236041410726 27.802995285456767 12.180817798727054 89.7950158276516 42.645236041410726 25.869435922037948 8.034609300376525 88.82761426401456 40.57123595706377 29.2647633873032 26.87242253517216 82.65630401728201 44.76356110048549 29.052670416572123 25.73992876394265 85.17006231233536 44.66296358808037 21.75629082248666 19.740070370450052 81.06666290668242 41.70931787288798
4.5 27.65690775297573 12.429161112258232 89.81749538870874 42.65226470892164 27.65690775297573 12.429161112258232 89.81749538870874 42.65226470892164 25.942048734699824 8.096998494251409 88.18297137507504 40.62905505189917 29.154445519696292 26.552712627258103 82.10582704953184 44.67007827649749 29.424535007482156 24.980708328212582 85.66147961731015 44.78263585933857 22.176590568548924 20.361515419772957 80.25787493377035 41.885993884839564
5.0 28.12583308931927 14.50139041274589 89.5869132904384 43.135115652155484 28.12583308931927 14.50139041274589 89.5869132904384 43.135115652155484 25.99482149352836 8.326690181928596 87.61751318669336 40.69470000099849 29.142740124992585 26.730834755693206 81.41516888701832 44.68258960683829 29.488027536724964 24.526145405888208 85.6631086559425 44.845401956409994 22.394452284188127 20.41172793403525 80.18628918527077 41.92385456014046
5.5 28.006817468481398 13.409349800260578 89.5770302544903 42.9891461168208 28.006817468481398 13.409349800260578 89.5770302544903 42.9891461168208 25.92727040782485 8.49980843245416 86.97443326827636 40.674708568034674 29.19809695223938 26.623300598115872 81.08201629092335 44.698619697322634 29.307431713548958 23.028322291185138 85.33672110238912 44.61586006125411 22.72038418924979 20.815899366239606 79.63299929095562 42.04699697444701
6.0 28.598325838700983 14.774158235397273 89.47265986469208 43.528172333730396 28.598325838700983 14.774158235397273 89.47265986469208 43.528172333730396 26.03326176847185 8.728883608622748 86.35126662228829 40.772660969158025 29.145199557365665 26.248689427254224 80.4645437570211 44.64198597535627 29.340939296963718 22.81191474514673 85.18078476842041 44.6695469726835 22.975831056649238 20.891024524137883 79.14165790342584 42.13052830472792
6.5 28.543078617623095 15.921495077691251 89.13155612923602 43.60906451513552 28.543078617623095 15.921495077691251 89.13155612923602 43.60906451513552 25.978001263694463 8.740080076758193 85.68119586393873 40.7398269041405 29.076483516208775 26.247234617698656 80.14384333289483 44.61654695481075 29.432519996597694 22.638915543030347 85.00472074587199 44.7127900683968 23.285492093001697 21.072359209230193 78.99171869498309 42.247320969272074
7.0 28.850122221341056 16.351997792261933 89.08224791684913 43.86650820000024 28.850122221341056 16.351997792261933 89.08224791684913 43.86650820000024 26.098783516165554 8.976317583046011 84.98230671843035 40.84560508270926 29.107364987014133 25.804967810496436 79.84995685536049 44.58803415989198 29.432257699502664 22.73593480391006 84.71563430801777 44.70938923535452 23.57556184043622 21.605520369561937 78.12056473117094 42.41690387322724
7.5 29.071940933875993 17.260731697018066 88.92686642217647 44.08357085569346 29.071940933875993 17.260731697018066 88.92686642217647 44.08357085569346 26.16930074500442 9.822967169397613 84.13762159033254 40.96133312407305 29.216972966524608 26.558840799721178 78.97257817874758 44.74838551972978 29.460961505846818 22.435085371430183 84.62701448882535 44.73277464937199 23.680084478314594 21.6810821224194 78.33183055543633 42.44268396423491
8.0 29.013724956062433 18.07014706414647 88.79307027050793 44.05056685566057 29.013724956062433 18.07014706414647 88.79307027050793 44.05056685566057 26.185616594381944 9.979845201901952 83.19783027943232 40.99462440116716 29.05706421480776 26.08154531759891 78.68927659692855 44.598892289066185 29.471613393741997 22.753742964802814 84.43930821043759 44.75441729896891 23.988862256298912 22.438605248257677 77.30827503769137 42.61848249404892
8.5 29.30817894534107 19.21291171112027 88.66226501945246 44.367564398644205 29.30817894534107 19.21291171112027 88.66226501945246 44.367564398644205 26.17816706773223 10.05931504119512 82.12325731532022 40.97805519171274 29.08045510885572 25.419139816238502 78.82752655836246 44.59090463690528 29.48919668599786 22.217382028093482 84.22024491983541 44.745454259888554 24.055225750901926 21.3135356052694 77.42041147522013 42.54174952373418
9.0 29.321857978006445 19.460905091274384 88.44677848969845 44.361761769994814 29.321857978006445 19.460905091274384 88.44677848969845 44.361761769994814 26.336384609514667 10.235724407588513 81.05338483376185 41.13179250413357 29.147906211058345 26.429122985943426 78.11399410790602 44.677147464828806 29.431253656792816 22.010029707891704 84.10729809990161 44.69174960741981 24.26752790348888 21.764519309067992 77.28888455892789 42.651511458853236
9.5 29.41863048481142 20.30046054622096 88.25736880351049 44.52755934631412 29.41863048481142 20.30046054622096 88.25736880351049 44.52755934631412 26.33201838233181 10.243064068668293 80.00834891220245 41.128799238711366 29.17228197513097 26.105439670320358 78.15545902088203 44.679715993902775 29.440644704588014 22.18187265918025 83.95629482564294 44.697693687803735 24.34678760075522 21.76669829815622 77.34097526725267 42.68363740957876
10.0 29.55539969357289 20.886125509939696 88.30747313568776 44.650062638731214 29.55539969357289 20.886125509939696 88.30747313568776 44.650062638731214 26.427172613670713 10.963950875930866 78.97228957272809 41.24301546314947 29.266435665445066 25.65825196930243 77.85621000684716 44.75024371830969 29.55585398609251 22.164786042865853 83.76078874132978 44.78724100749997 24.695269537855392 22.467031579400857 77.30454697628133 42.8871326265881


==> data/clustering/mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 41.25523742592835 6.859634732057683 98.03530936419985 46.86054154729469 41.25523742592835 6.859634732057683 98.03530936419985 46.86054154729469 41.25289381256689 6.47365435075506 98.43940223901264 46.84022186481822 45.233919073927105 17.324716915757904 94.7432442256398 50.66160107813328 47.735866924279854 18.41948232435404 93.78723730502554 53.09794207480335 17.401488484989002 17.427356525388575 72.01803598518526 40.90019585382947
1.2 43.49527254873525 10.451525871237463 96.64613921726811 49.014329269044346 43.49527254873525 10.451525871237463 96.64613921726811 49.014329269044346 41.969104050052984 7.910498249303241 97.71651576182036 47.549774220929564 47.649560458622645 25.386752858349652 92.52462168699454 53.043186725970806 53.580711257926716 37.537788369865616 91.56883576544035 58.76155651401411 18.166956733836244 18.970929939752885 72.03346733099046 41.260685263120045
1.3 45.40033410255567 13.560654326147997 95.582380829354 50.841308517915415 45.40033410255567 13.560654326147997 95.582380829354 50.841308517915415 42.252445472733086 9.978117466628335 96.73587774374481 47.90137182877083 50.02461299259061 35.981631022856 89.96221811288572 55.3599359207279 56.13017699054061 44.63671158597247 90.58189911433313 61.15843489063645 18.808780522615002 18.811657587689506 73.10787929800888 41.50054006193179
1.4 46.410961798041214 17.060207881546738 94.81729812636065 51.84790992378454 46.410961798041214 17.060207881546738 94.81729812636065 51.84790992378454 42.92647369944012 11.109285655093679 96.06274424274993 48.54884463809441 51.14569999994978 38.548990506695304 89.00801037604161 56.461031843036416 58.02292892222945 52.99650562461067 89.62210916072536 62.943022193880616 19.536634443512117 19.197913014793816 73.77758643763195 41.82212288428535
1.5 47.54498457452375 19.871650199176287 93.95824677967484 52.93524033994499 47.54498457452375 19.871650199176287 93.95824677967484 52.93524033994499 43.40546713495142 12.475048713997946 95.24014786499745 49.01317093216779 52.643756764778196 42.27735825057309 88.23027082227674 57.88941865980664 59.287389880168305 58.42087948138166 89.11904736492446 64.12892811344217 20.148914698964575 20.446974393026043 73.48703695830292 42.108706838171216
2.0 50.574662481021825 27.41104744173902 91.54932056893982 55.87861606213041 50.574662481021825 27.41104744173902 91.54932056893982 55.87861606213041 45.190940016718855 18.303687824086683 91.71524120368548 50.80764554209141 56.946634535537385 57.09920796500136 81.90583369133988 62.03452448072759 61.7822362822086 66.99493085992934 87.76727580520276 66.4769446446743 22.740155595942408 24.320418382643382 72.71585899492418 43.28005496240278
2.5 52.72189014966916 34.35593163046944 90.33896264022502 57.94511656316794 52.72189014966916 34.35593163046944 90.33896264022502 57.94511656316794 46.611042995493136 22.857199796889617 88.82386159587085 52.20758260183367 57.7461894858877 57.19913172142803 82.28843412714536 62.82231081843871 62.91083835435087 67.94099044170765 87.99500810676633 67.46520117946406 24.92614438433686 26.241126835128405 73.39607620239535 44.27755861879463
3.0 54.00000199794414 39.40958229694861 89.48128017663916 59.18701297537255 54.00000199794414 39.40958229694861 89.48128017663916 59.18701297537255 47.03720300864628 24.40173453837501 87.09675454913179 52.63223167943476 58.29761090374237 58.443745236869816 80.57300587670126 63.3532212214176 63.05268823676812 68.74177904156372 87.38611541867301 67.63508574279325 26.5633145616414 28.36185618797516 73.22390052450294 45.013125651381195
3.5 54.56119533998658 38.88920271519224 89.17334101044206 59.651956217773005 54.56119533998658 38.88920271519224 89.17334101044206 59.651956217773005 47.702060010382205 27.45296455385981 85.30625554642978 53.305463955667975 57.87341368526639 57.774655234487994 79.45447085706223 63.05359554410976 62.587860629777126 68.03585900824471 86.4358016353761 67.27852031546699 28.281029689972204 30.422399373192388 73.30361820874964 45.888016762862165
4.0 55.95290649679434 42.792398070245625 88.67821689482203 60.948561974012314 55.95290649679434 42.792398070245625 88.67821689482203 60.948561974012314 47.587578806443545 25.522888730430658 83.76032017738746 53.17663496609269 58.521072787726524 59.276847745475614 78.29141354143702 63.66293997021306 63.77342707409126 70.61530547466172 87.28529364475904 68.27333595070387 29.82406191484688 32.70719241495581 73.32111442181673 46.70289477205031
4.5 55.905611992309034 43.22239589760662 88.21143452763452 60.92347029869074 55.905611992309034 43.22239589760662 88.21143452763452 60.92347029869074 48.75765618636511 32.575326408548065 81.93757033352529 54.33773489028522 58.90841647532488 60.30319713454028 77.97161107749709 64.01128870516175 64.25701234574964 70.71814090561888 87.4975334512139 68.6823787948411 31.245196045715907 34.49879730122648 73.14595527335062 47.4651314729887
5.0 57.055096812044745 48.84496611867505 87.97049104317264 62.00732434958178 57.055096812044745 48.84496611867505 87.97049104317264 62.00732434958178 49.27570803265889 35.61742728590206 81.21361981118291 54.851199035357226 58.85863792665255 60.27717932937168 77.61655562008245 64.01468555301005 64.34961830203736 70.39266367769005 87.52127205781785 68.75431264483865 32.09162977168273 35.88083877061511 73.11286960197376 47.8794344661766
5.5 57.49307119546528 49.95730177447619 87.7472618905504 62.41821629504653 57.49307119546528 49.95730177447619 87.7472618905504 62.41821629504653 50.44848946502306 37.64365008147285 79.88382019098941 55.920052045979254 58.63525783767383 59.830544589542626 76.85480409164967 63.85919072001951 64.23805447193585 69.9284211599487 87.46427076726395 68.65030690702582 33.21842976648432 37.07294004166945 72.8241885822903 48.482458915979656
6.0 57.79223609723765 52.14304723316258 87.57535903371448 62.71836951229599 57.79223609723765 52.14304723316258 87.57535903371448 62.71836951229599 51.053087368582005 41.090873436257986 79.58760887803209 56.52387982467246 59.35787126905373 61.16013933463814 76.69158864382055 64.46325051003377 64.39273138100853 70.45218649567757 87.32543622377437 68.79409957279287 34.23667567892824 38.19728773701094 72.94161096530893 49.02723532241346
6.5 58.7066240705793 53.760784680096016 87.5265965875213 63.54749376422003 58.7066240705793 53.760784680096016 87.5265965875213 63.54749376422003 51.610986761380815 42.66498439897141 78.9121069856548 57.040435094956536 58.78760046705654 59.868845625847534 76.32845449340817 63.996121262886085 64.30723218406786 69.86036971602978 87.25283702370255 68.7073872544904 34.7963087142675 38.88430306440751 72.94258731418675 49.27594498480098
7.0 59.275955135564274 56.924432912548816 87.08751527667535 64.08099938500548 59.275955135564274 56.924432912548816 87.08751527667535 64.08099938500548 52.14111406930926 43.68063350870336 78.31034883805576 57.53571553103474 59.22660754574215 60.742301829195085 75.8737035274213 64.36041736561207 64.1920377572311 69.80402931587363 87.05200755892953 68.61171817518246 36.161448587261106 40.60771345599814 72.63778368516594 50.113297817076784
7.5 59.676943447546485 57.30316733583818 86.85474789323774 64.45768492688096 59.676943447546485 57.30316733583818 86.85474789323774 64.45768492688096 52.437992819118165 44.539418824304825 77.98271807140435 57.825681820852814 59.473892899928614 61.27457752991944 75.71116181589794 64.59088337614475 64.38256420627677 70.22725579098312 86.92306295001794 68.77978705487877 36.98082855446352 41.215728136457884 72.98076343963592 50.5503867531035
8.0 59.46310515705474 54.10491307330456 86.89118248428815 64.22986107002782 59.46310515705474 54.10491307330456 86.89118248428815 64.22986107002782 52.95762094363672 45.936930338853784 77.85427162580142 58.3121582475831 60.17316327082044 62.300771495554955 75.67882074188272 65.17907673340856 64.14019578256429 69.45249610194904 86.85143636511216 68.55769114616324 37.88263758668595 42.03867285463053 72.96422268853382 51.066428947396304
8.5 59.818727596697904 55.459000210110766 86.65906761210177 64.55732337135186 59.818727596697904 55.459000210110766 86.65906761210177 64.55732337135186 53.729492010635646 48.38863238514054 77.61660865433714 59.032108428394345 59.88860972375177 61.80682161197624 75.56846213465582 64.94095960026154 64.40724117488593 70.42363374795578 86.7034826269863 68.80687621812714 38.65913086262126 43.15361498277529 72.96379595249155 51.53783290476417
9.0 59.646031719359726 54.7664983709069 86.39167224037594 64.41297341823085 59.646031719359726 54.7664983709069 86.39167224037594 64.41297341823085 53.86300641833106 48.66003582333456 77.50345447286652 59.16044870711221 59.73837100078854 61.672752643478255 75.10144089978414 64.83087316110243 64.5830525989412 71.04418785655892 86.53978192573055 68.96917527219077 39.08143675447101 43.123265421896306 72.93513007156221 51.71420847830832
9.5 60.10440583946928 55.43246245239006 86.31043913485364 64.8182582995896 60.10440583946928 55.43246245239006 86.31043913485364 64.8182582995896 54.435616503061226 49.81638587112147 77.2319873060637 59.68939505575992 60.57862563595147 63.198413933758246 75.04974267556858 65.52612650756593 64.53657202935449 70.90596658509695 86.44555774751609 68.92889962439419 39.98856448706544 44.43168037985048 72.87916900089981 52.29959649913333
10.0 60.81236497629645 59.27974385641569 85.8751219280357 65.50611468664125 60.81236497629645 59.27974385641569 85.8751219280357 65.50611468664125 54.93570167792027 50.86363256158559 77.5367314233678 60.15522853687456 60.232587819018704 62.326407495205395 74.82875961956917 65.241602693984 64.53949332264666 70.74162643453177 86.38506619093734 68.92908867484098 40.65004092704778 45.25447897118541 72.80957159729698 52.6943778208705


==> data/clustering/ms_academic_phy.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 16.67763179571647 0.7684567301791867 98.47465794561975 16.965273681386012 16.67763179571647 0.7684567301791867 98.47465794561975 16.965273681386012 17.31917327896196 1.0674427304490808 97.8161950374272 17.61889909950529 18.97738171887085 1.6367372863392828 92.17823395269005 19.184281626790877 18.443164246166287 1.40398827668532 92.46439188310696 18.653966226560666 17.35161668589886 5.457397615727584 78.44073027662691 26.632550506704984
1.2 18.45088736963702 1.0905148987833557 96.37400986946012 18.7163127020826 18.45088736963702 1.0905148987833557 96.37400986946012 18.7163127020826 18.59799302215513 1.5318074571357079 95.81779747569217 18.94036330618483 21.14483681716186 2.991368693819843 87.37327271966416 21.311571933630653 20.43960387803983 2.2745993436343013 87.81111180705416 20.606384159741555 18.62938664910437 6.677260255508069 77.0311288260403 27.275913917194668
1.3 18.748206696208964 1.2622332294371843 94.18742188998289 19.01183771718719 18.748206696208964 1.2622332294371843 94.18742188998289 19.01183771718719 19.43712742533647 1.8610743662557994 94.13433644732268 19.787898948880613 23.832438084169038 5.755374695997642 84.04403327750329 23.98080958605117 23.0832476180578 3.29608509149871 84.35763906268775 23.22466453485573 19.433901601580956 7.881855148677368 75.89376680322667 27.586473605404265
1.4 20.656989219880167 1.6464670472217315 92.17382585479517 20.88314791791231 20.656989219880167 1.6464670472217315 92.17382585479517 20.88314791791231 20.332615105330326 2.097538381880424 92.69504850093547 20.706177608548277 26.741125307794743 8.01210863590183 81.72484506463998 26.865565026355192 25.613433859501818 4.8921297515209705 81.75436215098081 25.734471899459816 21.18019725017924 9.022273900103448 75.34572776404204 28.756283388678927
1.5 20.962654179757703 2.330778336178455 90.39130397898937 21.165283937083807 20.962654179757703 2.330778336178455 90.39130397898937 21.165283937083807 20.716798899801255 2.1942169865731356 91.43332284987096 21.090279100242608 28.09051012165066 9.968918342674744 79.76125760719685 28.214976672372728 27.693921289391977 6.385166059277026 79.68790925994274 27.79772479620996 22.31624366427354 10.016538581744392 74.53900247664288 29.372043389953106
2.0 26.312990646540346 4.258149869401131 84.03303403723697 26.449067938269323 26.312990646540346 4.258149869401131 84.03303403723697 26.449067938269323 25.52114575887873 3.885395979236929 86.92705759033015 25.95789618123085 35.19241387392179 16.088539869770667 74.57972688820028 35.28851299021599 36.16479460930703 15.082042060529243 74.60776170919993 36.22436138774536 27.194739971596064 12.375393519876985 71.69467756981847 32.232965384673186
2.5 31.754516732182868 7.6867059906156525 80.15825164798567 31.84667649949252 31.754516732182868 7.6867059906156525 80.15825164798567 31.84667649949252 28.45521106687633 5.834998518452558 84.10380513207164 28.883291030050888 38.760134758894594 18.53694840569459 72.02185201433976 38.841832423963915 40.52022379064376 18.767940362070835 73.04674392878859 40.57036566816148 31.48333527804832 14.563339760780883 70.1146547176822 35.0672234683537
3.0 35.46067941668333 9.859719675726042 77.32734007757102 35.52972511992935 35.46067941668333 9.859719675726042 77.32734007757102 35.52972511992935 31.317094965927662 8.95440440473386 81.65039983479245 31.614295743395047 40.48309448670082 19.34050459948324 70.31533515394537 40.54906207656739 41.718572284085134 20.849842742356234 71.66018278302106 41.76330117288949 34.42145772902047 16.54985543129113 68.79457281333225 37.01696890211409
3.5 38.90825582464793 13.863781028115655 75.25239815824196 38.96384350848549 38.90825582464793 13.863781028115655 75.25239815824196 38.96384350848549 34.278318624901964 11.94324176533286 79.24748849930407 34.45671172490034 41.6268450584482 20.062679857376924 69.17889681297946 41.68754379448938 43.00960442911222 20.83251157853454 70.8974723432894 43.05189926850312 37.30302148582657 17.955207022735703 68.75003875709382 39.177195182760215
4.0 39.46064894976266 14.339160982602706 74.07521528506376 39.50677213906681 39.46064894976266 14.339160982602706 74.07521528506376 39.50677213906681 37.57283544750037 14.519802850918936 77.57065241474848 37.70275474230182 42.841801276435625 20.55385297633622 68.67914527017422 42.895928542594795 44.6825934955638 22.735013577310323 70.66764737662734 44.726148307985696 39.65703151290628 19.54864672726794 67.82909162424227 41.02216834046716
4.5 41.01188367551393 15.255838026907176 72.69428281142592 41.0557402514396 41.01188367551393 15.255838026907176 72.69428281142592 41.0557402514396 39.427557579641224 16.335614309666454 75.72443691052848 39.51577876286899 43.281233998119795 20.757904368156115 67.99405148102433 43.331411191614436 44.93983387737469 23.281463329586867 69.91568868700699 44.981974657169886 40.66242051262854 19.140395205622035 67.51147729548052 41.63932935819996
5.0 43.38607880780402 19.446846670091517 71.57530715577923 43.42864531965168 43.38607880780402 19.446846670091517 71.57530715577923 43.42864531965168 40.68315669182043 17.113261761935135 73.84436405247932 40.746210039498074 44.15505663416493 22.0510028700528 67.68875791230624 44.20223901044819 45.6728430368289 23.65753026732842 69.58527078354143 45.7123936786276 42.16170658225813 20.444445715441855 67.24902712245166 42.831405405058696
5.5 44.34463415540214 20.404230126881544 70.1241191517643 44.38215237282634 44.34463415540214 20.404230126881544 70.1241191517643 44.38215237282634 43.429489793908395 19.08742524127514 71.78945061189737 43.474830337680956 44.85836377079447 21.683426339046775 67.31319584549368 44.90036276694539 45.616475788847474 23.457523652384783 68.94206015974895 45.65546683765375 42.76926540224313 20.72737510603174 67.15631710947923 43.241042719099305
6.0 44.96300114460773 21.788407228346905 69.07440512168324 45.00297503138751 44.96300114460773 21.788407228346905 69.07440512168324 45.00297503138751 42.73543965462046 17.791224465571727 69.49301907348982 42.77399890567924 44.758867533645564 22.173916094869835 67.11876927402338 44.80268125761365 45.77539278546831 22.853033140424422 68.28071517079064 45.812625150509554 43.88729363227834 21.968694415960677 66.67347762566081 44.19500922583449
6.5 45.98552619369869 22.64601245584576 68.0261541224094 46.0238637345968 45.98552619369869 22.64601245584576 68.0261541224094 46.0238637345968 44.25742834173054 20.639451316840805 67.9577572319641 44.29567693540667 44.976945537960916 21.86467979197879 66.87086940678957 45.018247657664965 45.54865695637454 22.4823576885975 67.57325227518335 45.58644677449945 44.61188549444768 21.62274578129039 66.89901721588222 44.79002184291815
7.0 44.30688345489574 20.081149200825315 66.65594584964566 44.34444064690249 44.30688345489574 20.081149200825315 66.65594584964566 44.34444064690249 46.1841158904544 22.46929990580278 67.08834948305473 46.221011750849705 44.721363218759215 20.735590812338618 66.64621098462115 44.7607424763501 45.33541511738395 21.484501479196798 66.99110217000238 45.374217353781724 44.6386233595588 21.153965972267173 66.6567494922157 44.70877133535554


==> data/clustering/pubmed.tex <==
degree mst-plus-best-filter-edge-modularity_ami mst-plus-best-filter-edge-modularity_ari mst-plus-best-filter-edge-modularity_modularity mst-plus-best-filter-edge-modularity_nmi mst-plus-best-filter-edge-significance_ami mst-plus-best-filter-edge-significance_ari mst-plus-best-filter-edge-significance_modularity mst-plus-best-filter-edge-significance_nmi mst-plus-best-filter-spectral-radius_ami mst-plus-best-filter-spectral-radius_ari mst-plus-best-filter-spectral-radius_modularity mst-plus-best-filter-spectral-radius_nmi random-plus-tree_ami random-plus-tree_ari random-plus-tree_modularity random-plus-tree_nmi random-tree_ami random-tree_ari random-tree_modularity random-tree_nmi random_ami random_ari random_modularity random_nmi
1.1 12.034015595574427 1.147173017250867 94.4057869978873 12.219187695173446 12.034015595574427 1.147173017250867 94.4057869978873 12.219187695173446 11.751900297577981 1.0927173324803734 95.69374806024774 11.972118437764507 13.431349124020114 2.1635023325369893 92.64639296943636 13.593508443498193 12.865124462512373 1.5864661933971447 92.42348055744041 13.02905172081614 9.713768574774907 3.8812601116168826 81.74102527183386 18.487255610044798
1.2 13.639721253800028 1.6612326171963927 90.52476493205731 13.785858371362709 13.639721253800028 1.6612326171963927 90.52476493205731 13.785858371362709 12.288526726462393 1.4033414770586317 92.87513594247615 12.498016308128319 15.238580033548338 3.905732932527338 89.04537163207425 15.371005551280264 14.899200940321384 3.244215287458893 88.50387018047302 15.0215014537929 10.441347282468804 4.301007775732118 80.8938103211245 18.50429925385379
1.3 14.541538002244076 2.5525977264414705 87.18862331909747 14.665608631025167 14.541538002244076 2.5525977264414705 87.18862331909747 14.665608631025167 13.54344059958939 1.8150237738152675 89.86412513201834 13.751730513674291 16.044262693767568 4.98121255075917 86.66503520404912 16.163197839647264 15.938410392722282 4.432248328419472 85.83946495971358 16.039055229419752 11.209063195418498 4.967115553765436 80.46529664080839 18.5771909528953
1.4 16.16093429434184 3.5264331777495146 84.96856639976778 16.252104725411385 16.16093429434184 3.5264331777495146 84.96856639976778 16.252104725411385 13.743614604167245 2.6293495065266255 87.33219209855955 13.923690165972639 16.821436090893886 6.010432188221264 84.66613345581878 16.929259307582992 17.04747334635944 5.447689247747854 83.70195805428034 17.13554722155642 12.140082990064045 5.447472481433726 79.61904096466729 18.79891574433795
1.5 16.29139079169006 4.700848796034103 82.92910609515329 16.374767935288705 16.29139079169006 4.700848796034103 82.92910609515329 16.374767935288705 14.105679903676899 2.741259600137503 84.81569567177732 14.276015083040633 17.328988016121738 6.6127333348830755 83.11100784357718 17.429523700143463 17.71930172723744 6.460527382412015 82.22656670827708 17.798692700775113 13.091734116900202 6.137265910292831 79.27847440315712 19.021702171780415
2.0 19.848885702608225 9.247594243514708 78.70594305013654 19.927501362234487 19.848885702608225 9.247594243514708 78.70594305013654 19.927501362234487 19.189805847931567 8.95217456848745 78.08111396049196 19.276810818511265 19.67806035800263 9.76701998153262 78.19090613684368 19.760281198170468 19.284628388252912 9.635183890177425 77.76282920788711 19.35725456351652 17.517401172140325 9.28714981022463 77.59950167492636 19.678840745314023


==> data/deepwalk/amazon_electronics_computers.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 36.85502617403839 36.89893786510887 38.358220165389575 42.84630908125332 42.14593733404142 38.41564372961081
1.2 41.48795994234125 41.91744935892573 38.60426371292011 49.34513314619528 50.290668386313634 40.93750853501252
1.3 46.7625900917988 46.79757984978378 38.50276913739473 53.67622335179425 55.24955617934907 42.69965859949928
1.4 50.099992413322205 50.28700402093923 38.82219861922464 55.97354525453304 58.71497610196496 44.60723010393749
1.5 53.74756088308929 53.846073894241705 39.26117896972915 58.74203019497762 61.16651240421819 46.620999924133216
2.0 63.400273120400584 63.68135953266064 43.576587512328345 65.28292997496396 69.30824671876185 54.074706016235496
2.5 66.80282224413929 67.46667931112965 46.868803580911916 69.21634929064562 73.03314619528109 59.336787800622105
3.0 69.72230483271376 69.38233821409605 49.97675441923982 71.35597450876261 75.16583718989455 63.183817616265834
3.5 70.78880965025417 70.87746756695243 52.383096881875424 72.86070859570593 76.5624535315985 66.14885820499204
4.0 71.8638115469236 72.20883089295197 54.211000682801 74.04662772172067 77.55097488809649 68.03107503224338
4.5 73.3234655944162 72.99915787876489 55.292200895227985 75.06048099537213 78.28013049085804 69.69463621879979
5.0 74.06247629163191 74.1800546240801 56.813284272816944 75.69711706243835 78.83997420529549 71.33351794249297
5.5 75.1473332827555 75.15446475988165 58.48454593733404 76.4534026249905 79.37218723920795 72.41725969198087
6.0 75.96110310295123 75.87295349366514 59.64332751688035 76.93574842576436 79.6265306122449 73.55817464532282
6.5 76.83930657764965 76.8376526818906 60.9517032091647 77.42150064486762 79.93659054699947 74.4448524391169
7.0 77.71188832410287 77.70908883999697 62.794696912222136 77.77463014945755 80.19333131021925 75.21839010697215
7.5 78.54036112586297 78.6321371671345 64.23538426523025 78.13118124573248 80.21075790911159 75.71494575525378
8.0 79.2866777937941 79.28120779910478 65.46340945300054 78.41917912146272 80.56376602685684 76.38233062741826
8.5 79.76640619072909 79.64693118883241 66.82140201805629 78.61536302253242 80.4402169789849 76.85595933540702
9.0 80.04387375768151 80.17462256277976 68.23391244973826 78.87005538274789 80.72644715878916 77.21826113344966
9.5 80.53206130035657 80.75520066762765 70.21623549047872 79.05066383430696 80.75388058569153 77.82154616493438
10.0 80.6831348152644 80.80211668310446 72.222737273348 79.34075563310824 80.83647674683256 77.99673772854867


==> data/deepwalk/amazon_electronics_photo.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 46.34043947045176 45.897516036577045 46.232741913470726 55.92597243073564 56.27922751467177 49.9965879623311
1.2 51.0930667394568 50.95942404804149 46.93581274737273 62.40652381602293 63.325863245530236 53.13003957963696
1.3 55.849283472089525 55.47832673672717 47.56406441927118 66.1550020472226 67.72171420772486 55.68087894090351
1.4 60.00737000136481 60.65889177016515 48.57862699604204 68.54509348983213 70.01031800191075 56.90135116691689
1.5 63.504585778626996 63.630176061143715 48.04465674901051 70.38561484918795 72.08463218233929 59.36510167872252
2.0 72.00135116691688 72.1662344752286 48.86998771666439 75.95037532414358 77.98476866384605 65.79890814794595
2.5 76.04707247168008 75.65530230653746 51.14778217551521 78.91744233656338 80.95010236113006 70.39370820253855
3.0 78.19601474000272 77.94037122969837 54.95668076975571 80.5211273372458 82.99142896137573 73.65561621400299
3.5 79.51478094718166 79.5050361675993 58.44042582230108 82.00536372321551 84.05683089941313 76.23139074655386
4.0 80.89163368363586 80.97185751330694 59.63624948819435 82.75775897365907 84.43863791456259 77.68889040535008
4.5 81.94685410126928 81.97110686501978 60.53895182202812 83.24250034120377 85.36919612392522 79.02991674628088
5.0 82.88696601610481 82.78258495973796 61.061089122423915 83.92725535689914 85.57264910604613 80.07017879077384
5.5 83.76971475365087 83.89533233246894 61.865088030571854 84.35541149174287 85.942363859697 81.05010236113007
6.0 84.48936809062373 84.45352804694964 63.3431008598335 84.88452299713389 86.23659069196124 82.18247577453256
6.5 85.27633410672854 85.16885492015831 65.13238706155316 85.06609799372184 86.52310631909377 82.69606933260543
7.0 85.52774669032347 85.56811792002183 66.60543196396888 85.38880851644602 86.74097174832809 83.08550566398253
7.5 85.96117101132796 85.84599426777673 69.82428006005186 85.53283745052545 86.75497475092125 83.72766480141941
8.0 86.55431963968881 86.40401255629861 71.59806196260408 85.79148355397844 86.93727309949502 84.17367271734679
8.5 86.6741776989218 86.8257677084755 73.42930257950047 86.07588371775624 87.02441654155861 84.37480551385288
9.0 86.80668759383104 86.78762112733725 74.82003548519177 86.24778217551523 87.16935990173333 84.81903917019244
9.5 87.10174696328647 87.14271871161458 75.41645966971475 86.28657021973522 87.19245257267639 85.15329602838816
10.0 87.22513989354441 87.26455575269551 76.22354305991537 86.43968882216458 87.26733997543332 85.41745598471408


==> data/deepwalk/arxiv.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 7.240699999406681 7.282927798840652 8.687958562503336 14.346378075624616 12.795041621425987 19.418857502239785
1.2 10.786780228191025 10.99685658852637 11.433946233305447 19.910017028295453 19.833609820639243 20.60740226529728
1.3 15.751940454364762 15.68040678046552 15.081486623591605 23.80116706122473 24.771101736648806 21.871663611066612
1.4 19.610883276077914 19.954730246880615 18.188610028301383 26.47682253193547 28.383353802887097 22.912889292346758
1.5 23.526336305868533 23.45196537382152 20.22213441080318 28.58869012655524 31.227159834582274 23.92174459930107
2.0 34.82107652053185 34.97716725108726 26.12152388411266 34.9934527093976 39.04010430572614 28.336317141619645
2.5 40.87093382697591 40.93705523219594 30.059005120355042 38.4166467904333 42.54984484671568 31.99015622126104
3.0 44.478318885981615 44.447060987403816 37.436795951181594 40.60776834398344 44.257198459740245 34.94967219047959
3.5 45.880839904356755 45.92571509941083 41.059498762926964 42.10366019354111 45.3919284692927 37.22329197890152
4.0 46.498624683315235 46.462791097820734 43.26793459235922 43.295025601775215 46.105027797060686 39.1660834327145
4.5 46.7178310579496 46.74374788629607 44.65851147778312 44.174133603887434 46.44392054253217 40.85007683499166
5.0 46.75490527639831 46.774386951697785 45.552615059658365 44.95823914372 46.573025874702594 42.479696575947976
5.5 46.58156850180666 46.69840040820443 46.238901051957065 45.52427095755979 46.68934633891648 43.857474353725756
6.0 46.72617136279762 46.64178280913476 46.4660816527533 46.18798822852329 46.741352651845524 45.02694089935506
6.5 46.66977091899397 46.659345092943646 46.65989094771067 46.56516437941653 46.838340364180056 46.13747945628119


==> data/deepwalk/cifar10_100.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 17.529426715617056 17.52785936176221 17.787574131601243 13.923722112397627 14.6160053657159 11.856241174809375
1.2 18.568010449025703 18.539134425303587 18.68962157582604 14.897465405252754 16.18369810787913 12.193596441683141
1.3 19.748347924315166 19.694344817848062 19.53680457497882 15.6580062129342 17.143243434058174 12.577972324202202
1.4 20.791273651510874 20.81131036430387 20.18726348489127 16.255838746116915 18.119846088675516 12.824442247952556
1.5 21.39250211804575 21.463146003953685 20.717968088110702 16.83229313753177 19.02532476701497 13.214240327591073
2.0 23.9010096018074 23.92432222536007 23.07435752612256 18.71567353854843 21.708705168031628 14.58388873199661
2.5 25.2200155323355 25.320552103925444 24.191118328155888 20.13009743010449 23.5870022592488 15.543921208698109
3.0 26.138089522733686 26.20593758825191 24.918081050550693 20.9990186388026 24.918511719853147 16.319704885625534
3.5 26.852682857949727 26.857744987291728 25.468935329003106 21.74809375882519 25.79739480372776 17.13177068624682
4.0 27.449724654052527 27.470382660265464 25.894027110985597 22.357504942106747 26.430563400169444 17.806347077096866
4.5 28.04476136684552 27.94843264614516 26.30631177633437 22.743751765038123 27.144704885625526 18.309510025416547
5.0 28.33067636260943 28.322648969217735 26.65479384354702 23.236338604913865 27.63856961310364 18.72158994634284
5.5 28.64710533747529 28.711691612538832 27.155831685964415 23.802704038407228 27.976765038124825 19.149039819260096
6.0 29.048503247670148 29.03244846088675 27.360865574696412 24.07149816436035 28.49556622423044 19.60636825755436
6.5 29.23027393391698 29.2509954815024 27.607321378141762 24.46087969500141 28.808733408641622 19.94218441118328
7.0 29.505358655746967 29.412185823213782 27.97786642191471 24.63751765038125 29.03729878565377 20.27737221123976
7.5 29.86541231290596 29.66721971194578 28.210244281276474 24.933811070319116 29.293582321378143 20.538456650663655
8.0 29.95136966958487 29.831841287771816 28.343984750070604 25.16403558316859 29.42825473030218 20.915461733973455
8.5 30.05558458062694 30.035223100818982 28.57915136966958 25.525367127929965 29.693088110703197 21.155683422761932
9.0 30.174795255577518 30.20158853431234 28.744302456933063 25.63690341711381 29.845813329567918 21.472536006777744
9.5 30.373743292855128 30.36123976277887 28.829440835922053 25.98141767862186 29.970785088957925 21.762044620163795
10.0 30.54692883366281 30.448517367975146 29.01945072013556 26.129815024004515 30.26846935893816 21.98542078508896

==> data/deepwalk/citeseer.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 45.18026496116948 45.14291457286432 47.48281407035176 54.02640475102787 53.39086340794884 45.667236180904524
1.2 47.80884422110553 47.749145728643214 50.74095477386935 56.24592964824121 56.790150753768856 48.42075376884423
1.3 52.82246231155779 52.62889447236181 53.375326633165834 57.383115577889455 58.16085427135679 51.1940201005025
1.4 55.67819095477387 55.59246231155779 55.37386934673366 58.70854271356784 58.92241206030151 53.47542713567839
1.5 58.364723618090444 58.56969849246232 56.300653266331665 59.243919597989944 59.6108040201005 55.85748743718594


==> data/deepwalk/cora.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 50.00592750533048 49.64294243070363 52.987718550106614 61.90588486140726 61.53031982942429 54.62575692963754
1.2 54.87667377398721 55.80622601279317 55.16396588486141 64.83611940298508 64.4866524520256 57.13565031982942
1.3 59.53953091684435 59.68810234541577 58.37441364605542 67.36575692963753 67.12622601279318 60.61164179104478
1.4 63.05965884861408 63.550874200426435 60.725842217484015 68.78447761194029 68.69296375266524 62.75846481876333
1.5 65.85006396588486 65.88098081023455 62.05313432835822 69.70004264392323 70.07377398720682 64.72413646055438
2.0 73.12865671641792 73.3710447761194 73.3426012793177 73.31292110874202 73.37547974413646 72.99513859275054


==> data/deepwalk/cora_full.tex <==
degree 


==> data/deepwalk/fashion_mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 33.18091660138167 33.13400398831992 35.739876077202474 45.07977352040453 45.712598817748024 38.49496118510078
1.2 37.2461149490777 37.1403746171925 37.48761484224771 52.643152197136956 57.684844384303126 39.902172209956554
1.3 40.423527526529455 40.24081974218362 38.56886973862261 56.2473648600527 62.516925432661495 41.09412078911758
1.4 42.68590912328182 42.69129691617407 38.996613489067734 58.38467345630654 64.62568549248628 42.27430382451393
1.5 45.32933195641336 45.168624029627516 39.21379175272416 60.04128267217433 66.20640267787194 43.22122355957553
2.0 52.53513282529734 52.557367708852645 40.33919592621608 64.48350188732996 69.85438715191225 47.45483939890321
2.5 56.78911758421765 56.8941101061178 43.43170714336586 66.66538351969234 71.57013389359732 50.76151627376968
3.0 60.24054554518909 59.997674667046496 46.25297699594046 67.9443095221138 72.68914251121714 53.18869382522612
3.5 62.25395627092086 62.535816537283665 47.22467416850651 68.91383092372338 73.32934620041308 55.171266291574675
4.0 64.43817391923653 64.4407698881846 47.78337369133253 69.49795598604088 73.67097072858058 56.88959119720819
4.5 65.94255394914892 65.80852859482943 48.465048785699025 70.228099850438 74.07432162951356 58.12217790755644
5.0 67.27740545545188 67.36827861263443 48.8746100705078 70.6937646891247 74.27161170856775 59.11381311872373
5.5 68.64834413503313 68.5087600598248 49.368114806637706 70.97170073356598 74.48213802435724 60.17302542553949
6.0 69.25221138095577 69.23052133038958 49.69784915604302 71.39982907200341 74.69123637917527 60.82631578947368
6.5 70.13997934620039 70.0081404458372 50.125653443486925 71.72391567552168 74.69951214300976 61.62212805355743
7.0 70.91764831564703 70.86600313367994 50.067295776654085 71.80889181682217 74.8852859482943 62.36690406666191
7.5 71.59431308311373 71.53237661135246 50.27304323053914 72.08889680222207 74.91634855067304 62.76060109678798
8.0 72.14892101702158 71.99783135104337 50.40754931984901 72.23215939035681 75.05180186596395 63.4173954846521
8.5 72.48066733138664 72.53046791539064 50.47467060750659 72.31114236877715 75.11712840965743 63.780457232390866
9.0 72.8015597179688 72.79629656007405 50.600121073997585 72.6045758849085 75.27301118153977 64.26802222063954
9.5 73.03330959333381 73.01024143579518 50.62491275550174 72.62822804643544 75.23792108824156 64.63667117726658
10.0 73.17449611851006 73.26083256178335 50.62958478740831 72.76010611779789 75.36317213873656 64.95131044797378

==> data/deepwalk/mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 39.25910367566247 39.417362722351115 38.835641307444945 50.4850022387756 64.58740994016364 37.129053201449096
1.2 51.854573207961906 52.3706313347173 45.23656327593927 61.888879391053045 86.0514694508894 38.767818618471935
1.3 60.893446493263326 60.09195668986852 49.17462246102496 68.32666585256645 91.52707086742377 39.98285504945659
1.4 64.89338136524607 65.20313225058005 52.5664102250987 72.90461594822322 93.50623804290308 41.29913298327024
1.5 68.37116457035862 68.78798998656734 55.39556315382425 75.98852932796028 94.53408027028127 42.514436032075544
2.0 82.86609679651565 82.61715716204665 63.03784751902959 83.92526356494486 96.19214393291814 47.46193063866162
2.5 88.65957992428868 89.13788618878984 67.03610127406685 87.45843814873611 96.52606545365735 51.20463019497701
3.0 91.78781699027151 91.68426140757929 69.86612325477266 89.3898909105711 96.6841026580372 54.30367973297514
3.5 92.87207636260023 92.8339520494973 71.78352464688403 90.53933935767493 96.77269507876419 57.18506329629176
4.0 93.58418406805878 93.36928806936135 73.49147840599178 91.54724427076974 96.84463711482884 59.537326494891516
4.5 93.97325680791305 93.77966581186143 74.62802336467618 92.14702853421257 96.89056254324908 61.68262710139618
5.0 94.20224895184597 93.97737819025521 76.02731713273904 92.63498188627021 96.8713864126674 63.63508975454879
5.5 94.2202018968535 94.11887491350186 77.1955407660683 93.04198314812552 96.90110310579232 65.34343835226116
6.0 94.38964464525583 94.27514144991248 78.3872430496194 93.37202955183783 96.84025114991654 67.01634916758253
6.5 94.46911914356659 94.46764969267717 79.73791875279848 93.58834004966012 96.95026865307119 68.3620690356983
7.0 94.48497171001749 94.53800016282004 80.58981153580007 93.82906541295233 96.90367159197297 69.78697236129767
7.5 94.62541620873529 94.67693857613871 81.93396222575001 94.11153783530752 96.9310864167379 70.8460841779623
8.0 94.84385557862171 94.80185614849188 82.72836935726787 94.20202914478773 96.9174705906297 72.13007082671878
8.5 94.82098343306062 94.86795294500753 83.60956160703383 94.41366670737168 96.96767411568365 73.12971872837547
9.0 95.00457320796191 95.01676842919363 84.49491390890218 94.55485000203525 96.9594822322628 74.0066430577604
9.5 95.17944396955265 95.13382993446493 85.41856555541987 94.69077420930516 96.95082427646844 74.80034802784223
10.0 95.3392233483942 95.31431188179265 86.32163267798266 94.80959417104245 96.96422029551839 75.70210444905767


==> data/deepwalk/ms_academic_phy.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 28.84154915244381 29.222225452853777 34.17960050010176 44.14615764835868 38.58591864623616 48.803410577733835
1.2 36.26715319977903 36.506966533887706 39.88151077254092 57.518393277701854 53.09847061902131 51.70245108016167
1.3 41.58336580118046 42.01165353414939 43.06851684935888 65.0479254499462 63.0484313668479 53.91751809961329
1.4 46.01367138661937 45.67877765824441 46.03213153839444 68.94710551565727 69.01519786002966 56.40487599220773
1.5 49.65303986276277 49.7463117494839 48.98071991393597 72.05478149623471 73.20599831361032 58.23895850899893
2.0 63.251225540080824 63.441307824266566 54.18779984299131 78.66127118890472 81.837187799843 66.18696537086034
2.5 73.48801500305294 73.46821155467683 54.70170674265111 81.45766871165645 84.3845520890879 71.9276974965836
3.0 79.56801965516237 79.74917570435844 58.24048788997761 83.06462361527055 85.71724769575204 75.64486959555725
3.5 83.44862326636235 83.5239583636205 66.85106271625041 84.20935655511296 86.45562759863927 78.96632454278489
4.0 85.75986974093566 85.57045619748206 74.42561858517722 85.09083243683307 86.81441572412992 80.9654261041491
4.5 86.73231471520366 86.69169016951123 79.98214753002064 85.77584101415987 87.11480533829558 82.92094030762073
5.0 87.32779635390922 87.23960689675224 83.97457331433723 86.23161399121915 87.3186898496787 84.13228563951965
5.5 87.38522373738843 87.40558253132905 86.34157532055943 86.57278806733929 87.3649870613206 85.130843485593
6.0 87.5743959526648 87.6324106649609 87.30469572296688 86.90884482307447 87.49289099526067 86.07847527113076
6.5 87.66388218532842 87.56363213444595 87.6036664437531 87.27380571627948 87.59017241880616 86.84211903585033
7.0 87.58431076091064 87.56992702003316 87.5526473410287 87.45409531009217 87.53120983921147 87.32228651179018


==> data/deepwalk/pubmed.tex <==
degree mst-plus-best-filter-edge-modularity_ACC mst-plus-best-filter-edge-significance_ACC mst-plus-best-filter-spectral-radius_ACC random-plus-tree_ACC random-tree_ACC random_ACC
1.1 44.63466449610825 44.69977616116395 45.04744365874752 51.5039120923844 50.33839344762679 52.628386834206644
1.2 50.88852317240678 50.89786335656509 47.520201454952435 57.82206847433484 57.132680470061544 54.521737803327056
1.3 56.30671007783488 56.28353767105866 51.744482881416296 60.55157958996794 60.623157145037396 55.9801800885181
1.4 60.00243170371877 60.10237574400976 55.90312865645826 62.20978786183039 62.935992267385664 57.54537314951417
1.5 63.22291295721625 63.22902273999084 57.874563768632036 63.465940886198304 64.40733580912652 59.02107646131148
2.0 67.52312153431349 67.58723609909954 67.95354326702956 67.31944345525767 67.96895253599227 65.19418527750929


==> data/gcn/amazon_electronics_computers.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 76.52530991735537 76.53195100354192 72.54198642266824 68.82681523022431 74.66226387249114 75.06832939787485
1.2 77.0633116883117 77.21288370720188 72.81884592680048 69.45476682408501 74.90547520661156 75.05925324675324
1.3 77.23819362455724 77.51188016528926 72.93440082644628 69.57541322314049 75.43012101534828 76.05283353010626
1.4 78.07216646989374 77.5180785123967 72.92414403778041 69.89912927981112 75.62529515938608 76.23413518299881
1.5 78.16927390791025 78.07445395513577 72.80917945690675 70.34297520661156 75.45609504132231 76.2991440377804
2.0 79.24786009445099 78.85765938606848 73.70853010625738 72.31700118063755 76.37824675324676 77.32238783943329
2.5 79.92252066115702 79.64344746162928 74.5707644628099 73.07533943329399 76.39138134592682 78.842606257379
3.0 80.59836186540734 80.2947904368359 75.27324380165291 74.63636363636364 77.15001475796929 78.33928571428574
3.5 80.49291617473436 80.8784681227863 75.5442739079103 74.77944214876032 77.19849468713103 78.58234946871309
4.0 80.81714876033058 81.22387839433294 76.03549291617473 75.23472550177095 77.3344893742621 78.78180342384888
4.5 81.58603896103895 81.04449527744981 76.36585005903189 75.91248524203071 77.27486717827625 79.06987898465172
5.0 80.99011216056672 80.93159681227864 76.65577036599763 75.92141381345925 77.29456906729634 78.9715909090909
5.5 81.19642857142857 81.28984651711924 77.7117030696576 75.92185655253836 77.73863636363636 79.16624852420307
6.0 81.24512987012989 81.02265348288076 78.09718122786305 76.63924144037783 77.6805637544274 79.25014757969302
6.5 80.68344155844156 81.41765053128692 78.60286304604486 76.55718713105077 77.70137249114521 79.18322018890198
7.0 81.07489669421486 80.8030548996458 78.86887544273908 76.60323199527744 77.98900531286895 78.85699527744981
7.5 80.91447756788664 80.72564935064938 79.1586481700118 76.90968122786305 77.47756788665879 79.37079397874852
8.0 81.07224025974025 80.58257083825265 78.9020808736718 77.10242030696578 77.79892266824086 78.90931227863048
8.5 80.1944362455726 80.27494096812278 79.36216056670601 77.31648465171192 77.71199822904367 79.43425324675324
9.0 80.33043093270365 80.4862012987013 78.6276564344746 77.44871605667059 77.84651711924437 78.92104486422667
9.5 80.24468713105075 80.53482880755605 79.25516528925618 76.9991145218418 77.6952479338843 78.9275383707202
10.0 80.17680047225501 80.32061688311688 79.02398170011807 77.32865997638724 77.92650531286895 79.06973140495867

==> data/gcn/amazon_electronics_photo.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 85.26728971962618 85.21455273698265 81.85327102803738 80.36648865153538 84.15447263017357 84.11415220293726
1.2 85.11575433911884 85.16662216288384 81.77890520694258 81.51615487316423 84.5154873164219 84.4237650200267
1.3 85.6173564753004 85.66822429906543 81.8652870493992 81.7638184245661 84.88838451268357 85.02817089452604
1.4 85.72336448598132 85.516955941255 81.88437917222964 81.8927903871829 85.42069425901201 85.3543391188251
1.5 85.90053404539387 85.79612817089455 81.91735647530041 82.23711615487316 85.3600801068091 85.92283044058745
2.0 86.80120160213619 86.3562082777036 82.42429906542057 83.59706275033378 86.34098798397865 86.986782376502
2.5 86.93978638184247 87.2902536715621 82.596261682243 84.64032042723633 86.66542056074766 87.883044058745
3.0 87.31508678237651 87.53337783711616 82.76074766355138 85.26141522029373 87.14712950600801 88.07823765020026
3.5 87.61241655540721 87.556608811749 83.02082777036048 86.07716955941252 87.43364485981307 88.47676902536715
4.0 88.08598130841122 87.96101468624832 83.09933244325768 85.9014686248331 87.83004005340453 88.45300400534046
4.5 88.38197596795726 88.36395193591454 83.55674232309745 86.36662216288384 87.86355140186916 88.82202937249669
5.0 88.49372496662215 88.61762349799733 83.44606141522027 86.76809078771696 87.57823765020025 88.90520694259013
5.5 88.51068090787714 88.7935914552737 83.90854472630177 87.28237650200266 88.29225634178903 88.65447263017356
6.0 88.87583444592791 88.70240320427237 84.26995994659548 87.26728971962615 88.26355140186914 89.15781041388519
6.5 88.86475300400535 88.87329773030707 84.43324432576767 87.45140186915887 88.43230974632844 89.18811748998664
7.0 88.90387182910547 89.0305740987984 85.01682242990654 87.64619492656877 88.30667556742324 89.04178905206943
7.5 88.98571428571428 89.09572763684915 85.27196261682244 88.14993324432578 88.44432576769024 88.95500667556742
8.0 89.15193591455272 88.816955941255 86.12042723631507 87.99599465954606 88.16702269692925 88.87903871829106
8.5 89.01028037383176 89.03217623497999 86.56395193591455 87.95834445927903 88.60360480640855 89.01388518024034
9.0 89.10667556742322 88.96154873164218 86.6708945260347 88.07636849132174 88.56969292389853 89.11708945260348
9.5 89.04672897196262 89.03230974632844 87.13204272363151 88.15246995994659 88.48958611481976 89.2154873164219
10.0 89.15140186915886 89.23484646194926 87.5929238985314 88.03671562082776 88.56301735647531 89.09198931909212

==> data/gcn/arxiv.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 36.69829064393063 36.21657381202424 35.93878120123648 34.177924921236716 36.76604783349057 38.00294286917879
1.2 37.304248767376876 37.162979180387204 36.664234053030974 34.60831294618518 38.359943753226176 37.55670659712952
1.3 37.24895130619486 37.29042440208137 37.326201622137965 35.21712559999525 38.34736536076847 39.150246524625764
1.4 38.52559880861264 38.276107580854735 37.32887156393325 36.198308019742306 38.495042808066785 39.04511014993207
1.5 37.87134440469198 39.00595100360146 37.78021039141347 36.73721246210165 38.71053677696493 39.67284313201972
2.0 40.051974866947894 41.256415276813634 38.93742249752289 38.63392592856291 41.09188753018518 41.94549758815258
2.5 41.96525515743757 41.82161228885211 40.239464113015664 40.324575924244854 42.31543285689705 42.9606094587138
3.0 42.878078591220046 43.26243154565897 40.83420848092178 41.236530567443154 42.26434797054758 44.02879054273654
3.5 43.7472336436399 44.403446004877104 42.01046617183746 41.19107092354275 43.16014310888023 44.563965542588214
4.0 44.23375637077779 44.5997163928493 42.74054692274375 42.33960736692977 43.89028319182642 45.19398610443626
4.5 44.84600369045288 45.552588953560814 43.91526198062216 43.555947147018856 44.042351210076944 44.55517286389823
5.0 45.33217042535139 45.2905786653851 43.88601128495399 43.69730573206837 44.235951656253896 45.62592335487087
5.5 45.12937351299075 45.1011907940407 44.8792889648339 44.8189037812309 45.45629305281144 45.17535584390927
6.0 46.02071874833129 45.34474881780911 44.88314554742707 44.57682081789876 45.59133277561217 45.26910046694315
6.5 45.42170247355274 45.57246518692559 45.76505698842432 45.058531057356284 45.016701969230404 45.547664394249544


==> data/gcn/cifar10_100.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random-plus-tree random-tree
1.1 10.02690763052209 10.023427041499332 9.983935742971887 9.991967871485944 10.05421686746988
2.0 10.007831325301204 10.003212851405623 nan nan 9.991967871485945
2.5 10.012248995983937 10.069277108433736 9.989959839357429 10.052208835341366 9.983935742971887
3.0 10.041365461847391 9.993402180149168 10.00878514056225 9.923694779116465 9.993975903614457
5.5 9.991164658634538 nan 9.981481481481483 nan 9.970883534136545
6.0 10.028915662650602 10.053012048192771 9.995180722891567 nan 10.052543507362786
6.5 10.010040160642571 9.977710843373496 9.977510040160643 nan 9.872824631860777
7.0 9.985441767068274 10.018473895582328 9.987951807228916 9.97289156626506 10.02058232931727
7.5 10.04066265060241 9.973226238286479 9.979250334672022 10.034538152610443 9.986947791164658
8.0 10.02565818830879 10.01706827309237 9.971218206157966 10.020833333333332 9.950803212851406
8.5 10.012048192771083 10.006024096385541 10.034805890227576 9.966867469879519 9.985943775100402
10.0 10.002409638554218 10.05371485943775 9.97991967871486 10.08433734939759 10.021586345381525


==> data/gcn/citeseer.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 64.41273638642062 64.42543859649123 64.54260651629073 63.78571428571429 64.82114376851217 64.49419002050581
1.2 64.7562656641604 64.59711779448622 64.75908521303259 63.7359022556391 64.81954887218045 65.0905388471178
1.3 64.61372180451127 64.6986215538847 64.62499999999999 64.08646616541353 64.81077694235589 64.61466165413535
1.4 64.8186090225564 64.86591478696742 64.94674185463658 64.42888471177945 64.70426065162907 64.74091478696742
1.5 64.87531328320803 64.7578320802005 65.03696741854637 64.57832080200502 64.99906015037595 65.10996240601504

==> data/gcn/cora.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 74.69587227414331 75.06308411214951 74.226246105919 73.15732087227413 75.57904984423678 75.17718068535824
1.2 75.19976635514018 75.32009345794393 74.65381619937693 73.6985981308411 75.8454049844237 75.85007788161994
1.3 75.21534267912773 75.56386292834891 75.25233644859814 74.28435444790584 76.49532710280373 76.35046728971962
1.4 75.77258566978195 76.29322429906543 75.55646417445482 74.77890273451021 76.68457943925233 76.91666666666667
1.5 76.56191588785046 76.40459501557632 75.98870716510903 75.5443925233645 77.047507788162 77.21495327102805
2.0 78.67834890965732 78.17172897196264 78.54633956386293 78.66433021806853 78.31191588785047 78.6176012461059

==> data/gcn/cora_full.tex <==
degree 


==> data/gcn/fashion_mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 14.560183946488293 15.116772575250836 14.67252508361204 13.713862876254183 15.071254180602006 14.417959866220736
1.2 15.108745819397996 14.27511705685619 14.575501672240804 13.759397993311037 14.347926421404683 15.071839464882942
1.3 14.74896321070234 14.887190635451505 15.423528428093643 13.657809364548495 14.96408026755853 15.2206856187291
1.4 14.775117056856187 14.665418060200668 14.304381270903011 14.605903010033447 14.993545150501674 15.745602006688964
1.5 14.835936454849497 15.313177257525085 15.196521739130434 13.867608695652173 15.558729096989964 15.850518394648827
2.0 14.789882943143812 15.171471571906356 14.77469899665552 14.338010033444814 16.634013377926426 16.241722408026757
2.5 15.44953177257525 15.457408026755854 15.250484949832774 14.539816053511705 16.66130434782609 16.871672240802678
3.0 16.008578595317726 15.213110367892977 15.245618729096988 15.439866220735784 16.571989966555186 16.534983277591973
3.5 15.090501672240809 14.928996655518398 15.634581939799332 15.152608695652175 16.808595317725757 17.918578595317726
4.0 15.841655518394655 15.927123745819397 15.030434782608696 16.015334448160534 16.394565217391307 16.780702341137125
4.5 16.418377926421407 17.167341137123746 15.445234113712376 15.726471571906353 16.48887959866221 18.043344481605352
5.0 16.440501672240803 16.64804347826087 16.298143812709032 15.737876254180602 17.780367892976585 18.116789297658862
5.5 16.36098662207358 16.571421404682273 15.464548494983276 16.10112040133779 17.19804347826087 19.003595317725747
6.0 16.26605351170568 16.483612040133778 15.795284280936455 16.022240802675583 17.111705685618727 17.715969899665552
6.5 15.996555183946489 15.90515050167224 16.48988294314381 16.007341137123746 17.644280936454848 19.01814381270903
7.0 15.983127090301002 16.218060200668898 15.9352508361204 16.22826086956522 17.86376254180602 17.754899665551836
7.5 16.453394648829434 16.392759197324413 16.067391304347822 16.147240802675586 17.165886287625415 18.338127090301008
8.0 16.72826086956522 16.802558528428097 16.289046822742478 15.884013377926424 17.25013377926421 17.63678929765886
8.5 16.47031772575251 17.41864548494983 16.784013377926417 15.540284280936453 18.25314381270903 17.844531772575255
9.0 16.50722408026756 16.358177257525085 16.781638795986623 16.16596989966555 17.62289297658863 19.622809364548495
9.5 17.718511705685625 15.906688963210701 15.78133779264214 16.86608695652174 17.60775919732442 18.722909698996652
10.0 17.062458193979932 17.58220735785953 16.44774247491639 16.055836120401338 16.71725752508361 18.75665551839465

==> data/gcn/mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 44.79297658862876 56.903010033444815 nan 32.27173913043478 52.82374581939799 47.73428093645485
1.2 53.394983277591976 nan 54.07107023411372 29.913879598662206 54.07157190635452 51.25367892976589
1.3 51.24999999999999 nan 48.47305834262356 30.734448160535116 49.16521739130435 52.38277591973244
1.4 51.7257525083612 43.28260869565217 48.83277591973244 32.72709030100335 47.238963210702344 52.539297658862885
1.5 48.207357859531776 54.25083612040134 nan 30.122575250836114 47.37374581939798 58.79581939799332
2.0 59.55369751021924 nan 58.45526755852843 34.61371237458194 53.89632107023412 60.54498327759197
2.5 59.96536072623029 nan 59.28846153846155 37.36404682274247 53.624749163879606 71.43645484949833
3.0 69.7962255136168 nan 59.96521739130436 37.94314381270903 61.58327759197324 70.63996655518395
3.5 66.57329988851728 nan 57.16789297658863 42.904347826086955 57.03996655518394 74.37441471571906
4.0 65.05602006688963 nan 60.95484949832777 41.55769230769231 62.09347826086956 71.66454849498328
4.5 70.0709507883421 74.27792642140469 60.7623745819398 39.08879598662207 62.292642140468224 77.15050167224081
5.0 72.82650501672241 69.3331475287997 60.538127090300996 42.39113712374582 61.12591973244148 75.10083612040133
5.5 nan 72.5018580453363 63.27424749163881 44.9 65.02408026755853 77.00752508361204
6.0 nan 71.94063545150502 65.94598662207358 49.88795986622073 60.86220735785953 74.8391304347826
6.5 nan 73.9314381270903 62.9148829431438 42.44715719063545 63.68561872909698 72.26705685618728
7.0 nan 72.25343738387218 63.5958193979933 45.06404682274249 67.38344481605351 76.7061872909699
7.5 nan 74.11204013377926 63.64498327759197 50.96672240802677 64.45217391304348 76.31321070234114
8.0 nan 73.15501672240802 65.50769230769231 50.290301003344474 64.43862876254181 75.85418060200668
8.5 66.61872909698997 75.05418060200668 65.29581939799331 54.90200668896321 65.4705685618729 77.17073578595318
9.0 nan nan 70.06404682274248 53.22441471571906 66.16488294314381 75.33595317725752
9.5 nan nan 67.38461538461539 54.728762541806006 66.45301003344481 72.89147157190635
10.0 74.04983277591974 nan 69.73578595317727 55.95200668896321 67.80351170568562 76.63327759197325


==> data/gcn/ms_academic_phy.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 90.98223475707266 91.0165440641991 88.8366237315733 90.30229988660483 90.32997993777802 90.25653475998023
1.2 91.09743261710234 90.89323408833194 88.82830808594771 90.59858110662051 90.5936382403396 90.67124124095018
1.3 91.04111301718372 91.27758555520019 88.94961183961854 90.50510278254296 90.70834181374117 90.82039949989823
1.4 91.18332218765447 91.12793300962406 89.11115633995291 90.6073910388742 90.96080597796063 90.97534381996337
1.5 91.23545488907628 90.99764486959556 89.18442706364667 90.62524350885354 91.02012037333178 91.08187712615941
2.0 91.4696013723723 91.63983950222429 89.48486610647517 90.91259849387957 91.46974675079231 91.60445439478964
2.5 91.94289535661325 91.97563457680342 89.97743726921175 91.4797197104062 91.7383479196348 91.94664611984997
3.0 92.39446980490217 92.31843689122788 90.3499549326898 91.83874625650569 92.09926438519467 92.2899427209025
3.5 92.40063384991132 92.41537522170209 91.06608902974442 91.78361875963131 92.02465618003663 92.36519059110867
4.0 92.46762422585991 92.61404937051144 91.72761899223678 91.9542639490594 92.287296833658 92.49111737853632
4.5 92.60852499055039 92.6457127903934 91.95752042566802 92.11702962812201 92.40075015264733 92.4782077748379
5.0 92.6244875410694 92.74558776495216 92.21577065100458 92.25007995813101 92.3888581978891 92.39307417206989
5.5 92.63847294507602 92.60407641089758 92.51929171633763 92.34193004390428 92.38740441368881 92.54958857907133
6.0 92.6495507806821 92.69159421975402 92.61431105166749 92.58732881691041 92.3660047102608 92.59442328380774
6.5 92.75521181635798 92.81249091384875 92.74163347192743 92.5888698281627 92.66231500596051 92.61134533189893
7.0 92.6291687261943 92.67976041636379 92.62303375686913 92.84883551885557 92.72793882476084 92.59328933213156

==> data/gcn/pubmed.tex <==
degree mst-plus-best-filter-edge-modularity mst-plus-best-filter-edge-significance mst-plus-best-filter-spectral-radius random random-plus-tree random-tree
1.1 72.65732309101084 72.72773057943735 72.26290888741923 71.80164826779266 72.86137253904462 73.03515287175053
1.2 73.08836546777229 73.08638144172559 72.43841888385816 71.92826982754235 73.09508063285344 73.04822709467363
1.3 72.92353868850793 73.09340184158316 72.79142290278271 72.42564989571146 72.98789235386884 73.18130945719082
1.4 73.33896321920943 73.28722592460701 72.67568805005851 72.21926031439182 73.14096759424123 73.0881111054586
1.5 74.16899832120875 73.38769903851046 72.55837615098947 72.71424937681233 72.82937375998372 73.30620135320751
2.0 73.77819606247135 74.27822149870276 73.69741059164673 72.61682861067305 73.63641450882636 73.87922877346493

==> data/stats/amazon_electronics_computers.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 2925480.460897503 10.652910655909785 3.7691675420544706 1471900.0 212975.35237988117 1112.6038254169048 919.5605747042988 100.0 2931435.013072368 10.652910655909785 3.7691675420544706 1471900.0 210888.37765095168 1112.7383578239487 919.5605747042988 100.0 2349216.2154552005 7.7349490782519 1.2334199246056827 1471900.0 200066.5279603055 1125.2899406964632 1246.8017914452605 100.0 1538045.6168812234 0.1052661232765542 0.1771032351440801 1471900.0 362072.8341779313 1126.219529118615 1080.319274787648 100.0 1552995.3819594192 0.19905680351191288 0.3716085266278857 1471900.0 368591.16228019644 1123.9114016686476 1050.4382613356797
1.2 100.0 2587936.1312259724 14.32438059546117 5.3207446963519 1605700.0 334879.8175636171 1130.2565388930477 974.9449987746008 100.0 2587473.8997691316 14.32438059546117 5.3207446963519 1605700.0 335124.0874122261 1129.9927128347872 974.9449987746008 100.0 2093454.5066047402 12.591445284949732 1.67230216100604 1605700.0 273936.5371044799 1151.5723937359783 1738.3299037165325 100.0 1355754.8230204603 0.2099233901596994 0.3913923877462098 1605700.0 497495.95780334575 1141.8649333663252 1152.1327244962163 100.0 1359856.7195906315 0.3432552581065432 0.7177155850118282 1605700.0 518098.4964114371 1137.5291878496407 1108.6157471883312
1.3 100.0 2320040.177962444 15.456452720892669 6.281347089582646 1739500.0 451182.37241392373 1145.318128628508 974.9866213526044 100.0 2314479.4450298036 15.456452720892669 6.281347089582646 1739500.0 452364.6860131974 1144.810360646114 974.9866213526044 100.0 1914455.0761752026 14.724669810434552 2.027063069456083 1739500.0 334493.86534284725 1177.2118623727495 2126.308200397335 100.0 1225886.595632483 0.2962496662799775 0.5914400506876418 1739500.0 615066.8582365249 1156.0587789595409 1257.8724180953234 100.0 1194441.8758563004 0.47007440932984007 1.1097815144474954 1739500.0 660125.9647570504 1150.223802495118 1173.5478574336673
1.4 100.0 2076646.2012510826 16.240828591912383 7.026118840137399 1873300.0 561586.5921411653 1158.8803176322613 975.0510133760185 100.0 2072285.3579461174 16.240828591912383 7.026118840137399 1873300.0 562033.7045814757 1159.1156955740573 975.0510133760185 100.0 1732013.0514006938 17.688870575206998 2.408584584398176 1873300.0 392653.01737802714 1204.2264638237066 2574.027976558067 100.0 1115891.6348633717 0.3655877136453844 0.798528120365091 1873300.0 722344.9568135695 1169.4927814515343 1310.5617919259084 100.0 1068026.995336259 0.5942014333528424 1.4561872745680442 1873300.0 785169.7534093384 1161.1742240739113 1221.5278965462244
1.5 100.0 1879561.0755686837 16.75652776708003 7.603373610387506 2007100.0 662418.640799149 1171.743048847312 1004.8133928770989 100.0 1881824.2720945906 16.75652776708003 7.603373610387506 2007100.0 662050.625450022 1171.8811242875988 1004.8133928770989 100.0 1582698.7102479534 23.12068041605408 2.8149104811537717 2007100.0 456662.4751370428 1233.513930720257 3811.144978819086 100.0 1024453.6530474119 0.41527499455209055 0.938617368471229 2007100.0 821712.121470214 1181.0787442721864 1376.9479164660452 100.0 967814.363025282 0.6747081279382642 1.7591560188898823 2007100.0 899656.5352735526 1171.8129547222422 1271.600239019091
2.0 100.0 1263907.2241422404 17.167604678082466 9.883271953036413 2676200.0 1094505.9276388003 1221.0568856468858 1151.2568972375955 100.0 1263420.8697841489 17.167604678082466 9.883271953036413 2676200.0 1095989.1706995415 1221.287435437598 1151.2568972375955 100.0 1292702.3878707818 27.810991320009006 5.0179667017387 2676200.0 685488.4749797772 1310.0019073211233 5482.753331862282 100.0 747475.5392705101 0.7474749899134832 1.9318237653659236 2676200.0 1212910.2057716793 1231.4655403629745 1748.0139910142277 100.0 610774.1477863252 1.0130415471342982 3.543559941929733 2676200.0 1404361.31130214 1214.773738519408 1446.7116697126482
2.5 100.0 953121.3237288527 16.957017020442056 11.401943781637605 3345200.0 1438272.608569303 1258.025710313732 1395.0539802319022 100.0 953396.3820766443 16.957017020442056 11.401943781637605 3345200.0 1439213.083130243 1258.1012057872035 1395.0539802319022 100.0 1097857.3868979414 27.386515028432168 7.588995932576761 3345200.0 927485.937546573 1346.1097688074774 5726.92057266399 100.0 591990.4776906216 1.0601424602105696 2.9582152798860766 3345200.0 1510904.4770629136 1270.4851589837263 2159.3632788404057 100.0 466953.6737018444 1.376866823274242 4.721932470781113 3345200.0 1735204.884731261 1250.218784460036 1628.878940337822
3.0 100.0 761934.5936228498 16.99214359411836 12.652990502183052 4014300.0 1718304.492020845 1287.8316834650368 1610.7053446207708 100.0 762474.4865305229 16.99214359411836 12.652990502183052 4014300.0 1717259.149007013 1287.7451520121338 1610.7053446207708 100.0 984400.7100778852 26.828260499566298 9.659745895977524 4014300.0 1143430.353882076 1364.9526140209734 5763.345204726693 100.0 494985.00378907955 1.3829621553066436 4.0038698730733 4014300.0 1748173.754821397 1300.9557482058779 2591.567390708478 100.0 371732.34061160794 1.6654731990276803 5.884847564937183 4014300.0 2012637.746140806 1278.3567999963902 1860.6270416690577
3.5 100.0 631586.2692366925 17.2135930951948 13.665965448652944 4683300.0 1954646.1826999858 1313.1799718750142 1763.0199714561916 100.0 631421.747287267 17.2135930951948 13.665965448652944 4683300.0 1954499.065912991 1312.7439741319538 1763.0199714561916 100.0 903924.1367274524 26.977307155621112 11.433065478375033 4683300.0 1324615.7672863735 1386.9280263077417 5766.113620846036 100.0 423384.8573881782 1.7008510467196487 5.087879058333327 4683300.0 1949135.004774859 1327.9299351383454 3063.6756845356454 100.0 314883.9472152135 1.9758469611342269 7.004987903701062 4683300.0 2228155.8894052277 1302.6014778529006 2022.263896892243
4.0 100.0 545624.4051091055 17.444429938446216 14.712106613716786 5352400.0 2151432.888351438 1335.2763718568951 2023.8817703349985 100.0 545066.6768206051 17.444429938446216 14.712106613716786 5352400.0 2151206.3993345313 1334.861087796669 2023.8817703349985 100.0 831319.0406165387 27.178411112081285 13.045147489672173 5352400.0 1498016.6294585085 1408.4805213527409 5768.241591960941 100.0 372236.3813650942 1.9900086971155695 6.072267560280762 5352400.0 2122535.532863155 1350.3689259500777 3528.5645837102566 100.0 271943.02615164284 2.262330342036428 8.025267506837128 5352400.0 2416354.9921043194 1324.6228496360463 2215.9356721484487
4.5 100.0 480289.3628256681 17.638582069406052 15.648250796213665 6021400.0 2322872.3822238515 1354.8592314568089 2228.501661142419 100.0 480227.6403206772 17.638582069406052 15.648250796213665 6021400.0 2321885.6012967657 1354.667691264656 2228.501661142419 100.0 770086.393465637 26.863683011253936 14.562040582417476 6021400.0 1657476.4912232407 1421.2056981855294 5769.1715380377755 100.0 332272.4741918978 2.30961287433832 7.186573216761068 6021400.0 2275954.861883338 1370.9198165091173 3968.4931751281324 100.0 241146.86435022246 2.4986347214959466 8.99500450305677 6021400.0 2577685.9306420637 1343.2371179429945 2422.7108223533705
5.0 100.0 427624.9500961955 17.857684706036725 16.465504614223427 6690500.0 2478364.580730678 1372.4040010416275 2366.666507047389 100.0 427743.6934137972 17.857684706036725 16.465504614223427 6690500.0 2478033.745999742 1371.9842941354154 2366.666507047389 100.0 707922.5347820526 26.143074632774045 15.852495557718873 6690500.0 1815419.7606384412 1435.2047137580757 5770.593449649277 100.0 298232.9377709371 2.6108686145769258 8.138090057624211 6690500.0 2416520.948347287 1390.49449351614 4437.399138153106 100.0 217965.08746489888 2.786577545470719 9.996946734351235 6690500.0 2716058.4444906004 1360.734358131542 2622.463646950032
5.5 100.0 381773.46419129014 18.042407922374 17.311948147093695 7359500.0 2617848.647435171 1388.4535497708748 2467.813685584581 100.0 381501.657265363 18.042407922374 17.311948147093695 7359500.0 2618007.22031782 1388.73925577933 2467.813685584581 100.0 649942.5461141678 24.975479437021594 16.875149553759467 7359500.0 1967250.5503816716 1446.8834364543402 5771.389033191723 100.0 272136.0087734598 2.9145248183601424 9.171208798854561 7359500.0 2539576.7131280103 1407.6981428340869 4904.804676328645 100.0 199409.373394215 3.016100255952808 10.858613053141642 7359500.0 2840918.053945475 1376.9070554763573 2836.0140005188373
6.0 100.0 343201.9655303632 18.00722715161696 18.042919332522207 8028600.0 2745062.9091647076 1403.7519320145943 2577.412313687276 100.0 343400.8597597576 18.00722715161696 18.042919332522207 8028600.0 2745669.9389772452 1403.9361117653968 2577.412313687276 100.0 580553.2134549007 23.69375807075364 17.865688198447998 8028600.0 2124131.6946766167 1457.8310256450568 5771.778090334921 100.0 250079.66120673405 3.216140410538719 10.24417187882534 8028600.0 2653116.81025263 1421.9894945567153 5357.643450757776 100.0 183914.18496747615 3.2492905842181354 11.749503754232204 8028600.0 2953952.0402635396 1391.9294193125002 3066.104726901984
6.5 100.0 306269.4405417616 17.83547370840111 18.62537936596395 8697600.0 2864856.550059158 1417.3324574430756 2815.5079541796495 100.0 306494.3725531433 17.83547370840111 18.62537936596395 8697600.0 2865632.2944353875 1417.215312405817 2815.5079541796495 100.0 511976.50005968224 22.423641392854883 18.94809437623502 8697600.0 2279470.653207942 1467.2450401918902 5772.272946674993 100.0 230739.19924995507 3.550321956067092 11.255678936789568 8697600.0 2758394.4628879796 1437.907710376446 5835.099295407095 100.0 171594.42484505594 3.469290910734682 12.594660308185057 8697600.0 3053944.2088322723 1405.7057500096732 3308.70682810629
7.0 100.0 275857.87146699906 17.706015266163526 19.2156239812874 9366700.0 2976201.417923421 1430.5337997338497 3095.001148024067 100.0 275786.6777636965 17.706015266163526 19.2156239812874 9366700.0 2976483.2255525156 1430.4479937004662 3095.001148024067 100.0 452426.3561794719 21.665052523721855 19.873833913117647 9366700.0 2431934.182957733 1476.89054976014 5772.453815137677 100.0 215320.8332549134 3.82877797281072 12.303329663306775 9366700.0 2853774.2401925684 1451.6181892073032 6302.197485121667 100.0 161254.79708285988 3.6921778027616323 13.483165592349422 9366700.0 3145388.2589178886 1419.012153405713 3563.652261771675
7.5 100.0 249069.7574765688 17.501796202827222 19.785410044754144 10035700.0 3080547.309528876 1442.5456254318926 3322.022732797954 100.0 248901.5890065339 17.501796202827222 19.785410044754144 10035700.0 3081367.631212646 1442.4506868924534 3322.022732797954 100.0 400851.30577793886 20.97096808117967 20.899666954652375 10035700.0 2572655.592645575 1484.7186792250238 5772.635382653114 100.0 201057.32310671895 4.129593787363002 13.312208743149245 10035700.0 2945441.936336318 1464.021715027377 6739.071812200225 100.0 152697.28764965208 3.9163063429313727 14.375917226196409 10035700.0 3227617.0738905994 1431.5321385950836 3822.515033152317
8.0 100.0 224759.57381539457 17.316148389548026 20.364842807236574 10704800.0 3178953.281173663 1454.7372887947968 3486.0241794992908 100.0 225071.80867964483 17.316148389548026 20.364842807236574 10704800.0 3178698.9152995795 1454.0438792918817 3486.0241794992908 100.0 352349.7490264949 20.17417106648746 22.129750795117403 10704800.0 2707136.4633806674 1493.9533915415584 5773.114889902123 100.0 188669.36620281453 4.430741395239606 14.29049817323743 10704800.0 3029733.102894854 1476.1511475955213 7237.238048925738 100.0 144918.28653192855 4.115172806254559 15.248469198061807 10704800.0 3305816.0015869318 1443.1144952520701 4095.0931264045075
8.5 100.0 205219.85708487488 17.133439478281637 20.868560553426725 11373800.0 3270099.399484421 1464.583476170569 3623.926262590889 100.0 205178.61817214516 17.133439478281637 20.868560553426725 11373800.0 3270101.283693878 1465.0174801811615 3623.926262590889 100.0 313941.7942308349 19.486320899114922 23.30399436493477 11373800.0 2831524.0336089744 1500.8045100986599 5773.882465320728 100.0 178424.9158092332 4.743936639645153 15.326179718605532 11373800.0 3106555.1480501164 1486.854726006638 7704.594388713074 100.0 138572.95532093022 4.348159363433925 16.117467482614458 11373800.0 3376662.0846183323 1454.4506097786416 4364.912260281141
9.0 100.0 187919.89914882343 16.940994001322903 21.383385319499652 12042900.0 3355652.2694607833 1474.9599832475135 3747.5804759798607 100.0 187944.42027229283 16.940994001322903 21.383385319499652 12042900.0 3356456.9922230607 1474.8208506439755 3747.5804759798607 100.0 280812.96992906416 18.822828330961332 24.379327086486626 12042900.0 2951607.458516727 1509.7828166988133 5912.242106883967 100.0 167719.23998758534 5.051278843771217 16.403646043539382 12042900.0 3185531.010948061 1500.0256343533895 8192.124081464974 100.0 132975.39620270388 4.540948381792152 16.91622011287402 12042900.0 3442378.966161175 1465.3583617934028 4651.606083257412
9.5 100.0 173532.24636497707 16.67949617388367 21.806244510108204 12711900.0 3438457.9326908947 1484.0322636099297 3823.6475048427174 100.0 173454.5888289866 16.67949617388367 21.806244510108204 12711900.0 3437411.055713136 1484.1963173701913 3823.6475048427174 100.0 250395.14722538 18.140108611933233 25.389906078057273 12711900.0 3067128.4932997786 1516.3883479978067 6346.993854320046 100.0 159727.08513570094 5.350161645971015 17.31572360898721 12711900.0 3255443.6418752484 1510.3881362710372 8638.563962645734 100.0 127693.40093835506 4.757808540300018 17.77280541145407 12711900.0 3504000.70082741 1476.1663514988275 4948.561817268883
10.0 100.0 163218.0799420094 16.462003252194602 22.320900406869566 13381000.0 3510127.8459574934 1493.0915919787817 4038.67468592283 100.0 163193.1974177558 16.462003252194602 22.320900406869566 13381000.0 3510405.4435213585 1492.7112760221694 4038.67468592283 100.0 221996.0526622848 17.523763537364715 26.420773252937867 13381000.0 3181148.83937864 1523.6466680803335 6712.653137258472 100.0 152125.9045842403 5.6828864465546225 18.491668234874467 13381000.0 3321334.288780966 1520.896570472372 9126.961220052212 100.0 122790.17087031748 4.94009228246066 18.55681787872468 13381000.0 3561570.3361832295 1486.6771410235847 5288.090112086165


==> data/stats/amazon_electronics_photo.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 1679951.7751106094 11.041856966310245 3.8145426097877015 823500.0 117368.18258814851 1054.9930326058482 804.4929646123026 100.0 1683970.3462632394 11.041856966310245 3.8145426097877015 823500.0 117735.0711631509 1055.0335926377988 804.4929646123026 100.0 1222567.5440955563 8.70447626564438 1.3313250934001102 823500.0 125275.92904525436 1069.314207490098 1403.5497807980926 100.0 957972.0593032769 0.1924298615533271 0.24641952043085794 823500.0 187801.34941046318 1063.4324116097605 818.4722627486542 100.0 965927.9263683731 0.2998305764841022 0.4758429033544463 823500.0 191990.709949521 1061.4184949606429 812.030159369732
1.2 100.0 1488394.7133369707 15.88923076923077 5.269901284326287 898400.0 184747.86977234544 1073.8333222008964 1115.1822510689865 100.0 1488538.520909519 15.88923076923077 5.269901284326287 898400.0 185318.3148735139 1073.5516311472843 1115.1822510689865 100.0 1052056.3273367686 18.66087632875292 1.8017085805795596 898400.0 170896.95504272226 1107.8006428635836 2341.731946139185 100.0 830392.4039109454 0.3565281651131183 0.49435312608898757 898400.0 268697.1014871639 1078.3353073578066 896.7147853856583 100.0 820129.6979080304 0.5547951873057547 0.9662041858085464 898400.0 281531.20264958334 1074.9699815665886 857.2751150285919
1.3 100.0 1321234.2470770017 17.18313561828399 6.498205280761712 973300.0 250216.45558374474 1089.9102832867388 1115.1822510689858 100.0 1321437.482248953 17.18313561828399 6.498205280761712 973300.0 250794.60186578194 1089.8577367668693 1115.1822510689858 100.0 965936.8212727171 25.186050301482965 2.20469564801348 973300.0 203590.28030097703 1145.8267828388246 3114.3190150857913 100.0 736697.3590451248 0.48872634645762136 0.7634906148012338 973300.0 338599.984013545 1092.7247624325603 949.8809545380961 100.0 718242.7454472226 0.7330908949009017 1.3158132570872112 973300.0 361705.6743443781 1087.416747971012 874.9996953357936
1.4 100.0 1170889.6692240075 17.30016313213703 7.044241320319856 1048100.0 313335.13965512894 1103.8805041138642 1115.1822510689851 100.0 1171492.0662723377 17.30016313213703 7.044241320319856 1048100.0 313805.32478835096 1103.513577907376 1115.1822510689851 100.0 898939.6209931627 29.919804905501106 2.669298299221729 1048100.0 234655.85890941788 1177.88541501596 3748.206074781926 100.0 671679.9993815352 0.6978208996568064 1.1225484248206592 1048100.0 400254.2115875577 1104.9762490847766 1001.4554767372734 100.0 639367.7405650653 0.9128284175205325 1.7699901446442912 1048100.0 432524.6348338549 1098.996626701074 943.1354916221986
1.5 100.0 1054154.6138417525 18.14447107155084 7.8189773912163325 1123000.0 370972.2835060123 1116.290372673923 1115.1822510689879 100.0 1054082.757676663 18.14447107155084 7.8189773912163325 1123000.0 371940.1061946971 1115.8443605380814 1115.1822510689879 100.0 847893.4355547772 31.935721934419586 3.1143922232076426 1123000.0 269515.47292571125 1201.3973769769066 4210.39648508277 100.0 616073.8028221353 0.8389732658534843 1.4283274527199408 1123000.0 455532.288041366 1116.7865483910514 1053.6534143038814 100.0 573931.0172778127 1.0468789238879272 2.209551729059236 1123000.0 499876.6058982358 1109.3333763956596 941.8616822323186
2.0 100.0 720661.8469415667 19.87486327872323 10.071573368564728 1497400.0 612220.7655796944 1167.5840637989443 1461.9473077521652 100.0 721422.8772563887 19.87486327872323 10.071573368564728 1497400.0 611278.762596182 1167.8805749439869 1461.9473077521652 100.0 742651.6021061279 29.957762206075124 4.656350159603572 1497400.0 378255.40596328443 1267.151671818136 5355.285878235883 100.0 442456.67830661876 1.4888855183544973 2.8681506968643595 1497400.0 684143.8403448759 1165.9650242495327 1377.775803002746 100.0 353764.07311464165 1.5539497437077479 4.254683143925713 1497400.0 785758.4328323188 1152.8984584764191 1128.9571387050862
2.5 100.0 544973.0175246259 19.671948722514017 11.9288251244456 1871700.0 801160.4426884706 1205.3601044882964 1563.8674535869632 100.0 545825.0216857065 19.671948722514017 11.9288251244456 1871700.0 801551.1596653964 1205.3413357268983 1563.8674535869632 100.0 656358.4548947224 30.174257433165696 6.583895271613119 1871700.0 467804.7172404231 1311.8078475342145 5942.7639733122005 100.0 350208.91442055156 2.024491871812277 4.231347691298272 1871700.0 853194.2860028862 1202.7956191755497 1735.3973957634719 100.0 269520.83726616285 2.119345049779665 5.719622810106134 1871700.0 972554.5338524225 1188.0264675185917 1319.257326001872
3.0 100.0 445428.80832109175 19.129648760330582 13.483844879311862 2246100.0 956133.553721299 1234.1366285312317 1567.0586790172024 100.0 446534.43321430124 19.129648760330582 13.483844879311862 2246100.0 957176.6232456052 1234.0147709531825 1567.0586790172024 100.0 597704.0894891698 29.904933312968783 9.0513062605358 2246100.0 564034.9616198082 1342.1819818893368 6016.7365923578 100.0 290527.7528211017 2.6741044041879047 5.612597440864735 2246100.0 989018.829841624 1234.0808651772254 2120.7877339525344 100.0 214311.88459188724 2.6245694057826294 7.0413420003572575 2246100.0 1127795.0244419135 1216.1215003731622 1465.5232896224281
3.5 100.0 371924.16705737985 19.17652255367111 14.96626724887211 2620400.0 1088726.2547235417 1259.2450215158956 1633.9809654970345 100.0 371585.4591098666 19.17652255367111 14.96626724887211 2620400.0 1088178.7419387386 1259.3785136103359 1633.9809654970345 100.0 543008.2307354553 29.75353524087042 11.719305651764907 2620400.0 675000.6944232084 1357.3924658676071 6035.458222018881 100.0 249704.10071545147 3.257379804328073 7.028212611124371 2620400.0 1103576.0650121188 1261.6800262942 2523.8090760539044 100.0 181584.85152507725 3.1722551964180306 8.459989527107801 2620400.0 1248678.9473924746 1241.2067239902867 1648.8714706312144
4.0 100.0 312078.2153901527 19.690914013081866 16.20748878270363 2994800.0 1202209.386494815 1281.9340522421585 1763.4239150320234 100.0 312151.6680818406 19.690914013081866 16.20748878270363 2994800.0 1202640.7544173528 1281.7694727129715 1763.4239150320234 100.0 496601.3974676095 29.377547114236958 13.303407054529043 2994800.0 784823.2432837663 1367.9354027680586 6035.458788117704 100.0 219918.1614516026 3.825232908402882 8.36427551737582 2994800.0 1201277.5974127708 1284.5437177291615 2902.028350471976 100.0 158111.1769373392 3.683056748897192 9.76602604747814 2994800.0 1352932.7106161357 1263.2146743915605 1822.0409444771847
4.5 100.0 268785.0160089431 20.43968324043927 17.41263893513177 3369100.0 1303532.8792742763 1302.1176737146536 2153.301195364701 100.0 268498.3566085736 20.43968324043927 17.41263893513177 3369100.0 1303599.5997205935 1301.8868726742085 2153.301195364701 100.0 464131.27808690007 29.526264371600064 14.836401297916375 3369100.0 869135.0875083777 1381.975148898311 6036.136993858236 100.0 195912.32361500137 4.4393824090996095 9.894920858202807 3369100.0 1288151.4576393017 1306.0444423136464 3302.423084556689 100.0 140338.55620136534 4.108798050765785 10.962673982970797 3369100.0 1443121.6818270308 1282.6223283861598 1996.3796199417552
5.0 100.0 234978.43030581385 20.85930509991053 18.37226731965837 3743500.0 1392845.6322569428 1320.302829699128 2432.6520090310773 100.0 234860.44367097292 20.85930509991053 18.37226731965837 3743500.0 1393640.8731683597 1320.6965576509997 2432.6520090310773 100.0 438043.51700958435 29.508219249197616 16.25844515863612 3743500.0 939430.7420595397 1396.7180205230254 6036.1371522206255 100.0 176568.36810092276 4.992715173968936 11.144313788606812 3743500.0 1365771.1723509007 1324.631627354712 3688.442464026212 100.0 127082.39326544912 4.549640975550512 12.180456819848825 3743500.0 1520821.1815274956 1301.001384806859 2213.5761529370307
5.5 100.0 205736.2315366725 21.401851030813564 19.410146624714013 4117800.0 1475624.2270887746 1337.3072933555927 2641.820521155568 100.0 205462.20998552354 21.401851030813564 19.410146624714013 4117800.0 1476102.1006361742 1336.2321968547567 2641.820521155568 100.0 413092.4823370135 29.56122578942462 18.208948985624314 4117800.0 1010845.6217010461 1408.30028766248 6036.137277899421 100.0 161051.3306665907 5.606852358483605 12.58280204338957 4117800.0 1436720.546048121 1341.954314755262 4063.8287446702975 100.0 117197.90840885774 5.066332164376869 13.363169322106957 4117800.0 1588908.8694916305 1316.944760581798 2410.7074969811047
6.0 100.0 181092.7686060857 21.901109969007862 20.493796596069007 4492200.0 1552733.5723324728 1352.3661971335466 2784.106197721389 100.0 180683.35526863343 21.901109969007862 20.493796596069007 4492200.0 1553575.2427757971 1352.3217896635435 2784.106197721389 100.0 376974.4556167072 29.31519683040296 20.384048518934865 4492200.0 1104335.157425249 1419.9858282804003 6036.155631637704 100.0 148250.72867519024 6.1877336508294505 13.926248654007162 4492200.0 1500268.2840528619 1357.9229505739042 4476.152466019298 100.0 108623.78512790622 5.470167656145038 14.462590308193985 4492200.0 1651298.592172373 1332.7692602783127 2634.531174411629
6.5 100.0 160176.50866160123 22.29725702301452 21.35807803822342 4866500.0 1622674.560941226 1366.085341837246 2857.3109760884176 100.0 160208.7399601701 22.29725702301452 21.35807803822342 4866500.0 1623004.9301965602 1366.8333259676876 2857.3109760884176 100.0 344039.0688493245 29.003998131427338 22.15647111983264 4866500.0 1194345.201758091 1426.9758915636587 6036.155636664923 100.0 136979.03064645984 6.743043048493716 15.339473622844096 4866500.0 1559651.3035198275 1372.5457516225538 4843.405384215355 100.0 101956.21257813789 6.008540463779137 15.598094142668906 4866500.0 1706687.4332509902 1347.0695032144602 2837.586251352413
7.0 100.0 144096.46851718085 22.634273646357965 22.253555651801662 5240900.0 1685265.6591694697 1378.8384551075428 3002.452395456829 100.0 144239.34633308952 22.634273646357965 22.253555651801662 5240900.0 1685207.5815907451 1378.975969425232 3002.452395456829 100.0 322559.6316913127 29.916924384185396 23.779647803481474 5240900.0 1258562.5507045425 1438.535584131265 6036.1556374881775 100.0 127387.60010510728 7.316289153759984 16.7701475703688 5240900.0 1614115.8280441125 1387.0525800949076 5243.639944242498 100.0 96148.31319185236 6.41461896712292 16.8598544296339 5240900.0 1757316.0239110733 1361.4194968996537 3091.264195999176
7.5 100.0 129453.90896437598 22.678631617897324 23.088873053971128 5615200.0 1745416.781444004 1390.9231682624227 3177.1505517202017 100.0 129304.9660436632 22.678631617897324 23.088873053971128 5615200.0 1745236.4472461813 1390.8849039501615 3177.1505517202017 100.0 284169.72249286907 32.4004747455929 25.808456679967374 5615200.0 1349437.3101494417 1454.0961720733094 7186.8964314064015 100.0 119412.70125177458 7.924044565512631 18.054092031171635 5615200.0 1663665.791597203 1401.417997127543 5644.360967477983 100.0 91170.41660969444 6.8897602495382655 17.92514581455999 5615200.0 1803302.8966937691 1374.370236771715 3313.163241657925
8.0 100.0 117287.71924387099 22.54968526872318 23.843196518232226 5989600.0 1802321.1831328834 1402.2565943837878 3290.74066985404 100.0 117328.71739840103 22.54968526872318 23.843196518232226 5989600.0 1801140.645797893 1402.1186148048614 3290.74066985404 100.0 244630.84538224622 32.54625067880196 27.554153296982207 5989600.0 1457232.5392574156 1460.8535526632654 7527.678266731573 100.0 111810.0329044585 8.5098426477722 19.605575348277167 5989600.0 1712546.320614118 1413.4862122898096 6031.1481065099415 100.0 86890.64897473995 7.332471389378754 19.085890716158666 5989600.0 1846169.0847381 1387.3409091554086 3571.903393088985
8.5 100.0 107531.43366744711 22.173678935982263 24.41100389715924 6363900.0 1852807.4470064323 1412.488300271359 3371.693482529507 100.0 107370.51169230053 22.173678935982263 24.41100389715924 6363900.0 1852723.868944109 1413.2651855446952 3371.693482529507 100.0 218673.18163456957 31.815945968347272 28.62143233128575 6363900.0 1544236.7683655724 1465.1154366691317 7547.600056290341 100.0 105656.03325577988 9.128568215285378 20.956849404151686 6363900.0 1756484.02138268 1425.6263288516257 6438.635462867925 100.0 83316.47082871539 7.7937758103162045 20.2225634054736 6363900.0 1885656.9171975954 1399.9192368709728 3828.990872128803
9.0 100.0 100734.07940560553 21.92323427573574 25.152763690346173 6738300.0 1898402.4581012363 1423.6451075631435 3431.4108780154947 100.0 100581.94912478696 21.92323427573574 25.152763690346173 6738300.0 1898030.6780081468 1423.4138766064855 3431.4108780154947 100.0 198251.95385526516 30.910472772490145 29.485728849675024 6738300.0 1616728.1342159705 1470.476404630525 7552.503408124914 100.0 100349.11156788789 9.689299118293324 22.279608756566148 6738300.0 1799197.3126793418 1438.5902435720152 6816.522182726314 100.0 80151.80129908826 8.225280204588532 21.375321081228673 6738300.0 1921309.2939803014 1411.5056789982286 4116.2481502066075
9.5 100.0 95049.63748451667 21.648722039664843 25.882584116423136 7112600.0 1938668.630318757 1432.759473461636 3537.201836088296 100.0 95052.04967244045 21.646531060757003 25.882094088418565 7112600.0 1938577.0593646811 1432.9543968596774 3537.201832110141 100.0 184430.47952190766 29.904888187276583 30.38035506294254 7112600.0 1674438.4455322302 1477.0273879353506 7556.029541781798 100.0 95132.08516270391 10.30060007348326 23.7585451291163 7112600.0 1838861.1394043132 1448.5756924425782 7225.740096717837 100.0 77459.28651437738 8.678455188125678 22.51170475401662 7112600.0 1955500.134505076 1422.5713598216075 4406.239077693878
10.0 100.0 90860.38287798896 21.208474788991712 26.455478263394262 7487000.0 1975206.7654190182 1443.4226449843209 3665.825596716364 100.0 90805.84160319105 21.208999663077172 26.456733913828145 7487000.0 1975084.5382754742 1443.3826271941903 3665.4519990232084 100.0 170957.09779946363 28.83688925842106 31.380541963558656 7487000.0 1726610.9891397743 1483.2338472840818 7557.626266627304 100.0 90187.66230573988 10.817123529388754 25.024391821212678 7487000.0 1877484.3615712398 1459.1726394315378 7639.605057946203 100.0 74755.20049195488 9.20149982253372 23.618173647052547 7487000.0 1985582.1895501032 1433.1058723957478 4692.646424576868


==> data/stats/arxiv.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 24998155.853934266 7.924223793421457 4.883037163586108 18627700.0 4120450.3353982945 1361.00055724913 807.1031755475648 100.0 25004204.482351135 7.924223793421457 4.883037163586108 18627700.0 4116525.6816500346 1360.9585835552582 807.1031755475648 100.0 22649334.04659702 10.45380096136728 2.982543810248248 18627700.0 3779823.218806955 1375.2396290023248 2082.075890164699 100.0 12805689.24617193 0.046225585848699485 0.3295035466413354 18627700.0 7081607.801154957 1409.411159753438 3649.4855956881997 100.0 12854853.08691928 0.09717776707773898 0.734797305712364 18627700.0 7126421.447635608 1404.592950904112 3566.3371008183935
1.2 100.0 22348420.685880773 10.483105421145805 6.473960398682796 20321100.0 5744425.100648059 1377.6831952854086 807.1031756115565 100.0 22356430.52458638 10.483105421145805 6.473960398682796 20321100.0 5743505.03567847 1377.6689925712271 807.1031756115565 100.0 21278527.903798115 14.211678224057717 4.541831337736486 20321100.0 4865327.613507854 1396.687070096133 2117.7332339620284 100.0 11527986.212493502 0.0838542485846119 0.6770708416984392 20321100.0 8671311.683794953 1428.5488418439404 3935.313532449466 100.0 11576861.294676896 0.17150073189828052 1.4573505445258905 20321100.0 8789327.448543373 1419.4510802848115 3769.7282178264204
1.3 100.0 20294857.87270512 11.997426170708758 7.691464069605924 22014500.0 7207547.151438641 1392.8206696639654 807.103175611565 100.0 20291849.959394827 11.997426170708758 7.691464069605924 22014500.0 7203274.553938635 1392.7873261064458 807.103175611565 100.0 18586216.28224059 15.541005781812883 5.857702535403041 22014500.0 6254328.806107466 1414.4605158358204 2216.924619688905 100.0 10555078.17532701 0.11614895987676571 1.041142576666347 22014500.0 10037770.367984816 1444.6660937367747 4167.694075726362 100.0 10491847.33942919 0.23118941852413202 2.17619750515416 22014500.0 10343766.66411295 1433.3421544094729 3936.5678325300005
1.4 100.0 18580404.53690074 12.64657213411064 8.5508158183258 23708000.0 8543092.589533199 1406.7862203781142 887.1206934333898 100.0 18590849.15395049 12.64657213411064 8.5508158183258 23708000.0 8544190.364270432 1406.7619061809094 887.1206934333898 100.0 17256322.06107495 15.906015800869328 6.904940082921908 23708000.0 7340928.461261104 1429.6712595697195 2442.9897187272336 100.0 9716583.114765959 0.1459663428243109 1.4020688987970273 23708000.0 11325570.629943267 1460.146588000334 4414.457201788919 100.0 9613570.597388087 0.280338513688753 2.865866233637333 23708000.0 11736693.109935239 1445.3570825577856 4119.920060212678
1.5 100.0 17173152.09120634 13.21535822667898 9.388748067834982 25401400.0 9770012.84728541 1419.6393591154006 957.5716098525813 100.0 17170066.54281575 13.21535822667898 9.388748067834982 25401400.0 9769285.838319942 1419.6023685399723 957.5716098525813 100.0 15915521.051468968 16.135798373083315 7.807757323982453 25401400.0 8407071.144911472 1444.3411613967892 2562.173558069653 100.0 9044465.619133888 0.17654077588753422 1.791006839511707 25401400.0 12468371.406167889 1473.7533353986078 4670.684664762938 100.0 8854320.413844008 0.3178293924086129 3.4947408022943987 25401400.0 13045432.194461552 1456.40403205103 4312.654671467139
2.0 100.0 12174352.037178194 13.400095082754099 12.13806823666726 33868600.0 14961416.059564644 1470.500354929587 1267.1803855178464 100.0 12172790.164821612 13.400095082754099 12.13806823666726 33868600.0 14955927.183303433 1470.5473106856903 1267.1803855178464 100.0 11444733.898103034 14.592242585904398 10.916686980944794 33868600.0 12822812.444146749 1507.097486781463 3904.0783612878863 100.0 6712251.763365837 0.31270224449419387 3.7141494541468263 33868600.0 17242026.20069385 1530.9746741831073 5828.648841588214 100.0 6310307.528295242 0.4524060794522557 6.509173799101233 33868600.0 18442438.09124986 1505.2587817974177 5123.477590249067
2.5 100.0 9322529.96435368 12.473474214149846 13.747898865151104 42335700.0 18971804.78461396 1508.6340232729797 1614.6784187554936 100.0 9323035.2116443 12.473474214149846 13.747898865151104 42335700.0 18968147.364978846 1508.700455489522 1614.6784187554936 100.0 8564712.069936693 12.319277272591814 13.54957158569669 42335700.0 16749044.242950732 1554.4599295912212 4393.284568293689 100.0 5417364.588383177 0.4481740457520895 5.635947923700604 42335700.0 20790158.887778983 1573.3349328345212 7002.50937578114 100.0 4982363.908220399 0.5464757580430329 8.73616553285141 42335700.0 22305255.969375886 1543.9727033003294 5935.557989281183
3.0 100.0 7658718.879894064 11.545783077064726 14.904880047449836 50802900.0 22084980.174055096 1540.3861827410367 1977.0796322329272 100.0 7658629.485134887 11.545783077064726 14.904880047449836 50802900.0 22083370.08506622 1540.464849113982 1977.0796322329272 100.0 6964923.042915588 10.85628131302154 16.103385127186982 50802900.0 20241907.833044343 1581.0470006673324 4533.23942845921 100.0 4560767.952168105 0.5815189512500819 7.634880901955933 50802900.0 23677605.182271563 1607.433800355302 8196.198737371365 100.0 4157260.744377527 0.6177488784453664 10.608499138208638 50802900.0 25317781.14220916 1576.8779307803409 6709.445712107349
3.5 100.0 6553473.002592659 10.484013070438888 15.725707724749514 59270000.0 24481056.591477636 1568.231725985298 2187.77925883031 100.0 6552965.084568677 10.484013070438888 15.725707724749514 59270000.0 24479966.437539667 1568.274480275364 2187.77925883031 100.0 5963462.64603398 9.488212901049243 17.20415308025651 59270000.0 23055354.728613414 1601.9802075676143 4537.343428619347 100.0 3942952.0610320573 0.7181066923498793 9.629398274105242 59270000.0 26127147.580551155 1636.553284721681 9448.092576070543 100.0 3597526.563344785 0.6731882630557313 12.197200017211184 59270000.0 27762257.286173284 1605.401330862489 7547.330079881969
4.0 100.0 5950743.748501704 9.453363917425081 16.416751577360156 67737200.0 26177898.915790565 1594.5894699395415 2312.9379952324234 100.0 5949912.199576512 9.453363917425081 16.416751577360156 67737200.0 26173037.523228135 1594.6119408903542 2312.9379952324234 100.0 5240205.804204194 8.152012716207922 18.076102063630724 67737200.0 25328248.84200998 1625.094426623983 4566.850366050755 100.0 3476864.9592850567 0.8505956853854666 11.555328147334938 67737200.0 28255030.41992856 1662.4505245154517 10709.460164145048 100.0 3189992.316914989 0.7206453163056239 13.617762200133694 67737200.0 29788038.55300674 1631.124140639667 8479.470753236566
4.5 100.0 5398528.809181779 8.455334942902393 17.079107950746604 76204300.0 27529261.50518816 1619.6600037398575 3205.5157083611275 100.0 5399978.982951741 8.455334942902393 17.079107950746604 76204300.0 27535796.40561667 1619.6547808380196 3205.5157083611275 100.0 4416134.4379663365 7.0758110716800795 18.819569568993526 76204300.0 27642201.00616513 1646.2856451096452 5413.785677856324 100.0 3110550.8023526412 0.9863662128656174 13.481695309485167 76204300.0 30141306.01747036 1685.5162307209937 11975.34758129503 100.0 2886800.6028650473 0.7732008714021021 14.910830915443535 76204300.0 31504476.88229432 1655.707848978549 9476.327714315179
5.0 100.0 4858788.180979165 7.412792517439956 17.73792137630596 84671500.0 28735093.274977606 1646.144144412401 3727.514298615636 100.0 4857831.476503067 7.412792517439956 17.73792137630596 84671500.0 28743970.023344334 1646.1394360474135 3727.514298615636 100.0 3750681.5852027116 6.127611846069638 19.49135412784813 84671500.0 29744909.948885232 1666.6470850415635 6140.838748172347 100.0 2816362.1842701873 1.1223739567682876 15.461612724802404 84671500.0 31817621.53566043 1707.1017111179008 13250.2581995968 100.0 2645580.1199905872 0.8303307081989595 16.119661281704172 84671500.0 32983759.93810712 1678.6332917901887 10565.955117975158
5.5 100.0 4398276.958838866 6.2278724918994754 18.43119707447778 93138600.0 29823074.08681303 1673.2276262705086 4130.322317462146 100.0 4398773.618047015 6.2278724918994754 18.431180671214715 93138600.0 29825315.64562061 1673.2063923308947 4130.321997144994 100.0 3341225.460839925 5.4752140407290195 20.00392736084777 93138600.0 31372213.27285968 1686.2174045112035 6688.199895535472 100.0 2569728.8984303162 1.2601519937504904 17.435917856538595 93138600.0 33358160.449412353 1724.9870995502797 14559.015907778195 100.0 2456020.762867664 0.8964811691383308 17.263806715105275 93138600.0 34254130.960628435 1700.14556297459 11840.201863268849
6.0 100.0 3714446.8137567695 4.798288386581005 19.15511851730121 101605800.0 31288625.88131755 1701.3269799879524 5704.669427190943 100.0 3715810.189337883 4.798301898603315 19.155554381325594 101605800.0 31285183.854687527 1701.3383814900735 5704.664559902877 100.0 2955961.4928129646 4.626457780782702 20.549711004606902 101605800.0 32899285.0366994 1710.125700094834 7978.146721744206 100.0 2367282.7947222795 1.3899039302012761 19.362553714121493 101605800.0 34752712.2174488 1744.224762319135 15834.342621337935 100.0 2302567.8249136684 0.9901423288092509 18.445296279053373 101605800.0 35346408.45863387 1722.8272886117466 13319.495659318176
6.5 100.0 2779939.381867214 2.969421481821676 20.043461189583347 110072900.0 33856720.3839879 1733.78941185536 9103.035679204206 100.0 2780318.556642895 2.9694173217453006 20.04346813560357 110072900.0 33858653.58725799 1733.9464613137675 9103.022945700282 100.0 2566542.667822286 3.341234122465788 21.221671413196525 110072900.0 34543035.441089414 1739.7852628387247 10502.154182370972 100.0 2192025.772882377 1.5280840802754354 21.307661035986957 110072900.0 36045516.27185689 1760.9085106667635 17151.349490266162 100.0 2178312.8969294475 1.1404358496393494 19.805544552204353 110072900.0 36276895.90132902 1747.7549455716478 15221.735896719832


==> data/stats/cifar10_100.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 2789259.9584494233 9.658034053512662 2.0402343908332177 1580000.0 221989.15373059653 1124.4314974925342 1305.6291127614454 100.0 2786415.288359338 9.658034053512662 2.0402343908332177 1580000.0 222986.44511866727 1124.4067467297161 1305.6291127614454 100.0 2256869.2015340026 17.9617968832448 1.505560153745652 1580000.0 237264.97761012593 1140.208169901712 2299.8096809276626 100.0 1996837.3920178048 0.016422505148189808 0.015568432078457142 1580000.0 289065.9041363197 1134.6734053356777 614.6413817001703 100.0 1944707.6865456803 0.08951393911729172 0.1630461959028963 1580000.0 315167.5401207736 1132.7164541968812 630.685064411619
1.2 100.0 2265421.5468190853 18.80810710301227 2.961994548747631 1723600.0 341962.59124630596 1151.9925891625057 2307.546671444649 100.0 2266671.3856340274 18.80810710301227 2.961994548747631 1723600.0 341981.4608255791 1152.2582590903414 2307.546671444649 100.0 1959265.5608541062 18.64966745380099 2.3822117903817808 1723600.0 332173.1446953849 1166.1850717925706 2304.653058749293 100.0 1760659.6986685866 0.035908038072681156 0.03396926886689426 1723600.0 417103.9925695806 1150.0515669549902 619.2453282175447 100.0 1673210.5501878748 0.1399246470932485 0.28393215353122425 1723600.0 473711.881856663 1146.3513780716728 630.2967074968518
1.3 100.0 2022387.128728942 18.031420251737742 3.6470394335356247 1867300.0 446634.6139750168 1168.7785859204066 2307.866559762676 100.0 2021602.8615341967 18.031420251737742 3.6470394335356247 1867300.0 445752.35164053977 1168.5589725296666 2307.866559762676 100.0 1793674.5103890186 18.61184693809407 2.9881502156880577 1867300.0 410973.44914586167 1189.0025614407489 2540.815984155656 100.0 1601514.7255503489 0.054291351234667294 0.05719463098961729 1867300.0 525157.8906275753 1164.2110660590886 645.8969727182829 100.0 1459571.5521878712 0.1838923624753719 0.4186751525710266 1867300.0 619405.9040409619 1158.9196215881984 657.706402258379
1.4 100.0 1820166.0100512959 17.401747129847728 4.166025280348216 2010900.0 545737.8547480959 1183.776951211726 2307.8932408144747 100.0 1821136.13608323 17.401747129847728 4.166025280348216 2010900.0 544887.4706054191 1184.464318011516 2307.8932408144747 100.0 1665371.637177763 18.93640983085371 3.5338910153179954 2010900.0 480101.5460298649 1211.852344301832 2952.868602151029 100.0 1489890.9342962871 0.08391279150138581 0.07550465865822231 2010900.0 616265.2773371984 1177.4498181925853 697.4514323847205 100.0 1308473.240269011 0.21516469340619954 0.5509622375065337 2010900.0 748186.8594445277 1170.3489051479814 688.3213886719077
1.5 100.0 1654039.9579661628 16.752935140192555 4.511728747532618 2154600.0 639019.0933238928 1197.8714464084035 2308.0250713448604 100.0 1655640.4922575785 16.752935140192555 4.511728747532618 2154600.0 638847.2639639792 1198.1587822042368 2308.0250713448604 100.0 1584924.6380184267 19.536239072478146 3.940549539109977 2154600.0 537491.8347145212 1231.5422669338136 3344.331474965492 100.0 1408151.9083311413 0.10776241423938603 0.10165205759109 2154600.0 696988.6333914537 1189.2642076861766 766.5344780767261 100.0 1187912.19124994 0.2563894746594628 0.6969947196120717 2154600.0 866687.0121524977 1180.9970105415764 717.6727402218181
2.0 100.0 1243638.6445996298 15.464898467876148 5.956485867948648 2872800.0 1015168.5993303722 1249.8928454437184 2357.8134222089197 100.0 1243964.6139974047 15.464898467876148 5.956485867948648 2872800.0 1014280.135479758 1249.1281613896404 2357.8134222089197 100.0 1290507.9221438696 20.63931376887758 5.827414540722129 2872800.0 801354.8431999234 1301.2361195263315 4809.949296424758 100.0 1166815.199258333 0.22167307561873126 0.2135148389435421 2872800.0 1002482.4591427161 1239.4391330420867 1152.3024348308643 100.0 774825.1372784283 0.36492261732053777 1.419312552531921 2872800.0 1382856.0627237146 1224.2604614726106 800.157425873343
2.5 100.0 1006192.3722613106 14.432141566013776 6.957751725398078 3591000.0 1322802.2557030194 1287.1534874060699 2668.4752007802854 100.0 1005942.6765930906 14.432141566013776 6.957751725398078 3591000.0 1321430.0433350776 1287.6942763319648 2668.4752007802854 100.0 1130099.9114958108 20.56073445186723 6.92559291320857 3591000.0 1009513.0287952058 1348.791127627326 5890.82045854169 100.0 1038878.4863708188 0.3605670717811525 0.3763883307095375 3591000.0 1223195.2743787921 1277.4987936632251 1545.563096023572 100.0 623869.7799428186 0.46754019500217603 1.898144692328445 3591000.0 1709606.318720075 1258.7500386664897 934.7021309988776
3.0 100.0 856924.0795550616 13.803436744502513 7.602391927557886 4309200.0 1575061.7571399286 1317.8093621181258 2926.263477504441 100.0 856834.9226228382 13.803436744502513 7.602391927557886 4309200.0 1574024.1335386657 1317.8696334335323 2926.263477504441 100.0 1022505.6591459375 20.43721808197686 7.933352516904855 4309200.0 1182877.736255845 1383.7936421670197 6784.463921861038 100.0 951946.1049063192 0.48219899056149085 0.47616634592237683 4309200.0 1400897.5527440405 1308.044581989986 1939.7888275225291 100.0 517915.4488734278 0.540905857992023 2.2495619044963173 4309200.0 1986583.9025697194 1286.7293553455884 1085.453896017865
3.5 100.0 748162.7892579191 13.493203589999322 8.137540027654454 5027400.0 1792960.5837613512 1342.4670987550708 3281.720802523667 100.0 747658.0982579888 13.493203589999322 8.137540027654454 5027400.0 1791689.492476295 1341.7124091265753 3281.720802523667 100.0 934041.8940584079 20.23426359442592 8.651028508410995 5027400.0 1335637.470033142 1415.618331051083 7528.790905181849 100.0 883590.3052782122 0.6053109578067597 0.6175226955654417 5027400.0 1550427.8327735898 1334.0877018038416 2332.349344093406 100.0 458979.17616528366 0.6122305286636065 2.6254550948262936 5027400.0 2196600.9591884366 1310.979929943423 1261.6717358510289
4.0 100.0 671190.7946485155 13.194291442672073 8.64430333372637 5745600.0 1975388.826425719 1364.582443186696 3610.529267784854 100.0 671059.6306469884 13.194291442672073 8.64430333372637 5745600.0 1976024.5799423784 1364.878290672004 3610.529267784854 100.0 849582.066723004 20.21712908038213 9.38596420791633 5745600.0 1482043.9449448385 1437.9279997273204 8255.72969488523 100.0 832557.3012039878 0.7295985642189494 0.7763844249974318 5745600.0 1676737.2422786118 1355.9913004821117 2727.9280979991017 100.0 414035.2700408209 0.6839631972301329 2.9314612322234432 5745600.0 2381370.1098532225 1331.6885226053878 1437.1183670617688
4.5 100.0 612354.3239485088 12.971743090307688 9.00471263228386 6463800.0 2137338.3063975936 1384.862024050924 3914.2515876469565 100.0 612215.8020444429 12.971743090307688 9.00471263228386 6463800.0 2137240.393890668 1384.7603857603665 3914.2515876469565 100.0 786795.7878408132 20.26639382926522 9.933548126566972 6463800.0 1611222.0016204435 1460.2151885349144 8945.75951885391 100.0 788376.7181874325 0.8624165748835112 0.9547939834048733 6463800.0 1792886.1704546402 1375.2342849868967 3119.1005037191244 100.0 378660.1153687745 0.7411744525047714 3.1913249017792125 6463800.0 2540388.521960588 1350.0719310251502 1618.8634118123193
5.0 100.0 561469.905322388 12.920162069310088 9.40232807685597 7182000.0 2284606.390218948 1403.1834285006298 4228.195907724692 100.0 561555.2224136909 12.920162069310088 9.40232807685597 7182000.0 2283939.1182618514 1402.6510710145792 4228.195907724692 100.0 732122.7930368031 20.35428753404835 10.563420330291313 7182000.0 1732653.630924089 1485.1861108089324 9572.136801248607 100.0 752115.7272252805 0.9880485331864266 1.0682101263408292 7182000.0 1892492.8504102735 1393.0372776550973 3518.6986312881386 100.0 354627.56007435673 0.8045939176541154 3.484456648674598 7182000.0 2673881.7604166884 1366.8165496730765 1808.7151586795435
5.5 100.0 520880.1631629559 12.813172638642694 9.787048857143022 7900200.0 2415342.4683006634 1418.8092150554478 4511.82388369265 100.0 520770.1951024737 12.813172638642694 9.787048857143022 7900200.0 2415840.904382839 1418.777422705899 4511.82388369265 100.0 687608.0504622184 20.423480037337686 11.095637315951649 7900200.0 1842809.1339292284 1497.321495815434 10180.04379155892 100.0 720352.328330856 1.1044368218937217 1.2546934626435369 7900200.0 1986464.5943648363 1408.340430727161 3903.373248554131 100.0 334906.6603966786 0.8875080768842725 3.7872679937105898 7900200.0 2796147.513575986 1381.8035992545044 1991.3105091768089
6.0 100.0 487248.2108148822 12.759935512365278 10.115381205872746 8618400.0 2536151.5797627647 1434.5209108136312 4791.94867227855 100.0 486410.3398602715 12.759935512365278 10.115381205872746 8618400.0 2534073.136677992 1433.5166269716926 4791.94867227855 100.0 645074.5778311503 20.5380325425236 11.558395381139611 8618400.0 1951244.3961343248 1510.388718711167 10778.064127929414 100.0 687448.0382605958 1.2414284666956426 1.4248205739547732 8618400.0 2073969.075213631 1422.808640539111 4298.479441023453 100.0 317811.2288889597 0.9413024262298268 4.056891553042682 8618400.0 2905565.1816904303 1395.5243755152737 2184.1029660968766
6.5 100.0 458448.70039773185 12.727097406667347 10.472971619989323 9336600.0 2644705.045274019 1447.263518499218 5078.755055373931 100.0 458434.0639332925 12.727097406667347 10.472971619989323 9336600.0 2644621.353043958 1447.9785271506034 5078.755055373931 100.0 610306.8428412635 20.817309105067512 12.013088684513765 9336600.0 2047540.557144043 1525.8388061140895 11409.99181919831 100.0 665433.1220994252 1.372269542013256 1.5702234363214207 9336600.0 2150909.750142941 1436.4268265579815 4702.317625722894 100.0 303780.29238391464 1.0170749799337468 4.29638577154828 9336600.0 3005219.025081866 1408.369099738754 2376.131466402526
7.0 100.0 433139.23580735456 12.74342823840299 10.730201861866698 10054800.0 2746613.795636441 1461.2341150012915 5349.845783243916 100.0 432687.1797248849 12.74342823840299 10.730201861866698 10054800.0 2747111.4054359817 1460.1934527680032 5349.845783243916 100.0 580328.4527523605 20.996483334215828 12.474595462899222 10054800.0 2138116.232992544 1543.68988718989 11995.577140345173 100.0 640601.4806162064 1.5016698271980589 1.7382314043449147 10054800.0 2226259.583904868 1448.8534166306497 5094.657852131154 100.0 292683.852232561 1.079281544369078 4.557487981270845 10054800.0 3094366.135428623 1420.1519861813276 2571.1631771258503
7.5 100.0 412369.82936119294 12.705632979241791 10.970863056653716 10773000.0 2841455.476607356 1472.7541204232427 5611.432697585258 100.0 412057.92680314137 12.705632979241791 10.970863056653716 10773000.0 2841195.183198739 1472.8289047082735 5611.432697585258 100.0 552448.1000859285 21.177917103239537 12.809846427508226 10773000.0 2223905.4033803074 1552.9363822043426 12571.86842726323 100.0 621159.0670260368 1.63504263850756 1.8684087772633942 10773000.0 2294359.0714827552 1459.801862958134 5491.942874079338 100.0 282093.9287285083 1.1394784364869284 4.7961695942069875 10773000.0 3176728.1436849474 1431.2316559599833 2768.6285311348997
8.0 100.0 392922.5036408907 12.711072274011654 11.283861023166358 11491200.0 2930304.0487903566 1484.6450383814931 5872.542994285223 100.0 393150.8614633861 12.711072274011654 11.283861023166358 11491200.0 2930593.8097771285 1484.1312752024096 5872.542994285223 100.0 524028.1195546683 21.31715472949102 13.201435181076409 11491200.0 2311952.4676799416 1566.6787003405839 13117.928492717425 100.0 598767.0403597391 1.7630584323088616 2.072672158299856 11491200.0 2362108.6758142947 1471.0015522891479 5892.436380541953 100.0 273434.55955341674 1.2078983624274462 5.011736668700744 11491200.0 3254664.3180411737 1441.6515159096184 2969.413802282145
8.5 100.0 376232.44906855363 12.726502484236185 11.49605733576659 12209400.0 3014086.5783728757 1495.572916578475 6126.980921705917 100.0 376242.8418649973 12.726502484236185 11.49605733576659 12209400.0 3013664.6809459818 1494.6927596532619 6126.980921705917 100.0 498409.3855295801 21.602453092440182 13.638023669511302 12209400.0 2392276.448738178 1576.8265497462853 13710.371687450272 100.0 579742.7087568651 1.8818317297112659 2.2006862355642487 12209400.0 2426473.9096961804 1480.3193051128433 6275.26620440551 100.0 265010.1556786559 1.2699965568924276 5.303251871523527 12209400.0 3327004.7043297514 1451.1876642913355 3170.1482668331287
9.0 100.0 361627.5165244133 12.76392227810928 11.753201500036809 12927600.0 3089527.1754635605 1505.9373989599333 6374.498060672609 100.0 361668.6523434632 12.76392227810928 11.753201500036809 12927600.0 3090508.034184774 1506.0945740436762 6374.498060672609 100.0 477446.01549724094 21.818589246309124 14.011931750982502 12927600.0 2468360.9984807298 1584.5855808697686 14281.999123942722 100.0 564332.2446423157 2.010356853800638 2.4274693838889907 12927600.0 2484132.5735159055 1490.0835681074052 6671.432907593629 100.0 259044.94640540789 1.3359573515823877 5.522432980206604 12927600.0 3391762.6998344595 1460.896321493927 3373.0434323165327
9.5 100.0 348063.902831994 12.840816778829556 11.986297428561992 13645800.0 3162879.6909942515 1516.6076846057053 6638.404737532344 100.0 348028.3987536552 12.840816778829556 11.986297428561992 13645800.0 3163285.3826357974 1515.454731846037 6638.404737532344 100.0 456834.89462445606 22.06346853197631 14.37862619287356 13645800.0 2540479.143788093 1598.929317730872 14866.25337038842 100.0 546369.7116761324 2.140827062744472 2.5630155314492744 13645800.0 2543028.220563504 1501.365955153225 7065.5497402517685 100.0 251205.0982420225 1.3929175087816645 5.760158734046583 13645800.0 3454922.808114654 1469.5218643759542 3581.60520439519
10.0 100.0 333874.0488610367 12.889922362152612 12.270957290046818 14364000.0 3233257.8888971144 1524.7532225252673 6892.444450505434 100.0 333889.31853545876 12.889922362152612 12.270957290046818 14364000.0 3234492.0832784264 1525.0795076662362 6892.444450505434 100.0 438115.4131356452 22.33232309886022 14.755691360196149 14364000.0 2609651.881757133 1604.5430238714982 15440.544507760547 100.0 531901.8579737955 2.2704279266065117 2.6992541011966105 14364000.0 2595777.7186468 1508.9080542852842 7465.1966352454365 100.0 245208.3567239989 1.4586080355339042 5.958156474627764 14364000.0 3513529.2066781693 1478.0067248367782 3787.7397345452423


==> data/stats/cora.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 586431.3155488624 9.98972250770812 8.507042253521126 273300.0 47953.033244332175 933.7202415472439 390.3538466432175 100.0 588962.3707744491 9.98972250770812 8.507042253521126 273300.0 47691.25573201788 933.6583707708744 390.3538466432175 100.0 507480.5106109621 9.293275217932752 4.72051545592793 273300.0 43726.974004876625 943.3914877107096 662.6809841266935 100.0 353469.9120401287 1.3629944584173916 2.328646457693366 273300.0 57168.30502060032 955.6569644088253 859.855634506272 100.0 351090.12754265906 1.315598347529737 2.418629461926606 273300.0 58184.492593351 954.8774774237197 860.4398697749951
1.2 100.0 480337.9613107528 12.369621903520207 10.90629491233113 298200.0 79444.45249257251 949.1034954709438 393.2943045147661 100.0 482116.3147509242 12.369621903520207 10.90629491233113 298200.0 79433.57222639691 948.944021598761 393.2943045147661 100.0 435303.9738171579 14.587593728698023 8.528272344912121 298200.0 67080.72411881281 963.00912078101 774.092409568941 100.0 302544.2662329934 2.323794562493429 4.345147694904446 298200.0 84428.79853250048 970.9460429410955 936.6392697696925 100.0 301546.6867358578 2.2634151328199894 4.630122280545753 298200.0 87385.97240329355 969.0581200073378 895.8081437556581
1.3 100.0 399697.16632076923 13.35440537337021 12.844527482354446 323000.0 107831.95380547736 963.186098919213 411.8371781553618 100.0 402267.6746084414 13.35440537337021 12.844527482354446 323000.0 107820.75082157974 963.0458039823278 411.8371781553618 100.0 377099.7769406492 15.522966242390707 10.901174191890625 323000.0 91568.87027154145 977.0034587316941 818.3519741673994 100.0 268867.17755134316 3.4876712732761903 7.189608374862855 323000.0 108777.04016502091 984.936864244162 990.5279378071438 100.0 263013.42715960374 3.250710383282652 7.114447911790298 323000.0 112641.71676520807 982.5443005202923 955.503758761375
1.4 100.0 336246.6164041971 13.713917802339306 14.18156558398007 347900.0 133277.472095239 976.5823718434038 465.18074550851054 100.0 337360.87180012884 13.713917802339306 14.18156558398007 347900.0 132870.25960948225 976.4712306598934 465.18074550851054 100.0 331443.5262144359 15.721707702733228 13.122124142408136 347900.0 114561.25063210343 990.6412740721967 821.2795767161032 100.0 241173.91719678027 4.439917085247828 9.640884407728652 347900.0 130322.13840697272 998.1383648906249 1055.3071466453998 100.0 234489.24459817872 3.95110544942057 9.16277279437313 347900.0 135549.33556529458 995.2718714816879 1008.5606549620851
1.5 100.0 290038.9495684895 14.044452222611131 15.500895706127096 372700.0 154529.76850961242 989.3216290246465 490.6834506130055 100.0 289736.80068207986 14.044452222611131 15.500895706127096 372700.0 154439.0322272415 989.7401124687526 490.6834506130055 100.0 289244.6979917404 15.268352868599628 15.215284985583915 372700.0 136017.69974509155 1003.2933502239779 826.2769324645827 100.0 217770.27861724028 5.22609625415228 12.005378309284058 372700.0 150862.17374860868 1010.052722043233 1127.0842999777403 100.0 211898.32280705715 4.874537692546656 11.901402124707298 372700.0 156704.84780673397 1005.6294567469422 1052.444197684137
2.0 100.0 151711.01155301306 9.91848168992757 21.76612408440148 497000.0 233159.8847967939 1056.1797445854784 1035.8878484442728 100.0 151778.02301674025 9.91848168992757 21.76612408440148 497000.0 233483.30298153954 1055.4423952109748 1035.8878484442728 100.0 152831.86371816587 10.612512283000328 22.503219483747788 497000.0 232710.5941879288 1056.1108296265336 1166.9111164090882 100.0 150368.0736242109 8.740098962045526 22.90081207391839 497000.0 231846.9633773716 1061.4819999525123 1413.2193806156213 100.0 149925.72846031075 8.335832954633563 22.190254197469123 497000.0 233752.0644895844 1059.5206082222073 1372.7567261375048


==> data/stats/cora_full.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 3622451.063615098 9.452351870777974 6.837609760216143 2068000.0 389885.6081406146 1139.072936289274 609.7166161156808 100.0 3628399.9710281137 9.452351870777974 6.837609760216143 2068000.0 392378.40764729324 1139.0427188613603 609.7166161156808 100.0 3149226.6019756375 9.557361213705326 3.9498444675848567 2068000.0 366835.8301385711 1149.5190275833995 886.6888236180495 100.0 2281243.035550219 0.7574596264545426 1.0838100451960633 2068000.0 483708.6153778966 1156.248583743718 1071.0340082951532 100.0 2281244.807368659 0.9132076952234024 1.4551355696943302 2068000.0 496383.95567922783 1155.2090895470399 1065.3075848970507
1.2 100.0 3131654.864273784 12.792079979732234 9.400877697952167 2256000.0 596436.8692802276 1155.2006505569502 609.7166161507116 100.0 3135230.988765189 12.792079979732234 9.400877697952167 2256000.0 596616.7922666032 1154.9886615178298 609.7166161507116 100.0 2870855.9716478894 12.748353457738748 6.113362484052284 2256000.0 515203.0714238329 1168.7379513876847 987.0816911652408 100.0 2033597.8330731527 1.4648608258719105 2.191913783659799 2256000.0 668674.9426597657 1171.5853940919903 1116.5936243045928 100.0 1993718.653475699 1.6314693010867976 2.862113318425968 2256000.0 699682.2134346894 1169.2409281975542 1115.3327106494776
1.3 100.0 2657888.244416537 13.877660160120797 10.904788769150473 2444000.0 799331.453293951 1169.4854337440513 609.7166522652506 100.0 2659596.9006265504 13.877660160120797 10.904788769150473 2444000.0 799465.0693483641 1169.4029498355862 609.7166522652506 100.0 2525551.5729524908 13.88278426430305 7.755259343391466 2444000.0 668822.2102145946 1185.4059691553052 1061.2092563692624 100.0 1833654.9773113606 2.1235521163287885 3.328340357450333 2444000.0 833989.5484353894 1185.3163397009876 1159.8230171639452 100.0 1784137.8287157016 2.280255394849022 4.297455238539404 2444000.0 883228.9124451581 1182.0375035276136 1176.809886957527
1.4 100.0 2308835.510038626 14.639481290524175 12.20555900954837 2632000.0 981264.6548692761 1182.1904548946936 609.7166524299539 100.0 2307632.3576840446 14.639481290524175 12.20555900954837 2632000.0 981604.4990993909 1182.4045653955625 609.7166524299539 100.0 2242893.705396496 14.205490679802319 8.904276643057377 2632000.0 807889.4033723974 1201.293652604096 1121.7135010521165 100.0 1687165.6660641977 2.6798686957899074 4.439939888108399 2632000.0 979190.8876862063 1198.3145368304374 1196.7244196035247 100.0 1612697.576763364 2.8739221509968846 5.63545424423681 2632000.0 1050576.739599624 1193.8662846691377 1201.0844083740797
1.5 100.0 2022661.4063334514 15.127100529448517 13.071102331474673 2820000.0 1150322.6470210215 1194.4637530757977 617.7604770185377 100.0 2023763.546232838 15.127100529448517 13.071102331474673 2820000.0 1149997.369219176 1194.425227633584 617.7604770185377 100.0 2063157.5995677055 14.172875432773191 9.958250933829449 2820000.0 929329.3912318092 1215.8303698496757 1197.1452563304415 100.0 1562423.0779139595 3.2704012251901005 5.548289745314243 2820000.0 1112519.90827617 1210.5151845300486 1243.8450547630414 100.0 1471857.882201673 3.391750569725168 7.0122749127731225 2820000.0 1201889.661244451 1205.0027145460394 1230.294866522342
2.0 100.0 1260936.7739919897 15.196465460366216 16.604428964957755 3760000.0 1794668.730168335 1244.6305196967432 828.5205440156868 100.0 1261039.8045704071 15.196465460366216 16.604428964957755 3760000.0 1794298.7683043554 1244.5996378649932 828.5205440156868 100.0 1395634.7623877858 14.253735199958657 15.94298150402505 3760000.0 1474706.6748590446 1273.3087550668558 2086.9717082346206 100.0 1165498.6259029831 6.082687870219546 11.43330233287744 3760000.0 1647844.3337651861 1261.8771630886692 1426.8018370242237 100.0 1042477.8376126585 5.607928545418874 12.967178500325078 3760000.0 1803928.374507084 1252.1566379380145 1417.1004167723152
2.5 100.0 993273.0086524673 14.624966474953066 19.537835737489015 4700000.0 2191851.280396376 1285.8550419974317 972.0294217758203 100.0 994551.3636561412 14.624966474953066 19.537835737489015 4700000.0 2191487.774576717 1286.0249789171735 972.0294217758203 100.0 1015303.495018968 13.712141197695498 21.764832755159798 4700000.0 1986851.8147353122 1309.3965799838227 2130.0094582562715 100.0 945821.5330723404 8.744709736029845 17.220300740791245 4700000.0 2049858.6855569414 1303.5857825361165 1807.5785870340212 100.0 856799.2578585861 7.804953382918144 17.909538535116624 4700000.0 2195867.8687204076 1291.896137087998 1587.6767178526984
3.0 100.0 865103.2764473379 13.735642757641866 22.65094170358961 5640000.0 2429005.3318225723 1325.7280564475532 1302.118397488888 100.0 864466.0726784003 13.735642757641866 22.65094170358961 5640000.0 2429591.6927839206 1325.556525280571 1302.118397488888 100.0 797101.5496034158 14.166767738023047 25.267410301964947 5640000.0 2387673.3652751846 1339.0850354089437 2512.690879060858 100.0 797473.484781842 11.34683121863829 22.874700671283403 5640000.0 2376185.197401426 1338.362884877768 2261.687165873927 100.0 762350.0254673637 10.252624402710705 22.709904996564468 5640000.0 2456811.6525510787 1329.6306623748546 1796.5350145019436


==> data/stats/fashion_mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 4933489.734716926 7.12436416801194 2.684691203488596 3104400.0 461855.5149557884 1200.6811059243144 881.0718058372908 100.0 4932495.457354477 7.12436416801194 2.684691203488596 3104400.0 463198.2704219756 1200.6241323668758 881.0718058372908 100.0 3571822.087589398 0.0 0.0 3104400.0 551112.6724330119 1224.3896898838107 2615.0904949934275 100.0 5291608.239221233 0.08432510791662061 0.05911407626381759 3104400.0 589067.3867445911 1181.0062814470687 408.68825971037575 100.0 5134050.907395344 0.27414182100641493 0.25559256372097416 3104400.0 633801.517154499 1179.8425822868264 382.32574650668323
1.2 100.0 4572697.133518198 11.604133021841045 3.7693210739237024 3386600.0 659460.2479931103 1218.8177697392473 1035.129351487251 100.0 4580451.812145016 11.604133021841045 3.7693210739237024 3386600.0 658398.0146685127 1218.5652475391198 1035.129351487251 100.0 3388060.262518782 0.0 0.0 3386600.0 678598.226141262 1256.967577685322 2875.683277287942 100.0 4405522.05463632 0.14254473162805878 0.10774964883461802 3386600.0 905155.716214426 1196.1542803367208 468.69624618428975 100.0 4049319.2330866586 0.5225416305927584 0.5342278824491283 3386600.0 1014016.0029198447 1193.5144970762433 402.7830689100371
1.3 100.0 4245963.130287798 14.979116099700601 4.641208796853956 3668800.0 837457.5017501817 1236.1063867051 1190.4687403604867 100.0 4246496.59085531 14.979116099700601 4.641208796853956 3668800.0 838384.1320743927 1236.1176314910892 1190.4687403604867 100.0 3237244.612779865 0.0 0.0 3668800.0 799513.0255752639 1285.4750930822188 -3235.8565424049298 100.0 3860672.1785592455 0.20646014799262824 0.16067327493123804 3668800.0 1159791.910217306 1210.1751441864922 541.7440952442132 100.0 3360735.652314671 0.6673004107399042 0.7693403711226686 3668800.0 1344331.1032319518 1205.8478894492239 419.99608373119486
1.4 100.0 3907336.882388375 17.73281776225521 5.463240505754429 3951000.0 1012173.4898611959 1251.6114599109708 1364.533292473985 100.0 3908289.460125791 17.73281776225521 5.463240505754429 3951000.0 1011957.3316517188 1251.9760528938457 1364.533292473985 100.0 3073476.837580898 5.686424186386556 0.9954565467756055 3951000.0 918624.2575608604 1310.560522635287 3967.4787795559896 100.0 3500328.056945988 0.2553819664017322 0.21177020545160544 3951000.0 1378360.1411413995 1223.2574249329182 616.58238693826 100.0 2867919.4109054212 0.8177782999434264 1.0086022526614347 3951000.0 1637464.0735124783 1217.3723397427364 447.46748001991625
1.5 100.0 3696057.475558341 19.470131330376297 6.169537850295388 4233300.0 1166397.536241615 1265.8799307289783 1590.8819452829525 100.0 3700920.543623114 19.470131330376297 6.169537850295388 4233300.0 1166269.6710143606 1266.0842323549462 1590.8819452829525 100.0 2901829.0258905706 15.689815865595893 2.369764243016914 4233300.0 1029219.591911694 1334.6183735852671 4833.405632663546 100.0 3201465.7800528016 0.31868598195589304 0.2677991954844181 4233300.0 1577719.5680993819 1235.3803914686277 681.9061382559188 100.0 2505400.8712797896 0.9416668658760745 1.2391233853745367 4233300.0 1904733.6807920227 1227.8725793543358 461.4865189257272
2.0 100.0 2709064.3985615005 24.36281352034385 8.932985653326334 5644400.0 1848891.5391584993 1324.5255563226212 2206.703771120136 100.0 2710163.4679400325 24.36281352034385 8.932985653326334 5644400.0 1847389.2866609495 1324.9518726378417 2206.703771120136 100.0 2573658.8670921796 34.448234290063 4.723704612382358 5644400.0 1333473.6913783322 1432.0710576589045 8058.599815228186 100.0 2391876.3889792906 0.5389146176820678 0.5236392446022942 5644400.0 2320083.954039331 1285.6656257902255 1052.8859916520303 100.0 1462603.623139068 1.3316524988440963 2.433698383298337 5644400.0 3014152.4625423453 1270.8087178919566 553.5868332975765
2.5 100.0 2324341.5487590274 25.905153929771718 10.978513974050347 7055500.0 2348077.129599726 1365.977087205149 2414.6308914323076 100.0 2323232.1621892075 25.905153929771718 10.978513974050347 7055500.0 2348848.593333895 1365.9184754799696 2414.6308914323076 100.0 2431466.9431445547 41.98203190665327 6.242481105159879 7055500.0 1547661.5668894951 1490.9872670690593 8856.20118629905 100.0 1990215.7694909358 0.7798822162775852 0.7848534454704144 7055500.0 2857049.5435137767 1323.8383951999733 1410.583676918558 100.0 1125212.2147034334 1.7930631515290472 3.3126084007283993 7055500.0 3714639.0371175082 1305.657119563481 690.6255137512392
3.0 100.0 2104045.417719165 26.684407101681014 12.536964207668994 8466600.0 2753376.4708638503 1400.2980077901416 2779.3047784318524 100.0 2106298.9410958593 26.684407101681014 12.536964207668994 8466600.0 2752067.5523769436 1400.1320282040285 2779.3047784318524 100.0 2345275.3103399957 42.928792778953614 7.226459071797694 8466600.0 1745083.6904237783 1525.8576299052384 9704.01052116421 100.0 1738673.1799412281 1.008783738098304 1.0307611132943622 8466600.0 3279538.591931595 1354.4462057144603 1777.1105335336767 100.0 907985.4666969033 2.1181405603425905 4.142635739121242 8466600.0 4296303.577658674 1333.6724232396164 815.9326500044867
3.5 100.0 1937999.8942058242 27.445717266511593 13.910649626655164 9877700.0 3090433.8003198965 1429.343322400332 3244.9917267504525 100.0 1938760.9117055875 27.445717266511593 13.910649626655164 9877700.0 3091224.827026705 1429.2369842189382 3244.9917267504525 100.0 2259399.406722434 44.73397203815496 7.875411252186941 9877700.0 1901654.729368327 1564.516502367589 12881.136682282622 100.0 1570782.8908264888 1.2315493939434934 1.3281450417041412 9877700.0 3630042.801935135 1380.1215601515514 2142.5490807714946 100.0 786888.0053685745 2.4410627508593756 4.809486103317972 9877700.0 4743343.621381584 1357.9047695345612 958.0404507558161
4.0 100.0 1786143.4286580342 28.177801193981626 15.134325095989535 11288800.0 3400010.2897812044 1455.5473575814256 3786.353466106108 100.0 1786124.2696069144 28.177801193981626 15.134325095989535 11288800.0 3399570.0695117647 1454.9388539388951 3786.353466106108 100.0 2148584.470918411 48.59459527906143 8.52895311698401 11288800.0 2057587.4846365473 1597.6599656844278 16176.680096485694 100.0 1431857.8196277125 1.4509013663049293 1.549419381667654 11288800.0 3931005.063406205 1402.4939146733761 2510.9318891011817 100.0 695648.2186708237 2.7369165322663767 5.510000173351972 11288800.0 5132525.809969269 1378.7683325441878 1091.6206383501506
4.5 100.0 1659816.5683148946 28.858905221131536 16.328102610640347 12699900.0 3679878.9010989233 1478.3351959278014 4280.916822750565 100.0 1660563.288854241 28.858905221131536 16.328102610640347 12699900.0 3679950.0330126714 1477.3688045197437 4280.916822750565 100.0 2026182.617616731 50.77496744191772 9.084321916593886 12699900.0 2221396.5116413184 1630.3641482496396 18518.62387754174 100.0 1329754.1420252617 1.677125907784969 1.7904029446726464 12699900.0 4194665.3384215655 1422.1864567994648 2874.874721173823 100.0 635196.9691333116 3.0411394217946386 6.160575506890929 12699900.0 5460130.267402512 1397.326270604973 1240.7473376537348
5.0 100.0 1549741.277171554 29.523596064526952 17.37434046689926 14111000.0 3939728.5820409334 1498.1587481939955 4653.816502154435 100.0 1551205.1879049374 29.523596064526952 17.37434046689926 14111000.0 3939473.991728879 1498.6992899924128 4653.816502154435 100.0 1936093.5835398613 51.46212599199396 9.583732851465761 14111000.0 2370876.3056915193 1654.6980802247397 19988.39117671004 100.0 1239006.5265803034 1.893192228284225 2.0692315734377917 14111000.0 4439513.194909289 1439.984363777412 3241.0738051375674 100.0 585721.6118542345 3.3044451245765374 6.745017885059503 14111000.0 5753895.012965605 1413.9839731767727 1377.5175556570923
5.5 100.0 1445885.769997833 29.961275930595153 18.37530386223934 15522100.0 4186175.868383928 1516.9006487905283 4887.159048120158 100.0 1445670.8489576452 29.961275930595153 18.37530386223934 15522100.0 4183747.673568617 1516.4121243349293 4887.159048120158 100.0 1868455.0274143824 51.591902855531124 10.02107891525249 15522100.0 2503731.272049019 1669.3465998896677 21021.957149972895 100.0 1163705.0077072144 2.1178744409188424 2.3709360979063447 15522100.0 4653826.231188676 1456.1203258434593 3609.2588880255553 100.0 547226.8859093925 3.555829632348838 7.329988271771747 15522100.0 6010361.282218909 1429.1314813511306 1521.2930384015299
6.0 100.0 1357353.575446565 30.35120208525238 19.297269118140186 16933200.0 4419170.08779914 1532.294637549506 4984.375122769944 100.0 1357415.3933296301 30.35120208525238 19.297269118140186 16933200.0 4420247.978832674 1532.249783910115 4984.375122769944 100.0 1808263.035247955 51.51268806910962 10.507624246411288 16933200.0 2632982.0843448695 1681.3835582744016 21781.455701765746 100.0 1099677.2664655212 2.350809466096324 2.6158482316513667 16933200.0 4853694.619174613 1471.225309239893 3967.4828944050646 100.0 519224.353714302 3.8121323509105416 7.878564145403384 16933200.0 6239451.369698417 1443.2610210463065 1674.351252702008
6.5 100.0 1277735.9533778708 30.63478596984705 20.128682699143425 18344300.0 4641481.881087124 1547.3270834298066 5096.687213379083 100.0 1278388.2524199663 30.63478596984705 20.128682699143425 18344300.0 4639682.541457149 1546.9315966516124 5096.687213379083 100.0 1748438.5659642743 51.33764971773858 10.893090414110281 18344300.0 2763785.659856754 1699.566050551011 22285.887715869194 100.0 1040924.8977165093 2.5659428221034224 2.857092878956103 18344300.0 5037818.82745512 1485.0957708832639 4346.22739223596 100.0 492986.0137007707 4.0411773575304695 8.396351139221814 18344300.0 6450958.135925491 1456.2319402931114 1822.8740921228105
7.0 100.0 1203265.498127628 30.89405397457174 20.945096697158487 19755400.0 4857404.7279482065 1560.685359167901 5482.324232296806 100.0 1203303.2471159685 30.89405397457174 20.945096697158487 19755400.0 4855486.247917953 1560.9891534319765 5482.324232296806 100.0 1714124.2778720793 50.88536095608633 11.180175774684265 19755400.0 2870598.0014162757 1709.5111989252664 22635.95736254857 100.0 998217.318463927 2.7834817882283094 3.123012592405474 19755400.0 5205196.996480413 1497.9180612429052 4704.360153533811 100.0 471655.3565157039 4.277520560288241 8.951212450887985 19755400.0 6641959.184793499 1468.4559514656403 1976.1023746109145
7.5 100.0 1135641.1422165632 31.22561159583058 21.69787015588922 21166500.0 5056310.712536395 1573.5125345524427 5875.155206535877 100.0 1136132.9999220278 31.22561159583058 21.69787015588922 21166500.0 5056585.206968235 1573.0918705792446 5875.155206535877 100.0 1669393.0350869796 49.99159693485355 11.382300867026133 21166500.0 2973069.9950012793 1721.030105891628 22892.118857106365 100.0 951932.562718445 3.0103481691938976 3.3827768679094996 21166500.0 5367148.676998716 1510.0905564673535 5079.690201806606 100.0 453792.7250485576 4.4969434183389545 9.419845156642227 21166500.0 6818336.755108551 1479.7519348197366 2128.506140752387
8.0 100.0 1067483.464395783 31.513031619701977 22.36618211228084 22577600.0 5259147.107163014 1585.9051451516332 6169.717970882588 100.0 1067937.1180450728 31.513031619701977 22.36618211228084 22577600.0 5256381.476995095 1585.2181950819163 6169.717970882588 100.0 1634585.8992071752 48.867624192260955 11.534349119445723 22577600.0 3065006.0668204785 1724.0437703052662 23083.456242273987 100.0 906794.1036570271 3.232856602855701 3.6658909079753235 22577600.0 5521367.6608152175 1521.5986551419912 5435.524038543936 100.0 439187.8225053116 4.726436725536364 9.946483359558728 22577600.0 6980060.163937933 1490.612435693331 2288.183487871409
8.5 100.0 1003896.4921111681 31.7107260537114 23.096481821026423 23988700.0 5449526.109154476 1596.6684724618465 6509.455674713823 100.0 1003510.6632675581 31.7107260537114 23.096481821026423 23988700.0 5447264.618330451 1596.7537872691532 6509.455674713823 100.0 1614609.5050786524 47.66125123617503 11.662024028344256 23988700.0 3134348.3123333543 1736.1321460598808 23236.534622408693 100.0 870834.4297208781 3.454720039483116 3.9264010738300463 23988700.0 5659683.759754669 1531.8678494619835 5816.955485739787 100.0 425179.60805704043 4.954768462867388 10.4404353637455 23988700.0 7133084.117145506 1500.5943790820006 2446.9270203182123
9.0 100.0 944722.1322177574 31.821278427855315 23.696998715697912 25399800.0 5631648.163384703 1606.4124149475895 6881.814999547592 100.0 944387.1292934539 31.821278427855315 23.696998715697912 25399800.0 5634418.149439951 1606.149180512814 6881.814999547592 100.0 1595504.5926504638 46.56079128249886 11.820573162920113 25399800.0 3198599.1430975907 1745.5739225913521 23362.195371393856 100.0 838690.2241214637 3.6704394596744274 4.1742609267727815 25399800.0 5792220.202024808 1541.4754993279455 6167.612049288107 100.0 413052.17484394216 5.172911662146018 10.93669963940724 25399800.0 7273066.873803831 1510.4004261196503 2605.9386816792803
9.5 100.0 888854.6449863814 31.929142445968527 24.30109591808158 26810900.0 5813271.421508115 1616.4527032786218 7234.8512703048755 100.0 888221.5373268831 31.929142445968527 24.30109591808158 26810900.0 5814455.23550581 1616.5766140877054 7234.8512703048755 100.0 1579751.5111385763 45.659777662237246 11.934464281971973 26810900.0 3252136.5679622996 1754.3409922723986 23486.674706507765 100.0 805385.7493338863 3.894701777692994 4.466713566927128 26810900.0 5924953.598723743 1550.9558210097641 6533.00240340276 100.0 402717.36640675634 5.385386245467965 11.410130523671343 26810900.0 7405663.351862673 1519.9601533728119 2768.499574333291
10.0 100.0 838457.823342747 32.030714577766155 24.883304799689405 28222000.0 5986153.943577355 1624.6257430097437 7526.071252369073 100.0 838919.853030153 32.030714577766155 24.883304799689405 28222000.0 5986307.22126894 1625.5785804689303 7526.071252369073 100.0 1566754.0419237502 44.86100379673445 12.080907492935891 28222000.0 3299838.3183977 1762.6081067423506 23602.696139522177 100.0 779486.9712882066 4.129156546640651 4.755766792529461 28222000.0 6042729.781362754 1560.7321255906365 6907.072121737898 100.0 393463.4384340433 5.594107192678436 11.830443068520296 28222000.0 7530170.754802167 1528.7092313210717 2938.175456239502


==> data/stats/mnist_100.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 5856196.973797673 4.539760885671796 3.482325996413644 5426700.0 1264545.8534743993 1253.494350101127 954.0576725366839 100.0 5852004.265807737 4.539760885671796 3.482325996413644 5426700.0 1265465.3378315216 1253.5596576916116 954.0576725366839 100.0 6853174.982365589 8.037456312424984 2.109703453576775 5426700.0 992624.7336551 1255.636174550624 1427.8625834134364 100.0 9918597.686273675 0.1117770962065606 0.07093548109885726 5426700.0 974542.0362396059 1235.4042127429875 446.9524856348751 100.0 9221071.129685657 0.5456302833204059 0.4814836553292791 5426700.0 1094631.6035495023 1234.3845442063018 392.85907296749303
1.2 100.0 5413760.908826879 7.082869255919233 4.9542047255591655 5920000.0 1680426.2684348742 1267.6969566446294 954.0576726298578 100.0 5413252.283263647 7.082869255919233 4.9542047255591655 5920000.0 1676855.077953607 1267.832288132144 954.0576726298578 100.0 6489217.257824449 13.146119776768291 3.1724162751571536 5920000.0 1274323.1239300426 1277.3012977954957 2111.6729526840054 100.0 8594804.02745416 0.21897921996493055 0.14062183487278698 5920000.0 1439833.6229245518 1251.4091980263747 590.1032566263091 100.0 7317765.652876699 0.9611831107432621 0.9337800132688038 5920000.0 1757659.4721666775 1248.106858823041 415.9225125843275
1.3 100.0 5066199.823962818 8.948479488788728 5.948931842820796 6413400.0 2045633.1987343961 1281.1075594424515 954.0576727549592 100.0 5068476.055603982 8.948479488788728 5.948931842820796 6413400.0 2042101.8247272638 1281.0974835545458 954.0576727549592 100.0 6207483.917127229 16.376263233708492 4.047845290201117 6413400.0 1522983.2573964891 1298.7632435369412 2316.586803003964 100.0 7712368.488971129 0.3220433324341579 0.21595171698269416 6413400.0 1808974.3108269908 1266.6872790751015 730.5944462983236 100.0 6089735.996886434 1.3113906108074835 1.4138319856384478 6413400.0 2327573.501158802 1260.6754545345525 432.9009075436613
1.4 100.0 4774152.264459194 10.527600652299158 6.834419269737115 6906700.0 2380504.6435164516 1293.6440841951003 954.0576728712164 100.0 4774171.145358322 10.527600652299158 6.834419269737115 6906700.0 2381150.4493802614 1293.5020732472751 954.0576728712164 100.0 5824251.523951711 18.851501343614906 4.775189902501773 6906700.0 1774406.1670477756 1318.9570933578964 2891.93640752756 100.0 7076976.041974383 0.43511954890496374 0.2765079318889948 6906700.0 2127099.682540791 1281.1202111236407 874.8160369104046 100.0 5235472.525201494 1.5793686493720753 1.8597640664673545 6906700.0 2835142.502814019 1272.3693249380024 455.5352323879403
1.5 100.0 4531070.497657392 11.773878267600383 7.583930288817278 7400100.0 2683336.135608915 1305.1765904108554 954.0576728717742 100.0 4530805.504195759 11.773878267600383 7.583930288817278 7400100.0 2683502.7992053935 1305.2878083364578 954.0576728717742 100.0 5443250.183219703 20.422507565503693 5.429099485421474 7400100.0 2018570.8200126807 1336.612102194464 3368.136947224049 100.0 6593528.692493037 0.5388984317194488 0.3485361185928862 7400100.0 2399206.7799055357 1294.7814811023736 1014.6223920913224 100.0 4593522.104040699 1.8088331494721228 2.2589157566642966 7400100.0 3291111.02055342 1283.134843315321 486.1671722902682
2.0 100.0 3689103.5432099905 15.539605867180626 10.665461837432218 9866800.0 3941538.477094509 1355.222701411948 1160.0893473961012 100.0 3690396.192012589 15.539605867180626 10.665461837432218 9866800.0 3940394.8552727634 1355.232616942451 1160.0893473961012 100.0 4384382.084105231 24.239831462644805 7.937595059652944 9866800.0 2957355.1252892786 1409.7557184755226 5306.211932726378 100.0 5039613.888044351 0.9968021791622473 0.6607011071315682 9866800.0 3454999.9207588234 1350.038618313246 1730.807793882914 100.0 2817235.0601649676 2.6036888128980133 4.254336143938966 9866800.0 5147022.190803783 1326.8874277100188 599.7368746912985
2.5 100.0 3186235.2283784347 17.481571244768784 13.011824023231892 12333500.0 4907000.277450182 1393.3595410700443 1467.9963113490824 100.0 3185625.7458406277 17.481571244768784 13.011824023231892 12333500.0 4909666.755762044 1393.3845520656348 1467.9963113490824 100.0 3732490.132760681 26.492881786721423 9.534603271356232 12333500.0 3671835.8786275713 1469.7187283639585 7527.504545508671 100.0 4273792.984451936 1.463864710644844 1.0145913962132067 12333500.0 4209214.422050737 1392.0822029071867 2433.3731475448353 100.0 2210131.3769307868 3.363836885129386 5.831009285176164 12333500.0 6334473.378085675 1362.4774396362052 749.6037242166983
3.0 100.0 2836515.635224386 18.811699839967993 14.918212982729855 14800200.0 5700656.008599361 1424.7943025936352 1670.195289778382 100.0 2836569.9913306315 18.811699839967993 14.918212982729855 14800200.0 5701882.456147681 1424.7917562127257 1670.195289778382 100.0 3290489.805215386 28.62589345640486 10.899412456018169 14800200.0 4262792.201018853 1514.4619403837196 9669.162906192887 100.0 3770274.4082407663 1.9306719029088906 1.3327644201696698 14800200.0 4812684.492054695 1426.6067786299477 3146.62868317407 100.0 1846002.74298471 3.912047400006265 7.172680127114239 14800200.0 7279768.439706476 1391.4471835521308 891.0874815541973
3.5 100.0 2576982.044635378 19.779127077036133 16.5198898422977 17266900.0 6375493.115600689 1452.3453828004176 1972.4136598081134 100.0 2577978.8081179103 19.779127077036133 16.5198898422977 17266900.0 6372486.345144999 1452.3066501019514 1972.4136598081134 100.0 3056598.6707878043 29.987070954136563 11.988559644183084 17266900.0 4709958.273230675 1552.6127133956147 11337.151968297005 100.0 3417968.4666753295 2.3774568433277197 1.6438567881667538 17266900.0 5320345.028259756 1456.207091818464 3868.5504798488623 100.0 1632187.0119649272 4.40289068734113 8.338347604815818 17266900.0 8027244.2094043335 1416.1608301369927 1047.9221084033106
4.0 100.0 2383757.789865845 20.419540638555073 17.76406943516389 19733600.0 6951703.2037114445 1476.4615621495768 2322.4366358012057 100.0 2384000.9676791285 20.419540638555073 17.76406943516389 19733600.0 6951406.900323989 1476.5627835291198 2322.4366358012057 100.0 2843160.322331081 30.72436104738065 13.054580865004638 19733600.0 5121187.561891142 1585.4732841275866 12783.070022165244 100.0 3127210.662399239 2.839749352557256 1.9876347016118785 19733600.0 5767985.133257309 1482.2755523589474 4573.974339971824 100.0 1491461.0432109344 4.865612308527735 9.416753136318084 19733600.0 8629462.607939133 1438.0710587219958 1225.3587155370278
4.5 100.0 2226972.5440737116 20.98936019563375 18.970661571124595 22200300.0 7459334.867447542 1497.900519638252 2599.7312809057894 100.0 2227543.8980776826 20.98936019563375 18.970661571124595 22200300.0 7457761.690513772 1498.0232688694439 2599.7312809057894 100.0 2666146.7308550277 31.37975355069783 13.973896030134128 22200300.0 5496408.5339472145 1612.299746137151 14180.861931648142 100.0 2917676.9820806687 3.2939971053622967 2.31076330632777 22200300.0 6150427.839956096 1504.6805795580947 5288.911825115364 100.0 1387477.29488207 5.307091717582322 10.451093418444202 22200300.0 9150218.286388794 1457.3361322109113 1400.6668494426624
5.0 100.0 2101737.4339366453 21.483932766499123 19.96551558533131 24667000.0 7907635.285729524 1517.203874089574 2914.7868891703315 100.0 2102150.92480437 21.483932766499123 19.96551558533131 24667000.0 7906390.570451876 1517.2978587740663 2914.7868891703315 100.0 2493593.722175382 31.958989487238433 14.801897167963169 24667000.0 5855771.8008756135 1635.4607150994273 15540.272333273746 100.0 2717133.647434433 3.747974399305503 2.6551135521789577 24667000.0 6511880.9251385825 1524.7408967051276 5993.584122618936 100.0 1312040.0631756277 5.704495092200195 11.40311066022334 24667000.0 9594790.154764868 1474.9954220622758 1588.9810275461382
5.5 100.0 1997053.5970734619 21.906345153193726 20.818048822800982 27133700.0 8309646.711839531 1535.1898842630017 3246.0156600977725 100.0 1996346.3124649297 21.906345153193726 20.818048822800982 27133700.0 8309920.752122131 1535.0962796396434 3246.0156600977725 100.0 2342654.0345883123 32.45994835186136 15.62161715161876 27133700.0 6194294.326739115 1650.1079531409196 16780.882429359048 100.0 2552633.1031165584 4.2079768430351026 2.9831466045094284 27133700.0 6839022.299693141 1542.763834207128 6698.088819904386 100.0 1252206.913187143 6.1015957299227574 12.305905025389556 27133700.0 9986616.002783481 1491.0209399623857 1785.8136609576857
6.0 100.0 1908367.2200473032 22.309674697105223 21.61829479524158 29600400.0 8669020.579727665 1551.6136780958595 3580.2113588539996 100.0 1908976.1689890213 22.309674697105223 21.61829479524158 29600400.0 8672143.07144777 1551.811616248957 3580.2113588539996 100.0 2226809.2075818274 32.73291510254593 16.277794689154128 29600400.0 6489288.52118284 1672.0545707944048 17873.287763091586 100.0 2411451.662727842 4.665818628474739 3.276691696916636 29600400.0 7136578.448386249 1559.6740672009196 7413.65586448248 100.0 1202958.17382107 6.425880257000285 13.092710506635816 29600400.0 10333530.050284326 1505.9880288850622 1986.8632696096179
6.5 100.0 1829382.911664563 22.699052188732853 22.369474134590398 32067100.0 8999694.206827682 1567.0366857992353 3801.349703051096 100.0 1829756.5370999444 22.699052188732853 22.369474134590398 32067100.0 8998449.429514103 1567.2084507991335 3801.349703051096 100.0 2139733.3650049963 32.99896726018029 16.936346343464486 32067100.0 6751075.025700146 1688.2085187626021 18903.339887535658 100.0 2290331.6609289604 5.1201758540892355 3.6088958372095528 32067100.0 7417613.815533442 1574.007690038487 8133.292573349364 100.0 1165409.4666870576 6.792612531888095 13.919133771080533 32067100.0 10640552.04163706 1520.0058212884858 2200.850975921788
7.0 100.0 1766702.3835984971 23.019021639575538 23.035722535638055 34533800.0 9292444.495385434 1581.7004366928973 4131.79120644691 100.0 1767682.6880847039 23.019021639575538 23.035722535638055 34533800.0 9292459.122106388 1581.4584210974663 4131.79120644691 100.0 2018451.5009385482 33.340091999589106 17.569899632147255 34533800.0 7045405.479737941 1703.0790868642698 19944.428623892578 100.0 2185593.427090842 5.5757009172592005 3.9629789760081904 34533800.0 7673760.664195619 1587.7135159135155 8844.143091183281 100.0 1132841.6494649332 7.125367875484696 14.68407279986555 34533800.0 10919180.249683801 1533.2259465363354 2431.7784689367677
7.5 100.0 1716706.6413271292 23.354523756258054 23.701404747634395 37000500.0 9554757.698461154 1594.9613558134945 4476.059510954791 100.0 1715822.6470758317 23.354523756258054 23.701404747634395 37000500.0 9557527.695632214 1595.199765807466 4476.059510954791 100.0 1936231.3399456434 33.77570580021003 18.209370532397635 37000500.0 7297282.1150576025 1717.1584969198434 21004.44578145197 100.0 2091045.2124741639 6.032788689592376 4.303878827906385 37000500.0 7915233.723042792 1602.724782205724 9553.961669153496 100.0 1102354.1868203736 7.4533991504385915 15.408405958569215 37000500.0 11173471.71569869 1545.6665995350784 2666.5276517211355
8.0 100.0 1660011.4774900496 23.626187699832485 24.275984349451335 39467200.0 9802678.448334873 1608.0268503210682 4802.178859796294 100.0 1658958.1580499723 23.626187699832485 24.275984349451335 39467200.0 9801535.152317524 1607.7629959075164 4802.178859796294 100.0 1872194.1817842477 34.285605019181915 18.82651503820166 39467200.0 7532768.250894619 1729.0261047999516 22108.06870902818 100.0 1995557.4597918526 6.491329664275619 4.608769838365435 39467200.0 8152385.055191003 1615.2683622517145 10258.881068137835 100.0 1080823.342752511 7.758310991142977 16.076190143714435 39467200.0 11402112.480507042 1557.5872781944497 2913.8706320036335
8.5 100.0 1611445.9550052143 23.889621710123716 24.86083578679988 41933900.0 10025291.056946814 1620.2101571913354 5084.977412193211 100.0 1611969.4868589116 23.889621710123716 24.86083578679988 41933900.0 10028161.069391733 1620.1663503292866 5084.977412193211 100.0 1790358.16597566 34.78678440328798 19.484170329566375 41933900.0 7785823.299655845 1748.0162215313999 23199.074910217056 100.0 1923945.9858464273 6.944016983378501 4.97815321797247 41933900.0 8364728.351658772 1626.9231822693205 10959.984707027937 100.0 1058013.9564262081 8.079278284641052 16.75898635339089 41933900.0 11615155.783205852 1568.893085190682 3167.873371002131
9.0 100.0 1564189.0317480876 24.101741559439432 25.37665522496329 44400600.0 10233851.36270325 1631.852227541669 5336.242554878537 100.0 1565390.703230057 24.101741559439432 25.37665522496329 44400600.0 10233682.19271192 1632.0075188109558 5336.242554878537 100.0 1694328.0730713282 35.13170255750443 20.081588111326543 44400600.0 8059585.105334118 1753.5266651469153 24189.267093357892 100.0 1847450.3244092783 7.408551324606447 5.289151811225536 44400600.0 8577040.079717496 1640.086509110902 11703.451982310025 100.0 1038844.4783599887 8.38447258795588 17.389964371491246 44400600.0 11810205.29735308 1579.7989566337312 3429.571488162881
9.5 100.0 1524899.7493195212 24.368180464823023 25.891699870843443 46867300.0 10422695.211531363 1643.2101600364217 5547.50394098652 100.0 1525096.3503352338 24.368180464823023 25.891699870843443 46867300.0 10422855.031494917 1643.0789855679986 5547.50394098652 100.0 1619274.2426073237 35.477417779223366 20.6587526934299 46867300.0 8317827.928619561 1766.957791887738 25095.294778486426 100.0 1784272.6440651626 7.853483058291319 5.635263153110846 46867300.0 8768063.732624179 1650.3951795912308 12374.811226609487 100.0 1020210.7621620086 8.689801023749903 18.020236027489574 46867300.0 11991864.469629742 1590.1773937245782 3703.0111139468872
10.0 100.0 1480253.1689254397 24.64772231051352 26.374224894592192 49334000.0 10597440.182267057 1654.0665696421406 5747.319538651409 100.0 1480555.7608772058 24.64772231051352 26.374224894592192 49334000.0 10596859.157899266 1654.288933304536 5747.319538651409 100.0 1549628.758773294 35.76733486721403 21.253334666110398 49334000.0 8564711.381992875 1773.6337143662292 25887.362052687233 100.0 1717341.5888224903 8.320639490686057 5.941017426720302 49334000.0 8963598.691370934 1663.5586605969315 13104.767631028957 100.0 1004239.518292174 8.975386061810704 18.611525984195705 49334000.0 12157854.8798405 1600.0078550994435 3984.4332712351907


==> data/stats/ms_academic_phy.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 9142372.163512195 13.077992195434865 7.433095465884729 3794200.0 543172.6622265056 1201.6712946864036 576.307239112395 100.0 9155598.944783757 13.077992195434865 7.433095465884729 3794200.0 541009.3911406199 1201.6220356482347 576.307239112395 100.0 7124833.159326025 12.607740020023245 4.127397967364286 3794200.0 548756.2923205685 1206.1669495115239 1029.3320750600844 100.0 5847235.445855628 0.8208140757264232 0.7467904129897782 3794200.0 771849.6546153534 1201.4822894753177 524.9956338868847 100.0 5913697.507403189 1.2670126502984385 1.2684015648744256 3794200.0 794164.2244297531 1200.1835870019543 481.39280638910594
1.2 100.0 7451736.8746735975 18.02970641950025 10.472288143119908 4139100.0 927179.6990114707 1217.2627294377708 680.5722621569421 100.0 7452684.87971573 18.02970641950025 10.472288143119908 4139100.0 930197.7215429486 1217.3250654045219 680.5722621569421 100.0 6086610.241988679 16.952839588176687 6.138640654861689 4139100.0 846202.7774535576 1225.4780651487415 1115.9625713307048 100.0 4778679.68597387 1.4283679791450155 1.4483417470943338 4139100.0 1188512.0143369252 1216.4332620675116 577.0936409977575 100.0 4768401.241562846 2.2318227916829647 2.5059655803882412 4139100.0 1247653.710980147 1214.0592366929918 508.2660485371407
1.3 100.0 6259345.265468738 20.755140057955014 12.727018163628493 4484000.0 1286789.112436139 1231.1007491827788 680.6330256058017 100.0 6262684.113345875 20.755140057955014 12.727018163628493 4484000.0 1288659.06366637 1231.2009048573252 680.6330256058017 100.0 5212977.276975382 19.32319549131715 7.79619555869073 4484000.0 1128578.6037636667 1242.6976144924997 1290.4214129537127 100.0 4086693.4487528414 1.9599983050133847 2.1992996652690158 4484000.0 1537328.2060683924 1230.2233411475675 643.8634958916042 100.0 4024422.160542235 2.9895312692016884 3.6928300355570007 4484000.0 1644532.587052398 1226.539492228647 524.221076872566
1.4 100.0 5396589.23035895 22.04678488886969 14.24956557244268 4829000.0 1620108.4920131108 1244.032878756341 706.499035201787 100.0 5389733.058534711 22.04678488886969 14.24956557244268 4829000.0 1619181.3888282452 1243.9587490279432 706.499035201787 100.0 4635573.964599978 21.01133822743732 9.274892463676624 4829000.0 1379949.324318708 1258.6463972499291 1441.1309519839247 100.0 3607976.227838938 2.412476292304653 2.9015126633520802 4829000.0 1844539.3552649217 1243.146957596024 723.2054906322444 100.0 3469043.5953849554 3.6859635183411705 4.816184299460153 4829000.0 2001180.9254115636 1238.2304313590425 550.6310159733541
1.5 100.0 4798376.8474616995 23.339421202946692 15.793757890270227 5173900.0 1920630.693828459 1255.3764108410135 801.7034558366216 100.0 4794587.214760757 23.339421202946692 15.793757890270227 5173900.0 1921880.5983067162 1255.3484113194659 801.7034558366216 100.0 4242645.252467108 22.26670174657465 10.540494552056021 5173900.0 1607678.569755035 1272.549134622222 1554.6353632260216 100.0 3244964.9509249763 2.794224335372945 3.607133095067293 5173900.0 2121652.8491807366 1254.8945384853123 794.5337790932746 100.0 3040069.9873338346 4.207528153429012 5.930430702328851 5173900.0 2326506.076467571 1248.99060835426 590.2086992109244
2.0 100.0 2909483.777173622 25.033137049652098 20.796956758166278 6898600.0 3178687.3774921424 1302.8277414060994 960.1441532143468 100.0 2906777.3714812445 25.033137049652098 20.796956758166278 6898600.0 3177576.5576354614 1302.7864635888009 960.1441532143468 100.0 3258718.000000221 25.100159792501326 15.722143069913558 6898600.0 2500338.2429440096 1328.6961078712727 1696.4133266982767 100.0 2217684.6172646554 4.463246085222382 7.035014907155943 6898600.0 3211262.936740702 1304.3904685192658 1152.3893629531588 100.0 1821527.6352548157 6.188214210864771 10.879022004015603 6898600.0 3650392.972312185 1293.1223864638823 689.0373306436392
2.5 100.0 1976795.1943918604 25.282275471675174 24.47953194927926 8623200.0 4153339.678174178 1338.534017361746 1044.3740859274428 100.0 1976763.965558097 25.282275471675174 24.47953194927926 8623200.0 4155892.4771836363 1338.5944221584477 1044.3740859274428 100.0 2667164.9413459394 25.89911656388834 19.513523785142745 8623200.0 3209882.1158260508 1371.3195636378352 2153.922919284878 100.0 1717929.1639737114 5.953223190225669 10.352380700070766 8623200.0 4010918.205077584 1343.1106915815317 1538.6127143116505 100.0 1374285.495616051 8.173189284227517 14.822864568416913 8623200.0 4520857.8994891 1329.1772406749915 813.117068262229
3.0 100.0 1459367.9890628112 25.08654649635908 26.882567581640977 10347900.0 4942638.335164554 1367.8987933914457 1173.2262643069885 100.0 1459232.2998647592 25.08654649635908 26.882567581640977 10347900.0 4941624.303182105 1367.9312637483572 1173.2262643069885 100.0 2165474.0484610912 25.664317973127453 23.58401883966053 10347900.0 3923526.752777299 1401.8190443551186 2709.70884586307 100.0 1404660.7098691554 7.362571509118407 13.50941301190586 10347900.0 4650893.853747245 1374.6959851659153 1923.7175682310615 100.0 1107679.1446158055 9.676521268257696 18.010822104135265 10347900.0 5205612.03891783 1359.2863913276708 969.2655102689046
3.5 100.0 1151737.7319345903 24.76795708603031 28.766090201005767 12072500.0 5587365.773333244 1392.90952851875 1321.2880610268248 100.0 1151264.9241346705 24.76795708603031 28.766090201005767 12072500.0 5588222.124160196 1392.8046656088095 1321.2880610268248 100.0 1715939.296543714 25.364311928123907 27.32699297580315 12072500.0 4654509.2020995105 1422.4950943231581 2818.54076526442 100.0 1189614.5928297297 8.73021955389868 16.59429288839316 12072500.0 5189086.954752463 1401.354631323458 2298.9429827258696 100.0 948243.261445087 11.102518308671549 21.054894483349646 12072500.0 5742635.388929861 1385.4623902251656 1160.3090946359346
4.0 100.0 959915.3885820224 24.438433814562227 30.241769925035573 13797200.0 6113699.434505591 1415.0766669823934 1394.1750557509351 100.0 959874.6781646236 24.438433814562227 30.241769925035573 13797200.0 6114442.123903222 1415.1132427138346 1394.1750557509351 100.0 1404798.6772778248 24.64964558097361 30.174382047539872 13797200.0 5277401.87159053 1441.3233144765925 2831.777310152689 100.0 1032026.2120437698 10.090949370164312 19.637553479533832 13797200.0 5655565.53164907 1424.471163940471 2678.6081024966484 100.0 845016.4180632986 12.420087833533263 23.828119772087902 13797200.0 6180629.084177181 1409.2042938119894 1376.9733289899552
4.5 100.0 839445.7051448242 23.943554373935356 31.4640016430297 15521800.0 6539725.924295678 1435.0963079564203 1535.8777599954817 100.0 839600.1667920655 23.943554373935356 31.4640016430297 15521800.0 6539314.21622501 1435.2120237028994 1535.8777599954817 100.0 1160214.4702473576 23.883696408889595 32.502485026796904 15521800.0 5833690.561828574 1457.5711675893108 2846.6436919843613 100.0 910559.0480814939 11.446503185050663 22.575861275074214 15521800.0 6063770.183338752 1445.6904433609793 3058.502137239706 100.0 768314.2594760365 13.595836297640767 26.377490217721768 15521800.0 6544635.104110271 1430.7280980503406 1636.9052912943926
5.0 100.0 765310.9718044783 23.399278116540426 32.58122191055383 17246500.0 6879341.670333336 1453.9847265409462 1768.2649851471986 100.0 765451.4830767005 23.399278116540426 32.58122191055383 17246500.0 6880384.910421295 1453.9479324755034 1768.2649851471986 100.0 936752.1808969668 23.260181067218426 34.560612447717176 17246500.0 6361835.960159467 1472.6198488266928 3187.192394711049 100.0 815679.4147670631 12.786242148128633 25.435669715890963 17246500.0 6427184.001756711 1464.6918182457507 3441.501030260584 100.0 715222.9680635863 14.739499599598794 28.78405885244676 17246500.0 6845515.64893475 1450.7472279492538 1925.9511244753025
5.5 100.0 718515.2738754124 22.67485489544182 33.61776783526164 18971100.0 7142751.286700826 1471.936682025156 1946.7569010411592 100.0 718543.6488614515 22.67485489544182 33.61776783526164 18971100.0 7143528.933459585 1471.8267824858383 1946.7569010411592 100.0 777531.5475720335 22.621260572261072 35.844005213815 18971100.0 6837478.561673557 1485.95167336464 3236.103937273462 100.0 738950.089265769 14.178890700651673 28.360364294429065 18971100.0 6757253.548202883 1482.5957931512892 3822.6081352512965 100.0 673652.0401617718 15.80467786341627 31.051288166051528 18971100.0 7102291.52483768 1469.892237023601 2274.2011372615084
6.0 100.0 687720.4674964088 21.93642445072844 34.72871124316962 20695800.0 7345269.002366011 1489.3550038354936 2246.172104487999 100.0 688094.7343626507 21.93642445072844 34.72871124316962 20695800.0 7344644.336189428 1489.244626541849 2246.172104487999 100.0 682033.4907947287 21.845277943777717 36.35278831185687 20695800.0 7209271.218703909 1498.2696449272237 3244.088031556067 100.0 677071.1382888565 15.526528822661549 31.12821824944701 20695800.0 7053044.417641297 1500.0618585888308 4210.366395525026 100.0 638212.6297968253 16.811215141675937 33.2114225974881 20695800.0 7314517.164048839 1488.4065154415653 2706.5360097030134
6.5 100.0 659559.9575629814 20.953789186915195 35.93284891146218 22420400.0 7494276.548062428 1506.8233647884786 2583.960255933734 100.0 659830.6616260277 20.953789186915195 35.93284891146218 22420400.0 7493576.944695165 1506.8173065925957 2583.960255933734 100.0 632112.2747118229 20.894672756284862 36.74746950365976 22420400.0 7462770.738812381 1511.8793842014331 3261.811206010998 100.0 623120.9513268851 16.880934790729025 33.96374600908499 22420400.0 7329189.443222389 1516.2335964613449 4595.521028002923 100.0 608896.3275567518 17.721662259105113 35.22824487562212 22420400.0 7489228.772884566 1506.7501870034914 3288.6936530113653
7.0 100.0 635884.947236669 19.49370843752775 37.14256941223103 24145100.0 7593512.129039755 1526.1784571360242 3619.0952898630867 100.0 636460.8224629129 19.49370843752775 37.14256941223103 24145100.0 7592832.972776879 1526.1191941131108 3619.0952898630867 100.0 608490.864465936 19.506936071559302 37.34813597672898 24145100.0 7607727.32281213 1528.2667955156307 3873.97018849884 100.0 577792.6612515771 18.22681377789455 36.72202073587437 24145100.0 7584428.993352683 1531.7643932593428 4971.828844478204 100.0 580423.1361995192 18.515334176115058 37.092131857183716 24145100.0 7629331.590147272 1526.998008124652 4215.649626201095


==> data/stats/pubmed.tex <==
degree mst-plus-best-filter-edge-modularity_cc_size mst-plus-best-filter-edge-modularity_effective_resistance mst-plus-best-filter-edge-modularity_global_clustering mst-plus-best-filter-edge-modularity_local_clustering mst-plus-best-filter-edge-modularity_number_of_edges mst-plus-best-filter-edge-modularity_number_of_trees mst-plus-best-filter-edge-modularity_number_of_triangles mst-plus-best-filter-edge-modularity_spectral_radius mst-plus-best-filter-edge-significance_cc_size mst-plus-best-filter-edge-significance_effective_resistance mst-plus-best-filter-edge-significance_global_clustering mst-plus-best-filter-edge-significance_local_clustering mst-plus-best-filter-edge-significance_number_of_edges mst-plus-best-filter-edge-significance_number_of_trees mst-plus-best-filter-edge-significance_number_of_triangles mst-plus-best-filter-edge-significance_spectral_radius mst-plus-best-filter-spectral-radius_cc_size mst-plus-best-filter-spectral-radius_effective_resistance mst-plus-best-filter-spectral-radius_global_clustering mst-plus-best-filter-spectral-radius_local_clustering mst-plus-best-filter-spectral-radius_number_of_edges mst-plus-best-filter-spectral-radius_number_of_trees mst-plus-best-filter-spectral-radius_number_of_triangles mst-plus-best-filter-spectral-radius_spectral_radius random-plus-tree_cc_size random-plus-tree_effective_resistance random-plus-tree_global_clustering random-plus-tree_local_clustering random-plus-tree_number_of_edges random-plus-tree_number_of_trees random-plus-tree_number_of_triangles random-plus-tree_spectral_radius random-tree_cc_size random-tree_effective_resistance random-tree_global_clustering random-tree_local_clustering random-tree_number_of_edges random-tree_number_of_trees random-tree_number_of_triangles random-tree_spectral_radius
1.1 100.0 2520538.046528393 0.6164031733348554 0.7399221686385046 2168800.0 450143.2072937694 1174.363636284402 656.2009322759095 100.0 2522676.031732551 0.6164031733348554 0.7399221686385046 2168800.0 448565.82287532336 1174.2440987347663 656.2009322759095 100.0 2496842.2389199813 1.8800040077604818 1.5234992175778446 2168800.0 389064.7861221353 1182.6922960615202 975.8577887947511 100.0 2214254.078295334 0.22399593807122414 0.3038412543424128 2168800.0 437056.62853487465 1183.190276088359 843.7584302230864 100.0 2189667.812538289 0.2205694162430985 0.38457918912017 2168800.0 454908.1028771241 1182.40594537143 842.9141541142739
1.2 100.0 2191338.7245867704 0.8879363135333742 1.0252687358737977 2366000.0 643054.1564453033 1189.0977974818259 656.2103334416616 100.0 2192075.53281852 0.8879363135333742 1.0252687358737977 2366000.0 644424.6952806658 1189.054194485439 656.2103334416616 100.0 2283362.6198515655 3.043087399395488 2.133868714352829 2366000.0 530378.5763463664 1200.344010171019 1381.0937112005752 100.0 2018996.0094304238 0.5328265694498177 0.6757970517483703 2366000.0 592494.9814672759 1197.896574539033 886.0672745820974 100.0 1974678.9404424406 0.42634623350705825 0.749694213552945 2366000.0 635561.8362338124 1195.852519190764 867.5065362941016
1.3 100.0 1958857.5799550693 1.0400811770674783 1.2299193725195172 2563200.0 811696.8918026611 1202.2389648927515 656.2444533850845 100.0 1958576.818601913 1.0400811770674783 1.2299193725195172 2563200.0 811587.7814863253 1202.227208522606 656.2444533850845 100.0 2011357.0337507746 3.587948350071736 2.6680088917703304 2563200.0 687652.2924902599 1215.050704904675 1583.1496025799713 100.0 1884305.9684129877 0.8747424061777 1.0206305118197383 2563200.0 724377.6063389431 1211.6195516328748 942.2115392289845 100.0 1823789.3998142686 0.648056248308679 1.1740956687104114 2563200.0 789087.4859147678 1208.5572279767437 895.3660873904994
1.4 100.0 1790231.3496880336 1.2725795845743242 1.5336377510659864 2760300.0 955941.2399664685 1214.706431353453 656.2823220313664 100.0 1791246.855332919 1.2725795845743242 1.5336377510659864 2760300.0 955469.7527113709 1214.7632512397995 656.2823220313664 100.0 1870476.2136771467 3.6290495550672763 2.9953072304574326 2760300.0 816366.9724761964 1228.386342793039 1584.6508283996632 100.0 1783503.5928500213 1.286157836807298 1.4739296533680912 2760300.0 840693.8362552504 1224.3807530044999 1012.8279924749952 100.0 1704116.5306775693 0.8609325522155098 1.5998110508159142 2760300.0 925400.9992625033 1220.6692120097011 930.9786244664672
1.5 100.0 1665269.3692235057 1.5528186208019097 1.921706090073944 2957500.0 1081479.632996606 1226.6735294624275 674.7429728677929 100.0 1666471.3652633436 1.5528186208019097 1.921706090073944 2957500.0 1081424.44348809 1226.724323519926 674.7429728677929 100.0 1765712.3403149839 3.5000316065615227 3.3027545071034723 2957500.0 924103.2803528729 1240.9415973096372 1587.180115491561 100.0 1698915.0844871209 1.7210300768524236 1.915515511510544 2957500.0 945793.4988897581 1237.1634414290982 1153.0334042330078 100.0 1608545.2290232095 1.1250909031342313 2.028621796840726 2957500.0 1044381.143782738 1232.0745928540866 966.0714265973022
2.0 100.0 1403026.5564297084 3.4249146757679183 4.381941935406459 3943400.0 1444280.2720363135 1281.2659439347267 1164.6477647600566 100.0 1402472.4259590684 3.4249146757679183 4.381941935406459 3943400.0 1445172.88545448 1281.0053402997682 1164.6477647600566 100.0 1358885.6700634668 4.381144345775732 5.295954457754095 3943400.0 1409795.5564057028 1293.0006921922802 2039.2489480720587 100.0 1408195.5025370892 4.120548323740052 4.542755388142831 3943400.0 1365799.341892583 1291.7862107864426 1927.435166754091 100.0 1371915.3791510335 2.9175788272043803 4.447002919568495 3943400.0 1439742.607131353 1283.9195927835842 1375.5020337939832


==> data/stats/sbm.tex <==
n mst_plus_best_filter_edge_modularity_algebraic_connectivity mst_plus_best_filter_edge_modularity_ami mst_plus_best_filter_edge_modularity_ari mst_plus_best_filter_edge_modularity_cc_size mst_plus_best_filter_edge_modularity_effective_resistance mst_plus_best_filter_edge_modularity_global_clustering mst_plus_best_filter_edge_modularity_local_clustering mst_plus_best_filter_edge_modularity_modularity mst_plus_best_filter_edge_modularity_nmi mst_plus_best_filter_edge_modularity_number_of_edges mst_plus_best_filter_edge_modularity_number_of_trees mst_plus_best_filter_edge_modularity_number_of_triangles mst_plus_best_filter_edge_modularity_spectral_radius mst_plus_best_filter_edge_significance_algebraic_connectivity mst_plus_best_filter_edge_significance_ami mst_plus_best_filter_edge_significance_ari mst_plus_best_filter_edge_significance_cc_size mst_plus_best_filter_edge_significance_effective_resistance mst_plus_best_filter_edge_significance_global_clustering mst_plus_best_filter_edge_significance_local_clustering mst_plus_best_filter_edge_significance_modularity mst_plus_best_filter_edge_significance_nmi mst_plus_best_filter_edge_significance_number_of_edges mst_plus_best_filter_edge_significance_number_of_trees mst_plus_best_filter_edge_significance_number_of_triangles mst_plus_best_filter_edge_significance_spectral_radius mst_plus_best_filter_spectral_radius_algebraic_connectivity mst_plus_best_filter_spectral_radius_ami mst_plus_best_filter_spectral_radius_ari mst_plus_best_filter_spectral_radius_cc_size mst_plus_best_filter_spectral_radius_effective_resistance mst_plus_best_filter_spectral_radius_global_clustering mst_plus_best_filter_spectral_radius_local_clustering mst_plus_best_filter_spectral_radius_modularity mst_plus_best_filter_spectral_radius_nmi mst_plus_best_filter_spectral_radius_number_of_edges mst_plus_best_filter_spectral_radius_number_of_trees mst_plus_best_filter_spectral_radius_number_of_triangles mst_plus_best_filter_spectral_radius_spectral_radius random_plus_tree_algebraic_connectivity random_plus_tree_ami random_plus_tree_ari random_plus_tree_cc_size random_plus_tree_effective_resistance random_plus_tree_global_clustering random_plus_tree_local_clustering random_plus_tree_modularity random_plus_tree_nmi random_plus_tree_number_of_edges random_plus_tree_number_of_trees random_plus_tree_number_of_triangles random_plus_tree_spectral_radius random_tree_algebraic_connectivity random_tree_ami random_tree_ari random_tree_cc_size random_tree_effective_resistance random_tree_global_clustering random_tree_local_clustering random_tree_modularity random_tree_nmi random_tree_number_of_edges random_tree_number_of_trees random_tree_number_of_triangles random_tree_spectral_radius
1000.0 0.2947619768813116 0.0745319524797431 0.03761932304472337 1.0 758.6535822932943 0.014725508849963894 0.021031221080466133 0.515315906125 0.10380766784234201 2000.0 585.2515547369702 10.151655679866062 12.54720092442751 0.294761976881312 0.0745319524797431 0.03761932304472337 1.0 758.6454682456431 0.014725508849963894 0.021031221080466133 0.515315906125 0.10380766784234201 2000.0 585.6095308875354 10.152907642951238 12.547200924427512 0.30164867679032836 0.07252228901235232 0.03647379574972416 1.0 765.4816302953604 0.016280413072184294 0.022628513504157934 0.515265305375 0.10197392128431602 2000.0 573.9015585372324 10.165520263614606 12.924590326476356 0.2422870020856219 0.027418988242844323 0.009985742773048208 1.0 482.0838088914196 0.003813305099998824 0.003636453957153957 0.5299420371250001 0.06003980262778029 2000.0 1110.6500958560407 9.321264970451397 4.954328846133596 0.47717112197278505 0.02682126552035432 0.009756950311465269 1.0 433.6220260960406 0.0029902511508683163 0.003331309140859141 0.5301207448749999 0.059428856654678654 2000.0 1154.3660709851017 9.295785920116305 4.601454108364458
2000.0 0.2769270630006692 0.05744998690837889 0.02416950041196034 1.0 1521.1092911365424 0.007680209962098545 0.011004515814838476 0.5235932786875 0.07644016274915345 4000.0 1159.4508055004665 10.844075961193115 12.770556119351443 0.2769270630006693 0.05744998690837889 0.02416950041196034 1.0 1521.1573840330225 0.007680209962098545 0.011004515814838476 0.5235932786875 0.07644016274915345 4000.0 1159.8945434655004 10.843761318984333 12.770556119351443 0.28303832693869857 0.056886815062998676 0.024085706009128974 1.0 1534.179312634668 0.00844832144069395 0.011826247023270647 0.52355061459375 0.07590173036309251 4000.0 1137.8335557510964 10.85625092958858 13.149689773027209 0.2112565566675593 0.018404951815626666 0.005895849939799819 1.0 952.5765924616965 0.001944922928070945 0.00184187437007437 0.533631054 0.03867093370651043 4000.0 2223.140714086667 10.013283115618718 4.96080092102784 0.458814852952911 0.01785549964692057 0.005660597918020594 1.0 847.1648420905209 0.0015136948011668357 0.0016648047619047617 0.5333361118437501 0.038291730124500455 4000.0 2311.776972309729 9.98753339856159 4.603018767381929
3000.0 0.2666971101132817 0.0482213319957211 0.01798487500004525 1.0 2282.5338982756552 0.005172596209379248 0.0074200878228008966 0.52643563475 0.0628827403024601 6000.0 1734.9234134435785 11.249768969937088 12.850758628449945 0.2666971101132814 0.0482213319957211 0.01798487500004525 1.0 2282.636517369118 0.005172596209379248 0.0074200878228008966 0.52643563475 0.0628827403024601 6000.0 1734.6185541594116 11.249200464698385 12.850758628449945 0.2743207137344809 0.04752048489704597 0.017857359835390524 1.0 2302.429377761514 0.005694302895490877 0.008009562144611505 0.5260202342777778 0.0622053334446684 6000.0 1701.2360616050146 11.261836633565192 13.230638500334258 0.19776907707249922 0.014060970295938833 0.004104036137981934 1.0 1423.9302082229503 0.0013377950939701835 0.0012750212102712105 0.5334631250972223 0.029489088573671197 6000.0 3335.991165537725 10.41839674677958 4.960299374428478 0.4486307769072788 0.013794980467147649 0.004005687221870928 1.0 1264.5709850015771 0.0010225800251014454 0.001123103896103896 0.532465244 0.02921954374738062 6000.0 3468.9912328777955 10.39271753400195 4.603419010350451
4000.0 0.26136145085463647 0.04173918123310307 0.014183820197011802 1.0 3042.9218541532578 0.003865563578211954 0.0055391592816724945 0.5277258471171875 0.05392770526942698 8000.0 2310.428817085755 11.537488148024138 12.885674659023051 0.2613614508546366 0.04173918123310307 0.014183820197011802 1.0 3042.9484147873504 0.003865563578211954 0.0055391592816724945 0.5277258471171875 0.05392770526942698 8000.0 2310.941497839885 11.536979405883484 12.885674659023051 0.2690027157533378 0.04137235214198823 0.014176487250976678 1.0 3068.635686403284 0.004257763376929777 0.0059777607406990676 0.5276178333203124 0.053517647666173826 8000.0 2267.7085901570094 11.548907854928053 13.261948824749968 0.18524556349598048 0.011520217160177737 0.0031689866200919504 1.0 1895.5537190308044 0.0009994434821827736 0.0009567644758019758 0.532349174359375 0.024086963120005803 8000.0 4448.576630273132 10.705925719520772 4.963115255980412 0.439085941957372 0.011029527400568742 0.003056941940892823 1.0 1682.716126369137 0.0007726351818976694 0.0008515011974136974 0.5316281359609376 0.02354635072558527 8000.0 4625.439652261697 10.680401353706246 4.604732725467288
5000.0 0.2575892563334435 0.036249610434401724 0.01143475219518417 1.0 3805.2689493642515 0.003125389312575169 0.0044684153612044 0.5289538628099999 0.046776673965326955 10000.0 2884.3433252332784 11.760451191158417 12.913858460757762 0.2575892563334435 0.036249610434401724 0.01143475219518417 1.0 3805.127788556068 0.003125389312575169 0.0044684153612044 0.5289538628099999 0.046776673965326955 10000.0 2884.6753741831994 11.760137181491434 12.913858460757758 0.2646820517719799 0.03668600053120346 0.011669199713010735 1.0 3836.850689854984 0.003432090423037313 0.004796898692893463 0.528612042405 0.04720317534892581 10000.0 2831.189333984811 11.77205011179919 13.289022751681637 0.17957997908308812 0.009767286484037577 0.002571443107306301 1.0 2368.1949748202883 0.0007924155057743151 0.0007568249406149406 0.531463056795 0.020493455707724123 10000.0 5560.377990988577 10.929142640057254 4.9639079454094315 0.4326741398946551 0.009235520485716695 0.002444800150998862 1.0 2100.4991482291 0.000605137156266714 0.000663372069042069 0.531137009465 0.01986685305542475 10000.0 5782.4781935588635 10.903416075331418 4.604245746712983
6000.0 0.25277067969355504 0.03376165217464386 0.009999561676938636 1.0 4568.11584658275 0.0026133004040088427 0.0037565433887197085 0.5297928911388888 0.0430898353932091 12000.0 3458.5806532629204 11.942295235047228 12.92723065495754 0.25277067969355516 0.03376165217464386 0.009999561676938636 1.0 4568.170975488195 0.0026133004040088427 0.0037565433887197085 0.5297928911388888 0.0430898353932091 12000.0 3458.1477399457895 11.942394042098382 12.92723065495754 0.2616403489785931 0.03339068632769777 0.010005387133555931 1.0 4605.713333919652 0.0028722785343977338 0.004042754521752356 0.5296124452395833 0.042706184821163465 12000.0 3395.195111290418 11.954306025582223 13.302453610055217 0.17073755175731406 0.008472397830928097 0.002155970712490154 1.0 2839.7317438237965 0.0006605727494347747 0.0006266750462500463 0.5308155936770834 0.01787309560866779 12000.0 6673.299557196413 11.111285376792207 4.963820856925466 0.43048184825111946 0.008054156214591877 0.0020608302490852273 1.0 2519.2781562528107 0.0005148810912237742 0.0005733639332889334 0.5309076078888888 0.01736581835261378 12000.0 6939.4809003649125 11.085702197780378 4.605295416940258
7000.0 0.2485318084149928 0.03093704542464571 0.008690702768932813 1.0 5333.402035484437 0.002246934298395472 0.003187487249941098 0.5308210194727891 0.039362912032077056 14000.0 4030.046286872459 12.09580696948572 12.939139367121347 0.24853180841499292 0.03093704542464571 0.008690702768932813 1.0 5333.571538907694 0.002246934298395472 0.003187487249941098 0.5308210194727891 0.039362912032077056 14000.0 4029.739436327313 12.095113432624643 12.939139367121347 0.2564623393186889 0.030640755624199215 0.008717500335567773 1.0 5374.086486209056 0.0024531520137775014 0.003442235341468427 0.5303620957537853 0.03904793360603777 14000.0 3958.200959560315 12.10765571506392 13.314555424816017 0.1663150346572916 0.007479518478624701 0.0018424113821499638 1.0 3312.9235920360134 0.0005800045422652683 0.0005528354530773885 0.5305820559002634 0.01587181847344732 14000.0 7784.5455058509115 11.265565771773876 4.965445597306702 0.4252359273608304 0.007247520452211702 0.001793488160812419 1.0 2937.973380973864 0.00045242943797192843 0.000499318427774649 0.5307744985791091 0.015585974324713207 14000.0 8096.001450482258 11.239798494526127 4.605155324985061
8000.0 0.24896484896952364 0.028493123764051605 0.007659318917986424 1.0 6088.976085273311 0.0019589605082320064 0.002800448721617819 0.5313974364413175 0.03619377121012636 16000.0 4610.761864722801 12.22964679650031 12.941113837226654 0.24896484896952423 0.028493123764051605 0.007659318917986424 1.0 6089.149917346641 0.0019589605082320064 0.002800448721617819 0.5313974364413175 0.03619377121012636 16000.0 4611.72528407496 12.230076326190883 12.941113837226654 0.25630164890908136 0.028192486923942252 0.007659613484379513 1.0 6138.6292761708155 0.0021538797053109776 0.0030303799521829997 0.5311337480379972 0.035873173405965866 16000.0 4526.706131944309 12.241232242514313 13.315545564912373 0.16375114895404308 0.006776705918498818 0.0016227692602209232 1.0 3782.829190830368 0.0004948931242813344 0.000474399032154714 0.5303008767622515 0.014403606314809764 16000.0 8898.542795451373 11.398790402826828 4.9641070269600025 0.42087143153890155 0.006588733099462061 0.0015813130089984305 1.0 3356.441761726917 0.0003915060292384633 0.00043741820994661903 0.5307091569446911 0.014159341278007834 16000.0 9253.529083969186 11.373180357888891 4.604951933379638
9000.0 0.24492511955678967 0.025957576780307474 0.006701356905954893 1.0 6849.032720750961 0.0017278143953725065 0.0024785668650520514 0.5316003751693766 0.033055121081312616 18000.0 5187.085338369304 12.347361831765419 12.947919330908837 0.24492511955679086 0.025957576780307474 0.006701356905954893 1.0 6848.7814674844785 0.0017278143953725065 0.0024785668650520514 0.5316003751693766 0.033055121081312616 18000.0 5187.195439419245 12.347832781704238 12.947919330908837 0.25268340963893715 0.026257157928291818 0.006816933772040264 1.0 6908.122540696002 0.001910439832517727 0.00268056736036218 0.5314602668812105 0.033364769862340764 18000.0 5090.054234994449 12.358771482497415 13.322798588405794 0.15623457551185221 0.006221758196727334 0.0014582980947732767 1.0 4255.676334454143 0.0004443494899153385 0.0004260903580009271 0.5302120087737128 0.013227589263018584 18000.0 10011.59188827841 11.516718417636632 4.965659190423766 0.4192889420028359 0.005972354508692407 0.0014019345013054005 1.0 3775.4678584564385 0.00035400110269442545 0.0003941631178216544 0.5305568368375488 0.01293341899735774 18000.0 10409.461952662881 11.490953738748235 4.605611209637135
10000.0 0.2503012072631747 0.024935643715134258 0.006170131970048198 1.0 7621.575445364462 0.0015929328162155522 0.0023729346273663305 0.5321414499999999 0.03168369652185411 20000.0 5752.478877094603 12.452012521519194 12.949786503266086 0.2503012072631738 0.024935643715134258 0.006170131970048198 1.0 7619.107228514506 0.0015929328162155522 0.0023729346273663305 0.5321414499999999 0.03168369652185411 20000.0 5751.071641729808 12.453396739537842 12.949786503266086 0.26081380869891574 0.024407647913667636 0.006235595696051497 1.0 7680.04556327232 0.0017727159863901935 0.0025737052512809183 0.5311817440000001 0.031003910736239253 20000.0 5648.514663111657 12.464370346559523 13.320554693718794 0.15843284663925009 0.005667555958279081 0.0013173749218114363 1.0 4724.4462342692395 0.0003321252366183274 0.0003094134199134199 0.5305604481250001 0.01194721248432027 20000.0 11122.968088927515 11.622116600283883 4.961856179302955 0.41700306475459936 0.005588981340603421 0.0012615011122522625 1.0 4192.73220517373 0.00033423523517472225 0.00035209523809523805 0.530689229875 0.01210220193526922 20000.0 11574.349264490815 11.596051595526031 4.602417490864932

